Fast and Provable ADMM for Learning with Generative Priors

In this work, we propose a (linearized) Alternating Direction Method-of-Multipliers (ADMM) algorithm for minimizing a convex function subject to a nonconvex constraint. We focus on the special case where such constraint arises from the specification that a variable should lie in the range of a neural network. This is motivated by recent successful applications of Generative Adversarial Networks (GANs) in tasks like compressive sensing, denoising and robustness against adversarial examples. The derived rates for our algorithm are characterized in terms of certain geometric properties of the generator network, which we show hold for feedforward architectures, under mild assumptions. Unlike gradient descent (GD), it can efficiently handle non-smooth objectives as well as exploit efficient partial minimization procedures, thus being faster in many practical scenarios.

==> figures_tex/cs_image_comparison.tex <==
\newcommand{\mnistimagesb}{figures/0611AM_Jan_20}
\newcommand{\foldercelebaimages}{figures/celeba_images}

\begin{figure*}
\centering
\begin{subfigure}[t!]{0.45\textwidth}
\centering

\begin{places}{0.7\textwidth}{1}
\place{Original}{
  \mnistimagesb/originals.png
}
\addlinespace[-2.0ex]
\place{gd}{
  \mnistimagesb/gd_best.png
}
 \addlinespace[-1.8ex]
\place{admm}{
  \mnistimagesb/admm_best.png
}
 \addlinespace[-1.8ex]
\place{eadmm}{
  \mnistimagesb/eadmm_best.png
}
\end{places}
\caption{
    MNIST: 156 linear measurements. $10^3$ iterations and 3 random restarts.}
\label{fig:mnist_recovered}
\end{subfigure}
\qquad
\begin{subfigure}[t!]{0.45\textwidth}
    \centering
\begin{places}{0.7\textwidth}{1}
\place{Original}{
  \foldercelebaimages/originals.png
}
\addlinespace[-2.0ex]
\place{gd}{
  \foldercelebaimages/gd_best.png
}
 \addlinespace[-1.7ex]
\place{admm}{
  \foldercelebaimages/admm_best.png
}
 \addlinespace[-1.7ex]
\place{eadmm}{
  \foldercelebaimages/eadmm_best.png
}
\end{places}
\caption{
    CelebA: 2457 linear measurements. $8\times10^3$ iterations and 3 random restarts.}
\label{fig:celeba_recovered}

\end{subfigure}
\centering
\caption{
Recovered images for compressive sensing using 20\%
relative Gaussian measurements.}
\label{fig:cs_recovered_images}
\end{figure*}


==> figures_tex/cs_performance.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/3002_mnist_linear_comparison_synthetic.pdf}
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/3002_mnist_linear_error_comparison_synthetic.pdf}
    \caption{MNIST}
    \label{fig:cs_mnist}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/8006_celeba_linear_comparison_synthetic.pdf}
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/8006_celeba_linear_error_comparison_synthetic.pdf}
    \caption{CelebA}
    \label{fig:cs_celeba}
\end{subfigure}
\caption{$\ell_2$ squared measurement error and reconstruction error per iteration}
\end{figure*}


==> figures_tex/denoising_image_comparison.tex <==
\newcommand{\folderdenoisingmnistimages}{figures/0613AM_Jan_20}
\newcommand{\folderdenoisingcelebaimages}{figures/celebadenoising}

\begin{figure}
\centering
\begin{minipage}{0.49\textwidth}
\begin{places}{0.8\textwidth}{1}
\place{original}{
  \folderdenoisingcelebaimages/originals.png
}
\addlinespace[-2.0ex]
\place{noisy}{
  \folderdenoisingcelebaimages/noisy.png
}
 \addlinespace[-1.8ex]
\place{gd}{
  \folderdenoisingcelebaimages/gd_best.png
}
 \addlinespace[-1.8ex]
\place{eadmm}{
  \folderdenoisingcelebaimages/l1eadmm_best.png
}
\end{places}
\caption{
Denoised images with $\ell_1$ metric  from the CelebA dataset, with Gaussian noise standard deviation $0.4$, after 8000 Iterations.}
\label{fig:celeba_denoised}
\end{minipage} \hfill
\begin{minipage}{0.49\textwidth}
\centering
    \includegraphics[width=0.48\textwidth]{\comparisonfolder/3007_celeba_1_denoise_perf_comparison.pdf}
    \includegraphics[width=0.48\textwidth]{\comparisonfolder/3007_celeba_1_denoise_error_comparison_synthetic.pdf}
    \caption{$\ell_1$ measurement error (left) and reconstruction error (right) vs.\ iteration, with CelebA dataset.}
    \label{fig:celeba_denoising}
\end{minipage}
\end{figure}


==> figures_tex/denoising_performance.tex <==
%\begin{figure}
%\centering
%\begin{subfigure}{0.22\textwidth}
%    \includegraphics[width=\linewidth]{\comparisonfolder/12000_mnist_linearm_comparison_one_row.pdf}
%    \caption{MNIST}
%    \label{fig:mnist_m_comparison}
%\end{subfigure} \quad
%\begin{subfigure}{0.22\textwidth}
%    \includegraphics[width=\linewidth]{\comparisonfolder/12000_mnist_linearm_comparison_one_row.pdf}
%    \caption{CelebA}
%    \label{fig:celeba_m_comparison}
%\end{subfigure}
%\caption{Reconstruction error of the true image vs number of relative measurement. Best of 3 random restarts.}
%\end{figure}

\begin{figure}
    \centering
\begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth]{\comparisonfolder/3007_celeba_1_denoise_perf_comparison.pdf}
\end{subfigure} \quad
\begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth]{\comparisonfolder/3007_celeba_1_denoise_error_comparison_synthetic.pdf}
\end{subfigure}
    \caption{$\ell_1$ measurement error (left) and reconstruction error (right) vs.\ iteration, with CelebA dataset.}
\label{fig:celeba_denoising}
\end{figure}


==> neurips2019 copy/definitions.tex <==
\usepackage{amsmath, amssymb, amsthm}
\usepackage{physics}
\usepackage{hyperref}
\usepackage{color, xcolor, pagecolor}
\usepackage{xparse, booktabs}
%\hypersetup{
%  colorlinks=True,
%  linkcolor=cyan,
%  urlcolor=magenta,
%  citecolor=green,
%}

%\usepackage{algorithm,algorithmic}
\usepackage{enumitem}

\usepackage{comment}

% Frequently used
\newcommand{\R}{\mathbb{R}} % Real Numbers
\newcommand{\E}{\mathbb{E}} % Expectation
\DeclareMathOperator*{\argmin}{arg\,min} % argmin
\DeclareMathOperator*{\argmax}{arg\,max} % argmax
\newcommand{\loss}{L_M} % Loss function
\newcommand{\lossf}{l} % Loss function
\newcommand{\bigo}{\mathcal{O}} % Big O notation
\newcommand{\normb}[1]{\|#1\|}

\DeclareMathOperator*{\diag}{diag} % diagonal of matrix
\DeclareMathOperator*{\Diag}{Diag} % diagonal matrix from vector

\newcommand{\geqmat}{\succcurlyeq} % PSD matrix order relation
\newcommand{\ones}{\mathbf{1}} % ones vector

% Used in the current project
\newcommand{\U}{U} % signals (edited from \X on Nov 21)
\newcommand{\up}{u} % signal (edited from \x on Nov 21)
\newcommand{\Lagr}{\mathcal{L}} % Lagrangian
\newcommand{\F}{\mathcal{F}} % function class
\newcommand{\G}{\mathcal{G}} % function class
\newcommand{\D}{D} % Bregman divergence
\newcommand{\Dom}{\mathcal{D}} % Domain
\newcommand{\Sprior}{\mathcal{Z}} % prior space
\newcommand{\prior}{z} % prior variable
\newcommand{\Prior}{Z} % prior variable
\newcommand{\Proj}{\text{P}} % projection
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\newcommand{\wh}[1]{#1^*}
\renewcommand{\b}{\beta} % Penalty weight
\renewcommand{\d}{\delta} % Error
\renewcommand{\k}{\kappa} % Convergence rates
\newcommand{\s}{\sigma} % Dual step size
\newcommand{\adjoint}{\dagger} % adjoint operator
\newcommand{\g}{\gamma} % Primal step size
\newcommand{\la}{\lambda} % Dual variable
\newcommand{\ol}[1]{\overline{#1}}
\renewcommand{\t}{\theta}
\renewcommand{\a}{\alpha}
\newcommand{\n}{\natural}

% Theorem style
\newtheorem{theorem}{Theorem} % reset theorem numbering for each section
\newtheorem{question}[theorem]{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}

%% Dark mode for screen, remove when printing (requires color, xcolor, pagecolor)
%\color{gray!40}
%\pagecolor{gray!100!black!165}

% FOLDERS FOR IMAGES

\newcommand{\mnistreallinearonehundredelu}{figures/mnist_real_linear_100_elu/0211AM_Jan_11}
\newcommand{\mnistreallineartwohundredelu}{figures/mnist_real_linear_200_elu/0211AM_Jan_11}
\newcommand{\mnistreallinearfourhundredelu}{figures/mnist_real_linear_400_elu/0211AM_Jan_11}

\newcommand{\mnistsyntheticlinearonehundredelu}{figures/mnist_synthetic_linear_100_elu/0211AM_Jan_11}
\newcommand{\mnistsyntheticlineartwohundredelu}{figures/mnist_synthetic_linear_200_elu/0211AM_Jan_11}
\newcommand{\mnistsyntheticlinearfourhundredelu}{figures/mnist_synthetic_linear_400_elu/0211AM_Jan_11}

\newcommand{\celebareallineartwohundredelu}{figures/celeba_real_linear_200_elu/0427PM_Jan_13}
\newcommand{\celebareallinearfourhundredelu}{figures/celeba_real_linear_400_elu/0427PM_Jan_13}
\newcommand{\celebareallineareighthundredelu}{figures/celeba_real_linear_800_elu/0427PM_Jan_13}

\newcommand{\celebasyntheticlineartwohundredelu}{figures/celeba_synthetic_linear_200_elu/0427PM_Jan_13}
\newcommand{\celebasyntheticlinearfourhundredelu}{figures/celeba_synthetic_linear_400_elu/0427PM_Jan_13}
\newcommand{\celebasyntheticlineareighthundredelu}{figures/celeba_synthetic_linear_800_elu/0427PM_Jan_13}

\newcommand{\comparisonfolder}{figures/comparison}


\ExplSyntaxOn
\NewDocumentEnvironment{places}{mm}
 {% #1 is the desired width, #2 is the number of photos per line
  \setlength{\tabcolsep}{0pt} % no space between rows
  \dim_set:Nn \l_places_width_dim
   {
    (#1-\ht\strutbox-\dp\strutbox-2pt)/(#2)
   }
  \begin{tabular}{r @{\hspace{2pt}} *{#2}{c}}
 }
 {
  \end{tabular}
 }

\NewDocumentCommand{\place}{mm}
 {% #1 is the name of the place, #2 is the comma separated list of images
  \seq_set_from_clist:Nn \l_places_images_in_seq { #2 }
  \seq_set_map:NNn \l_places_images_out_seq \l_places_images_in_seq { \places_set_image:n {##1} }
  \seq_put_left:Nn \l_places_images_out_seq
   {
    %\begin{tabular}{c}\rotatebox[origin=c]{90}{\strut#1}\end{tabular}
    \begin{tabular}{c}\rotatebox[origin=c]{30}{\strut#1}\end{tabular}
    %\begin{tabular}{c}\rotatebox[origin=c]{0}{\strut#1}\end{tabular}
    %\begin{tabular}{c}{\strut#1}\end{tabular}
   }
  \seq_use:Nn \l_places_images_out_seq { & } \\ \addlinespace
 }

\dim_new:N \l_places_width_dim
\seq_new:N \l_places_images_in_seq
\seq_new:N \l_places_images_out_seq

\cs_new_protected:Nn \places_set_image:n
 {
  \makebox[\l_places_width_dim]
   {
    \begin{tabular}{c}
    \includegraphics[
      width=\l_places_width_dim,
      height=\l_places_width_dim,
      keepaspectratio,
    ]{#1}
    \end{tabular}
   }
 }

\ExplSyntaxOff


\newcommand{\edita}[1]{{\color{red} #1}}
\newcommand{\editf}[1]{{\color{blue} #1}}


%\usepackage{pagecolor}
%\pagecolor{black}
%\color{white}
\usepackage{marginnote}


==> neurips2019 copy/figures_tex/attacks_performance.tex <==
%\begin{wrapfigure}{r}{0.49\textwidth}
%    \centering
%        \includegraphics[scale=0.8]{\comparisonfolder/attack_comparison_error_time9.pdf}
%    \caption{Test error on denoised adversarial examples vs computation time.}
%    \label{fig:attack_error_time}
%\end{wrapfigure}
%
%\begin{wrapfigure}{r}{0.49\textwidth}
%    \centering
%        \includegraphics[scale=0.8]{\comparisonfolder/mnist_denoising_meas_-1.pdf}
%    \caption{$\ell_\infty$ reconstruction error per iteration for ADAM, GD, and EADMM.}
%    \label{fig:linf_comparison}
%\end{wrapfigure}

\begin{figure}
    \centering
    \begin{minipage}{0.49\textwidth}
        \includegraphics[scale=0.7]{\comparisonfolder/attack_comparison_error_time9.pdf}
    \caption{Test error on denoised adversarial examples vs computation time.}
    \label{fig:attack_error_time}
    \end{minipage} \hfill
    \begin{minipage}{0.49\textwidth}
    \centering
        \includegraphics[scale=0.7]{\comparisonfolder/mnist_denoising_meas_-1.pdf}
    \caption{$\ell_\infty$ reconstruction error per iteration for ADAM, GD, and EADMM.}
    \label{fig:linf_comparison}
\end{minipage}
\end{figure}


==> neurips2019 copy/figures_tex/cs_image_comparison.tex <==
\newcommand{\mnistimagesb}{figures/0611AM_Jan_20}
\newcommand{\foldercelebaimages}{figures/celeba_images}

\begin{figure*}
\centering
\begin{subfigure}[t!]{0.45\textwidth}
\centering

\begin{places}{0.7\textwidth}{1}
\place{Original}{
  \mnistimagesb/originals.png
}
\addlinespace[-2.0ex]
\place{gd}{
  \mnistimagesb/gd_best.png
}
 \addlinespace[-1.8ex]
\place{admm}{
  \mnistimagesb/admm_best.png
}
 \addlinespace[-1.8ex]
\place{eadmm}{
  \mnistimagesb/eadmm_best.png
}
\end{places}
\caption{
    MNIST: 156 linear measurements. $10^3$ iterations and 3 random restarts.}
\label{fig:mnist_recovered}
\end{subfigure}
\qquad
\begin{subfigure}[t!]{0.45\textwidth}
    \centering
\begin{places}{0.7\textwidth}{1}
\place{Original}{
  \foldercelebaimages/originals.png
}
\addlinespace[-2.0ex]
\place{gd}{
  \foldercelebaimages/gd_best.png
}
 \addlinespace[-1.7ex]
\place{admm}{
  \foldercelebaimages/admm_best.png
}
 \addlinespace[-1.7ex]
\place{eadmm}{
  \foldercelebaimages/eadmm_best.png
}
\end{places}
\caption{
    CelebA: 2457 linear measurements. $8\times10^3$ iterations and 3 random restarts.}
\label{fig:celeba_recovered}

\end{subfigure}
\centering
\caption{
Recovered images for compressive sensing using 20\%
relative Gaussian measurements.}
\label{fig:cs_recovered_images}
\end{figure*}


==> neurips2019 copy/figures_tex/cs_performance.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/3002_mnist_linear_comparison_synthetic.pdf}
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/3002_mnist_linear_error_comparison_synthetic.pdf}
    \caption{MNIST}
    \label{fig:cs_mnist}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/8006_celeba_linear_comparison_synthetic.pdf}
    \includegraphics[width=0.45\textwidth]{\comparisonfolder/8006_celeba_linear_error_comparison_synthetic.pdf}
    \caption{CelebA}
    \label{fig:cs_celeba}
\end{subfigure}
\caption{$\ell_2$ squared measurement error and reconstruction error per iteration}
\end{figure*}


==> neurips2019 copy/figures_tex/denoising_image_comparison.tex <==
\newcommand{\folderdenoisingmnistimages}{figures/0613AM_Jan_20}
\newcommand{\folderdenoisingcelebaimages}{figures/celebadenoising}

\begin{figure}
\centering
\begin{minipage}{0.49\textwidth}
\begin{places}{0.8\textwidth}{1}
\place{original}{
  \folderdenoisingcelebaimages/originals.png
}
\addlinespace[-2.0ex]
\place{noisy}{
  \folderdenoisingcelebaimages/noisy.png
}
 \addlinespace[-1.8ex]
\place{gd}{
  \folderdenoisingcelebaimages/gd_best.png
}
 \addlinespace[-1.8ex]
\place{eadmm}{
  \folderdenoisingcelebaimages/l1eadmm_best.png
}
\end{places}
\caption{
Denoised images with $\ell_1$ metric  from the CelebA dataset, with Gaussian noise standard deviation $0.4$, after 8000 Iterations.}
\label{fig:celeba_denoised}
\end{minipage} \hfill
\begin{minipage}{0.49\textwidth}
\centering
    \includegraphics[width=0.48\textwidth]{\comparisonfolder/3007_celeba_1_denoise_perf_comparison.pdf}
    \includegraphics[width=0.48\textwidth]{\comparisonfolder/3007_celeba_1_denoise_error_comparison_synthetic.pdf}
    \caption{$\ell_1$ measurement error (left) and reconstruction error (right) vs.\ iteration, with CelebA dataset.}
    \label{fig:celeba_denoising}
\end{minipage}
\end{figure}


==> neurips2019 copy/figures_tex/denoising_performance.tex <==
%\begin{figure}
%\centering
%\begin{subfigure}{0.22\textwidth}
%    \includegraphics[width=\linewidth]{\comparisonfolder/12000_mnist_linearm_comparison_one_row.pdf}
%    \caption{MNIST}
%    \label{fig:mnist_m_comparison}
%\end{subfigure} \quad
%\begin{subfigure}{0.22\textwidth}
%    \includegraphics[width=\linewidth]{\comparisonfolder/12000_mnist_linearm_comparison_one_row.pdf}
%    \caption{CelebA}
%    \label{fig:celeba_m_comparison}
%\end{subfigure}
%\caption{Reconstruction error of the true image vs number of relative measurement. Best of 3 random restarts.}
%\end{figure}

\begin{figure}
    \centering
\begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth]{\comparisonfolder/3007_celeba_1_denoise_perf_comparison.pdf}
\end{subfigure} \quad
\begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth]{\comparisonfolder/3007_celeba_1_denoise_error_comparison_synthetic.pdf}
\end{subfigure}
    \caption{$\ell_1$ measurement error (left) and reconstruction error (right) vs.\ iteration, with CelebA dataset.}
\label{fig:celeba_denoising}
\end{figure}


==> neurips2019 copy/sections/algorithm.tex <==
In this section, we adapt the powerful Alternating Descent Method of
Multipliers (ADMM)~\citep{Glowinski1975,Gabay1976,Boyd2011} to solve the
non-convex {problem}~\eqref{eq:emp loss min}. We define the corresponding \emph{augmented Lagrangian} with the dual variable $\lambda
\in \R^p$ as
\begin{equation}
\begin{split}
    & \Lagr_\rho(w, z, \lambda) := L(w)+ \langle w - G(\prior), \lambda \rangle + \frac{\rho}{2}\norm{w - G(\prior)}_2^2,
\end{split}
\label{eq:defn_aug_lagr}
\end{equation}
for a penalty weight $\rho>0$.
By a standard duality argument, \eqref{eq:emp loss min} is equivalent to
\begin{align}
\underset{w,z}{\text{min}}\, \underset{\lambda}{\text{max}} \,
  \Lagr_\rho(w,z,\lambda)+ R(w)+H(z).
  \label{eq:aug lagr}
\end{align}
Applied to \eqref{eq:aug lagr}, every iteration of ADMM would minimize
the augmented Lagrangian with respect to $z$, then with respect to $w$, and then
update the dual variable $\lambda$. Note that $\Lagr_\rho(w, z, \lambda)$ is often
non-convex with respect to $z$ due to the {nonlinearity of the} generator $G:\R^s \rightarrow \R^d$
and, consequently, the minimization step with respect to $z$ in ADMM is often
intractable. 

To overcome this limitation, we next \emph{linearize} ADMM.
%\edita{This linearization finds precedent in \citet{liu2017linearized},
%but without any convergence rates. \marginnote{\textbf{Can we find any more
%references?}}} 
In the following, we let $\Proj_R$ and $\Proj_H$ denote the
\emph{proximal maps} of $R$ and $H$, respectively~\citep{Parikh2014}.

The equivalence of problems \eqref{eq:emp loss min} and \eqref{eq:aug
lagr} motivates us to consider the following algorithm for the penalty weight $\rho>0$, the primal
step sizes  $\alpha, \beta>0$, and the positive dual step sizes $\{\s_t\}_{t\ge
0}$:
\begin{equation}
\begin{split}
z_{ t+1} &= \Proj_{\b H} \l( z_{ t} - \b \nabla_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) \r), \\
    w_{ t+1} &= \Proj_{\a R} \left( w_{t} - \a \nabla_{w}
                        \Lagr_{\rho}(w_{t}, z_{t+1},  \lambda_{t}) \right), \\
    \lambda_{t+1} &= \lambda_{ t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1})).
\end{split}
\label{eq:aug lagr alg}
\end{equation}
As opposed to ADMM, to solve \eqref{eq:emp loss min}, the linearized ADMM in \eqref{eq:aug lagr alg} takes only
one descent step in both $z$ and $w$,
%The linearized ADMM developed above for
%solving \eqref{eq:emp loss min} 
see Algorithm \ref{alg:admm} for the summary. The particular choice of the dual step sizes $\{\s_t\}_t$ in
Algorithm~\ref{alg:admm} ensures that the dual variables $\{\lambda_t\}_t$
remain bounded,  see~\citep{bertsekas1976penalty} for a precedent in the convex
literature. 

{
\paragraph{Algorithm 2.} Let us introduce an important variant of Algorithm~\ref{alg:admm}. In our setting, $\Lagr_\rho(w,z,\lambda)$ is in fact convex with respect to
$w$ and therefore Algorithm 2 replaces the first step in \eqref{eq:aug lagr alg}
with exact minimization over $w$. {This} exact minimization step can be
executed with an off-the-shelf convex solver, or might sometimes have a closed-form solution. Moreover, Algorithm 2 gradually increases the penalty weight to emulate a multi-scale structure. More specifically, for an integer $K$, consider  the sequences of penalty weights and primal step sizes $\{\rho_k,\a_k,\b_k\}_{k=1}^K$, specified as 
\begin{align}
\rho_k =   2^k\rho,
\qquad 
\a_k = 2^{-k} \a, 
\qquad 
\b_k  =2^{-k} \b,
\qquad k\le K.
\end{align}
Consider also a sequence of integers $\{n_k\}_{k=1}^K$, where 
\begin{align}
n_k = 2^k n,
\qquad k\le K,
\end{align}
for an integer $n$. At (outer) iteration $k$, Algorithm~2 executes $n_k$ iterations of Algorithm~\ref{alg:admm} with exact minimization over $w$. Then it passes the current iterates of $w$, $z$, and dual step size to the next (outer) iteration. Loosely speaking, Algorithm~2 has a multi-scale structure, allowing it to take larger steps initially and then slowing down as it approaches the solution.  As discussed in Section~\ref{sec:guarantees1}, the theoretical guarantees for Algorithm~\ref{alg:admm} also apply to Algorithm~2. 
%Moreover, Algorithm~2 is closely related to gradient descent in \citep{Bora2017} and, in this sense, we establish the first rates for GD, albeit in the limit case discussed in Section~\ref{sec:guarantees1}.
}
%e also Supplementary~\ref{sec:relations} for the relation  with
%other  algorithms, and the applicability of our theoretical guarantees. %for them.


%In addition to Algorithm~\ref{alg:admm}, we consider a variant that gradually increases the penalty weight, which we will refer to as Algorithm 2. For an integer $K$, consider  the sequences of penalty weights and primal step sizes $\{\rho_k,\a_k,\b_k\}_{k=1}^K$, specified as 
%\begin{align}
%\rho_k =   2^k\rho,
%\qquad 
%\a_k = 2^{-k} \a, 
%\qquad 
%\b_k  =2^{-k} \b,
%\qquad k\le K.
%\end{align}
%Consider also a sequence of integers $\{n_k\}_{k=1}^K$, where 
%\begin{align}
%n_k = 2^k n,
%\qquad k\le K,
%\end{align}
%for an integer $n$. At (outer) iteration $k$, Algorithm~2 executes $n_k$ iterations of Algorithm~\ref{alg:admm} and then passes the current $w$, $z$, and dual step size to the next (outer) iteration. Loosely speaking, Algorithm~2 has a multi-scale structure, allowing it to take large steps initially and then refine its iterations as it approaches the solution. 
%

As the closing remark, akin to the convex case~\citep{he2000alternating,xu2017admm}, it is also possible to devise a variant of Algorithm~\ref{alg:admm} with adaptive primal step sizes, which we leave for a future work. 


% In fact, the common fixed dual step size in convex optimization
% fails for our problem in practice. \edita{<---is the last sentence correct? }  


%To avoid tuning  $\rho$ we adaptively
%choose a penalty parameter for each iteration as follows: %, which we also use  in our convergence charcterizations:
%\begin{align*}
%\rho_t =
%\begin{cases}
%\rho_{t-1}, \qquad \text{if } \|w_t - G(z_t)\|_2 \le  \frac{\rho_{0}}{\sqrt{t\log^{{2}} (t+1)}},\\
%\\
%\rho_{t-1}
%\sqrt{\dfrac{(t+1)\log^{{2}}(t+2)}{t\log^{{2}} (t+1)}}, \qquad
%\text{otherwise}
%\end{cases}
%%\label{eq:beta rule}
%\end{align*}
%for $t \ge 1$ and initialization penalty $\rho_0 > 0$.

\begin{algorithm}
    \caption{Linearized ADMM for solving problem \eqref{eq:emp loss min}}
    \label{alg:admm}
    \textbf{Input: } Differentiable  $L$,
    proximal-friendly convex regularizers $R$ and $H$, differentiable  prior $G$,
    penalty weight $\rho>0$, primal step sizes $\alpha,\beta>0$, initial dual
    step size $\s_0>0$, primal initialization $w_0$ and $z_0$, dual
    initialization $\lambda_0$, stopping threshold $\tau_c>0$.
    \begin{algorithmic}[1]
    \For{$t=0,1,\ldots, T-1$}
    
        \State $z_{ t+1} \gets \Proj_{\b H} \l( z_{ t} - \b \nabla_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) \r)$ \Comment{primal updates}
   
        \State $w_{ t+1} \gets \Proj_{\a R} \left( w_{t} - \a \nabla_{w}
                        \Lagr_{\rho}(w_{t}, z_{t+1},  \lambda_{t}) \right)$
                        
        \State $\s_{t+1} \gets \min\left(\s_0, \dfrac{\s_0}{\|w_{t+1}-G(z_{t+1})\|_2 t\log^2(t+1)}   \right )$ \Comment{dual step size}
        \State $\lambda_{t+1} \gets \lambda_{t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1}))$ \Comment{dual update}

        \State $s \gets \dfrac{\norm{z_{t+1}-z_t}_2^2}{\a}+\dfrac{\norm{w_{t+1}-w_t}_2^2}{\b} + \s_t \norm{w_t - G(z_t)}_2^2 \le \tau_c$ \Comment{stopping criterion}
        \If {$s \leq  \tau_c$}
        \State
        \Return{$(w_{t+1}, z_{t+1})$}
        \EndIf
    \EndFor \\
    \Return{$(w_T,z_T)$}
    \end{algorithmic}
\end{algorithm}

%\begin{center}%
%\begin{algorithm}[h]
%{
%\caption{Linearized ADMM for solving Program \eqref{eq:emp loss min} }
%    \label{alg:admm}
%\vspace{3mm}
%%\textbf{Input:} Differentiable $L:\R^d\rightarrow\R$,
%%proximable convex regularizers $R:\R^d\rightarrow\R$ and $H:\R^s\rightarrow\R$,
%%differentiable generative model $G:\R^s\rightarrow\R^d$, penalty weight
%%$\rho>0$, positive primal step sizes $\alpha,\beta$, initial dual step size
%%$\s_0>0$, primal initialization $w_0\in \R^d$ and $z_0\in \R^s$, dual
%%initialization $\lambda_0\in \R^d$, stopping threshold $\tau_c>0$.
%\textbf{Input:} Differentiable loss $L$, proximable convex regularizers $R$ and
%$H$, differentiable  prior $G$, penalty weight $\rho>0$,
%primal step sizes $\alpha,\beta>0$, initial dual step size $\s_0>0$, primal
%initialization $w_0$ and $z_0$, dual initialization $\lambda_0$, stopping
%threshold $\tau_c>0$.
%\vspace{3mm}
%
%%\textbf{Output:} Estimates $w$
%%\vspace{3mm}
%
%\textbf{Body:}
%\\
%For $t=0,1,\cdots$ and until convergence, execute\\
%\begin{enumerate}[leftmargin=*]
%\item \textbf{(Primal updates)}
%\begin{equation*}
%\begin{split}
%    z_{ t+1} &= \Proj_{\b H} \l( z_{ t} - \b \nabla_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) \r) \\
%    w_{ t+1} &= \Proj_{\a R} \left( w_{t} - \a \nabla_{w}
%                        \Lagr_{\rho}(w_{t}, z_{t+1},  \lambda_{t}) \right)
%\end{split}
%\end{equation*}
%%where the augmented Lagrangian $\Lagr_\rho$ was defined in (\ref{eq:defn_aug_lagr}) and $\Proj_H$ and $\Proj_R$ are the corresponding proximal operators in (\ref{eq:defn_of_proxs}).
%\item \textbf{(Dual step size)}
%\begin{align*}
%& \s_{t+1} = \min\Big(\s_0, \frac{\s_0}{\|w_{t+1}-G(z_{t+1})\|_2 t\log^2(t+1)}   \Big)
%\end{align*}
%\item  \textbf{(Dual update)}
%$
%    \lambda_{t+1} = \lambda_{ t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1}))
%$
%\item \textbf{(Stopping criterion)} If
%\begin{align*}
%\frac{\| z_{t+1}-z_t \|_2^2}{\a}+\frac{\|w_{t+1}-w_t\|_2^2}{\b} + \s_t \|w_t - G(z_t)\|_2^2 \le \tau_c,
%\end{align*}
%\textbf{Return} $w_t, z_t$.
%
%\end{enumerate}
%}
%\end{algorithm}
%\end{center}


==> neurips2019 copy/sections/conclusion.tex <==
We evaluated the a linearized ADMM and its partial exact minimization variant EADMM
on the compressive sensing tasks and $\ell_1$ denoising tasks.


==> neurips2019 copy/sections/experiments.tex <==
We now benchmark the following algorithms for solving problem \eqref{eq:final_problem}:
\begin{itemize}
    \item \textbf{Gradient Descent (GD): } \citep{Bora2017} Perform a fixed
        number of gradient descent iterations for the function
        $\loss(G(\prior))$.

    \item \textbf{Projected Gradient Descent (PGD): } \citep{Shah2018,
        Hegde2018} Performs a step in the direction of the gradient of
        $\loss(w)$ and the resulting iterate $w'$ is projected back to
        $G(z)$ via minimization of the function $\norm{G(z) - w'}_2^2$. This
        projection step is approximately achieved via a fixed number of
        gradient descent iterations.

    \item \textbf{Inexact ADMM (IADMM): } \ref{alg:admm} (Ours).

    \item \textbf{Partial exact minimization ADMM (PADMM): } Our algorithm
        \ref{alg:admm} with the following change: we perform exact minimization
        on the primal variable $w$. For example, in the
        linear regression case this involves one matrix inversion per
        iteration. Performing SVD once on the measurement matrix $X$ allows us
        to perform such inversion with small overhead per iteration.
\end{itemize}

We now describe the generator architecture $G$, for each of the test datasets
that we consider:
\begin{itemize}
    \item \textbf{MNIST:} We use the same architecture as one in \cite{gulrajani2017improved},
        which contains one fully-connected layer followed by three deconvolutional layers.
    \item \textbf{LSUN \& CelebA:} As a practice in \cite{gulrajani2017improved},
        we downsampled the images into $64 \times 64$ pixels and use the same generator architecture.
        The generator networks includes 4 residual blocks followed by a convolutional layer.
\end{itemize}

Notice that in the the \textit{Deep Image Prior} setting, we use the
network architecture initialized with random weight matrices. We consider
three different tasks: $(i)$ Linear regression with generative prior (LIN-G),
$(ii)$ Phase retrieval with generative prior (PHASE-G), and $(iii)$
Linear Regression with deep image prior (LIN-DIP). For MNIST we run the
algorithms for $4000$ iterations using either $100$, $200$ or $400$ measurements.
For the CelebA and LSUN datasets we use $8000$ iterations using either
$200$, $800$ or $1600$ measurements. For the (LIN-G) and (PHASE-G) tasks, we
consider two scenarios for the test images: either we choose random images from
a test set, not used for the training of the generative model, or we choose
random images on the image of the generative model, by choosing random latent
vectors $z$. For the (LIN-DIP) task we consider only images on a test set.

%\begin{figure}[H]
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/originals.png}
%    \label{fig:1}
%  \end{subfigure}
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/gd.png}
%    \label{fig:2}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/admm.png}
%    \label{fig:3}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/eadmm.png}
%    \label{fig:4}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/pgd.png}
%    \label{fig:5}
%  \end{subfigure}%
%
%  \caption{Recovered test images from 200 linear measurements. MNIST dataset.
%  From top to bottom: Original images, GD, IADMM (ours), PADMM (ours), PGD.}
%  \label{fig:images}
%\end{figure}
%
%\begin{figure}[H]
%    \centering
%    \includegraphics[width=\linewidth]{\comparisonfolder/4000_mnist_comparison.pdf}
%    \label{fig:mnist_comparison}
%
%    \caption{Function value across iterations for task (LIN-G). Recovering images on the test set (top).
%    Recovering images on the range of the generator (bottom).}
%  \label{fig:images}
%\end{figure}


==> neurips2019 copy/sections/experiments_old.tex <==
In this section we evaluate our algorithms for image recovery tasks with a GAN
prior. The datasets we consider are the CelebA dataset of face images \citep{Liu2015}
and the MNIST dataset of handwritten digits~\citep{Lecun2010}. We
train a generator $G$ with ELU activation functions~\cite{clevert2015fast}, in
order to satisfy Assumption~\ref{assump:G_ssmth}. The generators are trained
using the Wasserstein GAN framework \citep{Arjovsky2017}. For the CelebA
dataset we downsample the images to $64 \times 64$ pixels as
in~\citet{gulrajani2017improved} and we use the same residual architecture
\citep{He2015} for the generator with four residual blocks followed by a
convolutional layer. For MNIST, we use the same architecture as one
in~\cite{gulrajani2017improved}, which contains one fully connected layer
followed by three deconvolutional layers.

We recover images on the range of the generator $G$, by choosing $z^\star \in
\mathbb{R}^s$ and setting $w^\star:=G(z^\star)$ as the true image to be
recovered. This sets the global minimum of our objective functions at zero, and
allows us to illustrate and compare the convergence rates of various algorithms.

Our Algorithm \ref{alg:admm} mantains iterates $\{w_t, z_t\}_t$ where $w_t$
might not be feasible, namely, $w_t$ might not be in the range of $G$. As the goal
in the following tasks is to recover an element in the range of $G$ (feasible
points of \eqref{eq:emp loss min}), we plot the objective value at the point $G(z_t)$.

\textbf{Baseline. } We compare to the most widely-used algorithm in the current
literature, the gradient descent algorithm (GD) as used in \citep{Bora2017},
where a fixed number of iterations with constant step size are performed for
the function $L(G(z))$. We tune its learning rate to be as large
as possible without \textit{overshooting}. (See Supplementary \ref{sec:exp_setup}
for details on the hyperparameter tuning).

Our goal is to illustrate our theoretical results and highlight scenarios
where Algorithm \ref{alg:admm} can have better performance than GD in
optimization problems with a generative prior. Hence, we do not compare with
sparsity-prior based algorithms, such as LASSO \citep{Tibshirani1996}, or argue
about GAN vs.\ sparsity priors as in \cite{Bora2017}.

\textbf{Our algorithms. } We will use $(i)$ (linearized) 
ADMM (Algorithm \ref{alg:admm}), and ($ii$) ADMM with exact minimization
(Algorithm 2 a.k.a. EADMM), described in Section~\ref{sec:algorithm}. For both
ADMM and EADMM, we choose a starting iterate (random $z_0$ and $w_0=G(z_0)$) and initial
dual variable $\lambda_0=0$ (for GD we choose the same $z_0$ as initial
iterate).. We carefully track the objective function value vs.
computation time for a fair comparison.


\textbf{Compressive sensing} The exact minimization step of EADMM  involves the
solution of a system of linear equations in each iteration. Performing Singular
Value Decomposition (SVD) once on the measurement matrix $A$, and storing its
components in memory, allows us to solve such linear systems with a very low
per-iteration complexity (see Supplementary~\ref{subsec:fast_exact}). We plot
the objective function value as well as the reconstruction error with $50\%$
relative measurements in Figure \ref{fig:reconst}(average over 20 images
(MNIST) and 10 images (CelebA)).

\begin{figure}[t]
    \centering
    \begin{minipage}{0.24\textwidth}
        \includegraphics[scale=0.5]{\comparisonfolder/mnist392_cs_l2_error.pdf}
    \label{fig:attack_error_time}
    \end{minipage} \hfill
    \begin{minipage}{0.24\textwidth}
        \includegraphics[scale=0.5]{\comparisonfolder/mnist392_cs_meas_error.pdf}
    \label{fig:attack_error_time}
    \end{minipage} \hfill
    \begin{minipage}{0.24\textwidth}
        \includegraphics[scale=0.5]{\comparisonfolder/celeba6144_cs_l2_error.pdf}
    \label{fig:attack_error_time}
    \end{minipage} \hfill
    \begin{minipage}{0.24\textwidth}
    \centering
        \includegraphics[scale=0.5]{\comparisonfolder/celeba6144_cs_meas_error.pdf}
    \label{fig:linf_comparison}
    \end{minipage}
    \caption{Reconstruction error and measurement error vs time. MNIST (left) and CelebA (right)}
    \label{fig:reconst}
\end{figure}

\textbf{Adversarial Denoising with $\ell_\infty$-norm}
\label{exp:ellinf}
Projection onto the range of a deep-net prior has been considered
by~\cite{Samangouei2018, Ilyas2017} as a defense mechanism against adversarial
examples~\citep{Szegedy2013}. In their settings, samples are denoised with a
generative prior, before being fed to a classifier. Even though the adversarial noise
introduced is typically bounded in $\ell_\infty$-norm, the projection is done
in $\ell_2$-norm. Such projection corresponds to $F(w,z)=\|w-w^\natural\|^2$
in~\eqref{eq:emp loss min}. We instead propose to project using the
$\ell_\infty$-norm that bounds the adversarial perturbation. To this end we
let $F(w, z) = \gamma\|w-w^\natural\|_2^2 + \|w-w^\natural\|_\infty$ in the
template~\eqref{eq:emp loss min}, for some small value of $\gamma$.
The proximal of the $\ell_\infty$ norm is efficiently
computable~\citep{Duchi2008}, allowing us to split $F(w, z)$ in its components
$L(w)=\gamma \|w-w^\natural\|_2^2$ and $R(w)=\|w-w^\natural\|_\infty$ (Note
that the small $\gamma$ ensures that Assumption~\ref{assump:risk} holds)
\input{figures_tex/attacks_performance.tex}

We compare the ADAM optimizer \citep{Kingma2014},
GD and ADMM (450 iterations and for GD and ADAM, and 300 iterations for
EADMM). We use ADAM to solve the $\ell_2$ projection, while ADMM solves
the $\ell_\infty$ projection. We evaluate on a test set of 2000 adversarial
examples from the MNIST dataset, obtained with the Projected Gradient Algorithm
of \cite{Madry2018} with 30 iterations, stepsize 0.01 and attack size 0.2. For
the classifier, we use a standard convolutional network trained on clean MNIST
samples. We also test ADAM, GD (3000 iterations) and EADMM (2000 iterations)
on the $\ell_\infty$ denoising task.

The test error as a function of computation time is
in Figure~\ref{fig:attack_error_time}. We observe that the
$\ell_\infty$ denoising performs better when faced with $\ell_\infty$ bounded
attacks, in the sense that it achieves a lower error with less computation
time. In Figure~\ref{fig:linf_comparison}, we plot the $\ell_\infty$
reconstruction error achieved by ADAM, GD and EADMM, averaged over 7 images. GD
was unable to decrease the initial error, while ADAM takes a considerable
number of iterations to do so. In contrast, our ADMM already achieves the final
error of ADAM within its first 100 iterations.

%\subsection{$\ell_1$ Denoising}
%\label{exp:ell1}
%Given a noisy observation of an unknown signal $w^\n + \eta$, where $\eta$ is
%some random noise, one may attempt to recover $w^\n$ by projecting the noisy
%image back onto the prior. The projection via in $\ell_2$ norm often yields
%good results~\citep{Tripathi2018}. We instead consider denoising in $\ell_1$
%norm by solving the program 
%\begin{align}
%\label{ex:denoising}
%\begin{array}{lll}
%    \underset{w, z}{\text{minimize}} & & \norm{w^\n + \eta - w}_1 \\
%\text{subject to } && w=G(z).
%\end{array}
%\end{align}
%which might be motivated, for example, as being more robust to outliers
%\citep{Zhao2017}.  This is a special case of Program~\eqref{eq:emp loss min},
%where $L_m(w)=0$, $R(w)=\norm{w^\n + \eta - w}_1$ and $H(z)=0$. Note also that
%the proximal operator for $R(w)$  above is inexpensive (soft-thresholding). 
%
%\input{figures_tex/denoising_image_comparison.tex}
%%\input{figures_tex/denoising_performance.tex}
%
%\textbf{Experimental setup. }
%We generate an image $w^\n=G(z^\n)$ and  add Gaussian noise with
%standard deviation values of 0.3 and 0.5, clipping the resulting
%values to the pixel value range $[-1,1]$. We then run EADMM along GD for a fixed
%computational budget.
%
%\textbf{Results and discussion. }
%For the CelebA dataset, the $\ell_1$ measurement and reconstruction error per
%iteration are shown in Figure~\ref{fig:celeba_denoising}. Denoised images are
%shown in Figure~\ref{fig:celeba_denoised}. We observe that our algorithm
%consistently recovers the true signal faithfully and faster, while GD might
%still present some artifacts and require more time to obtain a similar result.
%We should note that, due to the non-smoothness of the objective function in
%Program~\eqref{ex:denoising}, GD uses sub-gradients, which exhibits slow
%convergence.


==> neurips2019 copy/sections/fast_exact.tex <==
\subsection{Per-Iteration Computational Complexity}
\label{subsec:comp_complexity}

The gradient of the function
\begin{equation}
    h(z) = \dfrac{1}{2} \norm{AG(z) - b}_2^2
\end{equation}
follows the formula
\begin{equation}
    \grad h(z) = \grad G(z) A^\top (AG(z) - b)
\end{equation}
which involves one forward pass through the network $G$, in order to compute $G(z)$,
as well as one backward pass to compute $\grad G(z)$, and finally matrix-vector
products to compute the final result.

On the other hand our ADMM first computes the iterate $z_{t+1}$ with
gradient descent on
the augmented lagrangian \eqref{eq:defn_aug_lagr}
 as \begin{equation}
    z_{t+1} = z_t - \beta \grad_z \Lagr_\rho(w_t, z_t, \lambda_t) = - \grad G(z_t)
    \lambda_t^\top - \rho \nabla G(z_t)(w_t-G(z_t))^\top
\end{equation}
which involves one forward and one backward pass on the network $G$, as well as matrix-vector
products. Then we perform the exact minimization procedure on the $w$ variable, 
%, as
%described in \ref{subsec:fast_exact}, 
 which requires recomputing $G(z)$ on the new iterate
$z_{t+1}$, involving one forward pass through the network, as well as the matrix-vector
operations as described before. Recomputing the quantity $w_{t+1} - G(z_{t+1})$ is immediate
upon which the dual stepsize $\sigma_{t+1}$ can be computed at negligible cost. Finally the
dual variable update reads as
\begin{equation}
    \lambda_{t+1} = \lambda_t + \sigma (w_{t+1} - G(z_{t+1}))
\end{equation}
which involves only scalar products and vector additions of values already computed.
All in all each GD iteration involves one forward and one backward pass, while
ADMM computes two forward and one backward pass. Both algorithms require a few
additional matrix-vector operations of similar complexity. For networks with
multiple large layers, as usually encountered in practice, the complexity per
iteration can then be estimated as the number of forward and backward passes,
which are of similar complexity.

\subsection{Parameter Tuning}
\label{subsec:alg_parameters}
We run a grid search for the gradient descent (GD) algorithm
In order to do so we fix a number of
iterations and compare the average objective function over a batch of 100
random images and choose the best performing parameters. We repeat
the tuning in all possible escenarios in the experiments. The results
figures \ref{fig:gd_tuning_mnist} - \ref{fig:gd_tuning_celeba} (GD,
Compressive sensing setup).

\begin{figure}[h]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[scale=0.4]{figures/param_tuning/mnist_156_gd.pdf}
    \end{minipage} \qquad
    \begin{minipage}{0.4\textwidth}
    \centering
        \includegraphics[scale=0.4]{figures/param_tuning/mnist_313_gd_simba.pdf}
    \end{minipage}
\caption{Performance of GD on the compressive sensing task for different
    step sizes. MNIST dataset. 156 (top) and 313 (bottom) linear measurements.}
\label{fig:gd_tuning_mnist}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[scale=0.4]{figures/param_tuning/celeba_2457_gd_glcloud.pdf}
    \end{minipage} \qquad
    \begin{minipage}{0.4\textwidth}
    \centering
        \includegraphics[scale=0.4]{figures/param_tuning/celeba_4915_gd_gcloud.pdf}
    \end{minipage}
\caption{Performance of GD on the compressive sensing task for different
    step sizes. CelebA dataset. 2457 (top) and 4915 (bottom) linear measurements.}
\label{fig:gd_tuning_celeba}
\end{figure}



\subsection{Fast Exact Augmented Lagrangian Minimization with Respect to Primal Variable $w$}
\label{subsec:fast_exact}
In the compressive sensing setup, the augmented lagrangian takes the form
\begin{equation}
    \label{eq:auglagr_appendix}
    \Lagr_\rho(w, z, \lambda) := \dfrac{1}{2} \norm{Aw-b}_2^2 + \langle \lambda, w-G(z)\rangle 
    +\dfrac{\rho}{2} \norm{w-G(z)}_2^2
\end{equation}
with respect to $w$, this is a strongly convex function which admits a unique minimizer
given by the first order optimality condition
\begin{equation}
    \grad_w \Lagr_\rho(w, z, \lambda) = A^\top(Aw-b)+\lambda + \rho(w-G(z))=0
\end{equation}
with solution
\begin{equation}
    w^* = (A^\top A + \rho I)^{-1}(-\lambda +G(z) +A^\top b)
\end{equation}
Given the SVD of $A=USV^\top $ we have $A^\top A=VDV^\top$, where $D$ corresponds to
the diagonal matrix with the eigenvalues of $A^TA$. We then have that
$A^\top A + \rho I=V(D + \rho I)V^\top$ so that
\begin{equation}
    w^* = V(D + \rho I)V^\top(-\lambda + G(z) + A^\top b)
\end{equation}
which involves only a fixed number of matrix-vector products per-iteration.


==> neurips2019 copy/sections/guarantees1.tex <==
Let us study the theoretical guarantees of Algorithm \ref{alg:admm} for
solving program \eqref{eq:emp loss min}, whose constraints are nonlinear and non-convex (since $G$ is specified by a neural network). The main contribution of this section is Theorem \ref{thm:main}, which is
inherently an optimization result stating that Algorithm \ref{alg:admm}
succeeds under certain assumptions on 
\eqref{eq:emp loss min}. 

From an optimization perspective, to our knowledge, Theorem \ref{thm:main} is the first to provide (fast) rates for non-convex and linearized ADMM, see Section \ref{sec:related_works} for a detailed literature review. The  assumptions   imposed below on $L$ and
the generator $G$ ensure the success of Algorithm \ref{alg:admm} and are shortly justified for our setup, where $G$ is a generator network.
\begin{assumption}
\textbf{\emph{strong convexity / smoothness of $L$:}}
\label{assump:risk}
We assume that $L$ in (\ref{eq:emp loss min}) is both strongly convex and
smooth, namely, there exist $0<\mu_L\le \nu_L$ such that
%the population risk $L$ defined as
%\begin{equation}
%    \label{eq:poploss}
%L(w) := \E_{x \sim \chi} l(w,x),
%\end{equation}
%\end{comment}
\begin{align}
\frac{\mu_L}{2} \| w-w'\|^2&  \le L(w') - L(w) - \langle w'-w,\nabla L(w) \rangle  \le \frac{\nu_L}{2} \| w-w'\|^2,
\quad \forall w, w'\in \R^d.
\label{eq:L_str_cvx}
\end{align}
\end{assumption}
Assumption~\ref{assump:risk} is necessary to establish fast rates for Algorithm~\ref{alg:admm}, %, which is arguably the most important regime in practice. 
 and is readily met for
$L(w)=\|{  w-\widehat{w}}\|_2^2$ with $\mu_L = \nu_L = 1$, which renders Algorithm~\ref{alg:admm} applicable to $\ell_2$-denoising with generative prior  in~\citep{Tripathi2018,Samangouei2018,Ilyas2017}.  Here, $\widehat{w}$ is the noisy image.
%Loosely speaking, Assumption \ref{assump:risk} guides Algorithm~\ref{alg:admm} to reach the solution of problem~\eqref{eq:emp loss min}. 
%Recalling the setup in Section \ref{sec:introduction}, we observe that Assumption \ref{assump:risk} evidently holds for DARN with $\ell_2$, where $L(w)=\frac{1}{2}\| w^\natural - w\|_2^2$ and, consequently, $\mu_L = \nu_L = 1$.  

In Supplementary \ref{sec:statLearn}, we also relax the strong
convexity/smoothness in Assumption \ref{assump:risk} to \emph{restricted}
strong convexity/smoothness, which enables us to apply Theorem \ref{thm:main}
in the context of statistical learning with a generative prior, for example in
compressive sensing~\citep{Bora2017}.  Under Assumption~\ref{assump:risk}, even
though $L$ and consequently the objective function of \eqref{eq:emp loss min}
are strongly convex, problem \eqref{eq:emp loss min} might \emph{not} have a
unique solution, which is in stark contrast with convex optimization. Indeed, a
simple example is minimizing $x^2+y^2$ with the constraint $x^2+y^2=1$. We
next state our assumptions on the generator $G$.
%\begin{comment}
%Assumptions~\ref{assump:props_of_l} and \ref{assump:risk}
% are standard in statistical learning~\cite{mohri2018foundations}. For example, in linear regression, we might take
% \[
% l(w,x)= \frac{1}{2}|\langle w-w^\n,x \rangle|^2,
% \]
% \[
% L_m(w) = \frac{1}{2m} \sum_{i=1}^m |\langle w-w^\n,x_i \rangle|^2,
% \]
%for which both Assumptions \ref{assump:props_of_l} and \ref{assump:risk} are met.
%\end{comment}
\begin{assumption}
\label{assump:G_ssmth}
\textbf{\emph{Strong smoothness of $G$:}}
Let $DG$ be the Jacobian of $G$. We assume that $G:\R^s \to \R^d$ is strongly
    smooth, namely, there exists $\nu_G \ge 0$ such that 
\begin{align}
 \| G(z') - G(z) - DG(z)\cdot  (z'-z) \|_2 \le \frac{\nu_G}{2} \|z'-z\|_2^2,
 \qquad \forall z,z'\in \R^s,
\end{align}
\end{assumption}

\begin{assumption}
\label{defn:G_iso}
\textbf{\emph{Near-isometry of $G$:}}
We assume that the generative prior $G$ is a near-isometric map, namely, there exist
$0 <\iota_G\le \kappa_G$  such that 
\begin{align}
\iota_G \|z' - z\|_2  \le  \|G(z') - G(z)\|_2
\le  \kappa_G \|z' - z\|_2 ,
\qquad \forall z,z'\in \R^s.
\label{eq:lipsG}
\end{align}
\end{assumption}

The invertibility of  certain GAN architechtures have been established before
in \citep{ma2018invertibility,hand2017global}.  More concretely, Assumptions
\ref{assump:G_ssmth} and \ref{defn:G_iso} hold for a broad class of generators,
as summarized in Proposition \ref{pr:G-assumptions} and proved in Supplementary
\ref{sec:proposition}.

\begin{proposition}
\label{pr:G-assumptions}
Let $G_\Xi:\Dom \subset \R^d
\to \R^s$ be a feedforward neural network with weights $\Xi \in \R^h$, $k$
layers, non-decreasing layer sizes $s \leq s_1 \leq \ldots s_k \leq d$, with 
$\omega_i$ as activation function in the $i$-th layer, and compact domain
$\Dom$. For every layer $i$, suppose that the activation $\omega_i:\R \to \R$ is of class $C^1$ (continuously-differentiable)  and strictly increasing. 
%Let $G_\Xi:\Dom \subset \R^d
%\to \R^s$ be a feedforward neural network with parameters $\Xi \in \R^h$, $L$
%layers, non-decreasing layer sizes $s \leq s_1 \leq \ldots s_k \leq d$,
%$\omega_i$ as activation function in the $i$-th layer and compact domain
%$\Dom$. 
Then, after an arbitrarily small perturbation to the weights $\Xi$, Assumptions \ref{assump:G_ssmth} and \ref{defn:G_iso} hold 
almost surely  with respect to the Lebesgue measure.
\end{proposition}

A few comments about the preceding result are in order.

\textbf{Choice of the activation function: } Strictly-increasing $C^1$
activation functions in Proposition \ref{pr:G-assumptions}, such as the
Exponential Linear Unit (ELU) \citep{clevert2015fast} or
softplus \citep{Dugas2000}, achieve similar or better performance compared to the commonly-used (but
non-smooth) Rectified Linear Activation Unit (ReLU)~\citep{Xu2015,clevert2015fast,gulrajani2017improved,Kumar2017,kim2018memorization}.
%Even whet In the context of GANs,
%\citet{gulrajani2017improved} reports unsuccesful training with ELUs but
%succeeds at training with other $C^1$ and increasing  activation functions like softplus. 
%\edita{<--- not a good thing to say.}
%On the other hand, training GANs with ELUs has been succesful in
%\citep{Kumar2017} and \citep{kim2018memorization}. 
In our experiments in Section \ref{sec:experiments}, we found that using ELU
activations for the generator $G$ does not  
%noticeable 
adversely effect the representation power of the trained generator. Lastly,
the activation function for the final layer of the generator is typically
chosen as the sigmoid or tanh~\citep{Radford2015}, for which the conditions in
Proposition \ref{pr:G-assumptions} are also met.

\textbf{Compact domain: } The compactness
requirement in Proposition \ref{pr:G-assumptions} is mild.  Indeed, even though the
Gaussian distribution is the default choice as the input for the generator in a GAN,
training has also been successful using compactly-supported distributions,
such as the uniform distribution~\citep{Lipton2017}. Interestingly, even after
training with Gaussian noise, limiting the resulting generator to a
truncated Gaussian distribution can in fact boost the performance of GAN~\citep{brock2018large}, as measured with common metrics like the Inception
Score~\citep{Salimans2016} or
Frechet Inception Distance~\citep{Heusel2017}. This evidence suggests that
obtaining a good generator $G$ with compact domain is straightforward. In the
experiments of Section~\ref{sec:experiments}, we use truncated Gaussian on an Euclidean ball centered at the origin.
%the
%disk $\norm{z}_2 \leq r$ for some large $r > 0$.

\textbf{Non-decreasing layer sizes:} This is a standard feature of popular generator
architectures such as the DCGAN \citep{Radford2015} or infoGAN
\citep{Chen2016}. This property is also exploited in the analysis of the optimization
landscape of problem \eqref{eq:emp loss min} by \cite{hand2017global,Heckel2019}
and for showing invertiblity of (de)convolutional generators
\citep{ma2018invertibility}.

\paragraph{Necessity of assumptions on $G$:} Assumptions \ref{assump:G_ssmth}
and \ref{defn:G_iso} on the generator $G$ are necessary for the provable success of
Algorithm \ref{alg:admm}. Loosely speaking, Assumption \ref{assump:G_ssmth}
controls the curvature of the generative prior, without which the dual
iterations can oscillate without improving the objective. 

On the
other hand, the lower bound in \eqref{eq:lipsG} means that the generative prior
$G$ must be \emph{stably} injective: Faraway latent parameters should be mapped
to faraway outputs under $G$. As a pathological example, consider the
parametrization of a circle as $\{(\sin z,\cos z):z \in [0,2\pi)\}$.

This stable injectivity property in \eqref{eq:lipsG} is necessary for the
success of Algorithm \ref{alg:admm} and is not an artifact of our proof
techniques. Indeed, without this condition, the $z$ updates in Algorithm
\ref{alg:admm} might not reduce the feasibility gap $\norm{w-G(z)}_2$. Geometric assumptions on nonlinear
constraints have precedent in the optimization literature
\citep{birgin2016evaluation,flores2012complete,cartis2018optimality} and to a lesser extent in the literature of neural networks too
\citep{hand2017global,ma2018invertibility}, which we further discuss in Section
\ref{sec:related_works}.

Having stated and justified our assumptions on $L$ and the generator $G$ in
\eqref{eq:emp loss min}, we are now prepared to present the main technical
result of this section. Theorem \ref{thm:main} states that Algorithm
\ref{alg:admm} converges linearly to a small neighborhood of a solution, see
Supplementary \ref{sec:theory} for the proof. 

\begin{theorem}
\label{thm:main}
\textbf{\emph{(guarantees for Algorithm \ref{alg:admm})}}
Suppose that Assumptions~\ref{assump:risk}-\ref{defn:G_iso} hold. 
\begin{comment}
and $L_m$
satisfies the restricted strong convexity and smoothness in
Definition~\ref{defn:Lm_scvx} for a set $W\subset \R^p$ that contains a
solution $w^*$ of Program (\ref{eq:emp loss min}) and all the iterates
$\{w_t\}_{t\ge 0}$ of Algorithm \ref{alg:admm}.\footnote{If necessary, the inclusion
$\{w_t\}_{t\ge 0}\subset W$ might be enforced by adding the indicator function
of the convex hull of $W$ to $R$ in Program \eqref{eq:emp loss min}, similar
to \cite{agarwal2010fast}.}
\end{comment}
Let $(w^*,z^*)$ be a solution of program (\ref{eq:emp loss min}) and let $\lambda^*$ be a corresponding optimal dual variable.  Let also
$\{w_t,z_t,\lambda_t\}_{t\ge 0}$ denote the output sequence of
Algorithm~\ref{alg:admm}. 
Suppose that the primal step sizes $\a,\b$  satisfy
\begin{align}
\a  \le  \frac{1}{\nu_\rho},
%\widetilde{\alpha},%(\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
\qquad
\b \le \frac{1}{\xi_\rho + 2\a\tau_\rho^2}.
%\frac{\xi_\rho}{2}+\a \tau_\rho^2 \le \frac{1}{2\b}, 
%\widetilde{\beta},%(\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,%\lambda_0),
%,(\a,\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
\qquad \s_0 \le \s_{0,\rho}.
\label{eq:step_size_reqs_thm}
\end{align}
Then  it holds that
\begin{align}
\frac{\|w_t-\wh{w}\|_2^2}{\a}+\frac{\|z_t-\wh{z}\|_2^2}{\b} \le 2(1-\eta_{\rho})^t \Delta_{0} +
\frac{\ol{\eta}_\rho}{\rho},
\label{eq:linr_cvg_thm}
\end{align}
\begin{align}
\label{eq:feas-thm}
\|w_t - G(z_t)\|_2^2 \le 
\frac{4(1-\eta_\rho)^t\Delta_0}{\rho}+ \frac{\widetilde{\eta}_\rho}{\rho^2}
,
\end{align}
for every iteration $t$. Above, $\Delta_0 = \mathcal{L}_\rho(w_0,z_0,\lambda_0)- \mathcal{L}_\rho(w^*,z^*,\lambda^*)$ is the initialization error, see~(\ref{eq:defn_aug_lagr}).
The convergence rate $ 1-\eta_\rho\in (0,1)$ and the quantities  $\nu_\rho,\xi_\rho,\tau_\rho,\s_{0,\rho},\ol{\eta}_\rho,\widetilde{\eta}_\rho$ above depend on the parameters in  Assumptions \ref{assump:risk}-\ref{defn:G_iso} and on $\lambda^*$,  as  specified in  the proof. As an example,  in the regime where $\mu_L \gg \rho$ and $\iota_G^2 \gg \nu_G$, we can take 
\begin{align*}
\a \approx \frac{1}{\nu_L}, \qquad \b\approx \frac{1}{\rho \kappa_G^2},
\qquad \frac{\rho \nu_G}{\kappa_G^2}\lesssim\s_0 \lesssim \rho\min \l(\frac{\mu_L^2}{\nu_L^2},\frac{\iota_G^4}{\kappa_G^4}\r),
\end{align*}
\begin{align}
\eta_\rho \approx \min\l(\frac{\mu_L}{\nu_L}, \frac{\iota_G^2}{\kappa_G^2}  \r),
\qquad 
\ol{\eta}_\rho \approx \widetilde{\eta}_\rho \approx  \max\l(\frac{\nu_L}{\mu_L}, \frac{\kappa_G^2}{\iota_G^2}  \r).
\label{eq:step-sizes-example}
\end{align}
Above, for the sake of clarity,   $\approx$ and $\lesssim$   suppress the universal constants, dependence on the initial dual  $\lambda_0$ and the corresponding step size $\s_0$. 
%Note that, in this regime, $\eta_\rho,\ol{\eta}_\rho,\widetilde{\eta}_\rho$ are nearly independent of $\rho$.
\end{theorem}
A few clarifying comments about Theorem \ref{thm:main} are in order. 

\textbf{Error:} According to Theorem \ref{thm:main}, if the primal and dual
step sizes are sufficiently small and Assumptions
\ref{assump:risk}-\ref{defn:G_iso} are met,  Algorithm \ref{alg:admm} converges
linearly to a \emph{neighborhood} of a solution $(w^*,z^*)$. The size of this
neighborhood depends on the penalty weight $\rho$ in \eqref{eq:defn_aug_lagr}.
For instance, in the example in Theorem~\ref{thm:main}, it is easy to verify that this neighborhood has a
radius of $O(1/\rho)$, which can be made smaller by increasing $\rho$. Theorem~\ref{thm:main} is however silent about
the behavior of Algorithm \ref{alg:admm} within this neighborhood. This is
to be expected. Indeed, even in the simpler convex case, where $G$ in program~\eqref{eq:emp loss min} would  have been an affine map, provably no first-order
algorithm could converge linearly to the solution
\citep{ouyang2018lower,agarwal2010fast}. 

Investigating the behavior of Algorithm \ref{alg:admm} within this
neighborhood, while interesting, arguably has  little practical value. For
example, in the convex case, ADMM would converge  slowly (sublinearly) in this neighborhood, which does not appeal to the practitioners.  As another example, when Algorithm~\ref{alg:admm} is applied in the context of statistical learning, there is no
benefit in solving~\eqref{eq:emp loss min} beyond the statistical accuracy of
the problem at hand \citep{agarwal2010fast}, see the discussion in Supplementary~\ref{sec:gen-err}. As such, we defer the study of the
local behavior of Algorithm \ref{alg:admm} to a future work. 

\textbf{Feasibility gap:} Likewise, according to \eqref{eq:feas-thm} in
Theorem \ref{thm:main}, the feasibility gap of Algorithm \ref{alg:admm} rapidly
reaches a plateau. In the example in Theorem \ref{thm:main}, the feasibility
gap rapidly reaches $O(1/\rho)$, where $\rho$ is the penalty weight in \eqref{eq:defn_aug_lagr}. As before, even in the convex case, no first-order algorithm could
achieve exact feasibility at linear rate~\citep{ouyang2018lower,agarwal2010fast}. 
%Understanding the sublinear local
%behavior of Algorithm \ref{alg:admm}, while interesting, is arguably of little
%practical interest and thus deferred to a future work. 
%\marginnote{\editf{it
%seems that the little practical interest argument is repeated here and in te
%preceding paragraph}} \marginnote{\textbf{\edita{what other aspects of theorem should we discuss? what did the reviewers pointed out?}}} 

\textbf{Intution:} While the exact expressions for the quantities in Theorem
\ref{thm:main} are given in Supplementary~\ref{sec:theory}, the example
provided in Theorem~\ref{thm:main} highlights the simple but instructive regime
where $\mu_L \gg \rho$ and $\iota_G^2 \gg \nu_G$, see Assumptions
\ref{assump:risk}-\ref{defn:G_iso}. 
Intuitively, $\mu_L \gg \rho$ means that minimizing the objective of~\eqref{eq:emp loss min} is prioritized over reducing the feasibility gap, see
\eqref{eq:defn_aug_lagr}. In addition,  $\iota_G^2 \gg \nu_G$ suggests that the
generative prior $G$ is very smooth. 

In this regime, the primal step size $\a$ for $w$ updates
is determined by how smooth $L$ is, and the primal step size $\b$ in the
latent variable $z$ is determined  by how smooth $G$ is, see
\eqref{eq:step-sizes-example}. Similar restrictions are standard in first-order
algorithms to avoid oscillations  \citep{nesterov2013introductory}. 
 
As discussed earlier, the algorithm rapidly reaches a neighborhood of size
$O(1/{\rho})$ of a solution and the feasibility gap plateaus at
$O(1/\rho)$. Note the  trade-off here for the choice of $\rho$: the larger the
penalty weight $\rho$ is, the more accurate Algorithm \ref{alg:admm} would be
and yet increasing $\rho$ is restricted by the assumption $\rho\ll \mu_L$.
Moreover, in this example, the rate $1-\eta_\rho$ of Algorithm~\ref{alg:admm}
depends only on the regularity of $L$ and $G$ in program \eqref{eq:emp loss
min}, see \eqref{eq:step-sizes-example}. Indeed, the more well-conditioned $L$
is and the more near-isometric $G$ is, the larger $\eta_\rho$ and the faster
the convergence would be.  

Generally speaking, increasing the penalty weight $\rho$ reduces the bias of Algorithm \ref{alg:admm} at the cost of a slower rate. 
Beyond our work, such dependence on the geometry of
the constraints has precedent in the literature of
optimization~\citep{birgin2016evaluation,flores2012complete,cartis2018optimality}
and manifold embedding theory~\citep{eftekhari2015new,eftekhari2017happens}. 

{\paragraph{Relation to simple gradient descent:} %, the variant of Algorithm \ref{alg:admm} introduced in Section \ref{sec:algorithm}, 
Consider a variant of Algorithm~\ref{alg:admm} that replaces the linearized
update for $w$ in \eqref{eq:aug lagr alg} with exact minimization with respect
to $w$, which can be achieved with an off-the-shelf convex solver or might have
a closed-form solution in some cases. The exact minimization over $w$ and
Lemma~\ref{lem:str cvx} together guarantee that Theorem~\ref{thm:main} also
applies to this variant of Algorithm~1. 

Moreover, as a special case of \eqref{eq:emp loss min} where $R\equiv 0$ and
$H\equiv 0$, this variant is closely related to GD~\citep{Bora2017}, presented
there without any rates. In Appendix~\ref{sec:gd-admm},  we establish that the
updates of both algorithms match as the feasibility gap vanishes. In this
sense, Theorem \ref{thm:main} provides the first rates for GD, albeit limited
to the limit case of vanishing feasibility gap. Indeed, one key advantage of
the primal-dual formulation studied in this paper is exactly this versatility
in providing a family of algorithms, such as Algorithms \ref{alg:admm} and 2,
that can be tuned for various scenarios and can also efficiently handle the
non-smooth case where $R$ or $H$ are nonzero in~\eqref{eq:emp loss min}. } 

%\paragraph{Algorithm 2.} Even though Theorem \ref{thm:main} is about Algorithm \ref{alg:admm}, as a corollary we see that Algorithm~2 in Section \ref{sec:algorithm} also has linear rates as long as the primal and dual step sizes in each outer iteration of Algorithm~2 satisfy the conditions in Theorem~\ref{thm:main}. In particular, if the example regime in Theorem \ref{thm:main} is applicable, the convergence rate remains the same across outer iterations at $1-\min(\mu_L/\nu_L, \iota_G^2/\kappa_G^2)$. 


%However,
%Assumption~\ref{assump:risk} does not hold when $L(w) = \|{w^\natural -
%w}\|_\infty$ for $\alpha=1$ or $\infty$. That is, Theorem \ref{thm:main} below
%does not directly apply to, for example, adversarial denoising. Nevertheless,
%the  flexibility of our template $\eqref{eq:emp loss min}$
%allows us to still approximately solve such problems by taking
%$L(w)=\frac{\gamma}{2}\|{w^\natural - w}\|_2^2$ and $R(w)=\|{w^\natural -
%w}\|_\alpha$ for a small $\gamma\ge 0$.
%%, and noting that the proximal operator of
%%$R$ can be efficiently computed when $\alpha=1$ or $\infty$. 
%The resulting guarantees by Theorem \ref{thm:main} degrade gracefully as
%$\gamma$ tends to zero. The derivation of sublinear rates for the particular
%case of $\g=0$ is left for a future work.



%More specifically, Theorem \ref{thm:main} identifies the key attributes of $L$ and the generator $G$  required for the success of Algorithm
%\ref{alg:admm}. 
%Due to its optimization nature, Theorem \ref{thm:main} might
%also be of independent interest in other applications of program
%\ref{eq:emp loss min}, such as statistical learning with nonlinear prior, see
%Sections~\ref{sec:introduction}~and~\ref{sec:related_works}.  

%\begin{comment}
%As detailed in Supplementary
%\ref{sec:relations}, our result includes as a special case the
%convergence rate of the algorithm proposed in \citep{Bora2017} without
%convergence analysis. Our characterizations are based on the precise adaptive update rules on the penalty parameters, as described in Section 2. 
%
%Our strategy is to pinpoint 
%To the best of our knowledge, in the context of learning
%with deep-net priors, the only existing convergence rate appears in
%\cite{Shah2018, Hegde2018} for the special case of linear regression and relies on a
%projection oracle onto a non-convex set. Establishing the accuracy of the
%numerical approach used in \cite{Shah2018, Hegde2018} in lieu of this oracle is
%an open question and arguably a daunting task in itself. In this sense,
%Theorem \ref{thm:main} below provides the first convergence rate for solving
%Program \eqref{eq:emp loss min} and its equivalent formulations. We defer a
%detailed review of the literature to Section \ref{sec:related_works} and turn
%to the technical details now.
%\end{comment}

%\begin{comment}
%Our main theoretical result in this paper, Theorem
%\ref{thm:main} below, establishes the linear convergence of Algorithm~\ref{alg:admm}
%to a neighborhood of solutions $(w^*,z^*)$ under certain technical assumptions,
%described below.
%\begin{assumption}
%\label{assump:props_of_l}
%\textbf{\emph{(Convexity / strong smoothness of loss) }}
%We assume that $\lossf(\cdot, \cdot)$ is convex in both of its arguments.
%Moreover, we assume that $\lossf(w, \cdot)$ is strongly smooth, namely, there
%exists $\s_\lossf \ge 0$ such that for every $x,x'\in \mathbb{X}$
%\begin{align}
%    \D_\lossf(x,x';w) \le \dfrac{\s_\lossf}{2}\norm{x-x'}_2^2,
%\label{eq:props_of_l}
%\end{align}
%where $\D_\lossf$ stands for the \emph{Bregman divergence} associated with $l(w,\cdot)$,
%\begin{align*}
%\D_l(x,x';w) = l(w,x') - l(w,x) - \langle x'-x, \nabla_x l(w,x) \rangle .
%\end{align*}
%\end{assumption}
%\end{comment}

%\begin{comment}
%On the other hand, the Lipschitz-continuity of
%$DG$ can be enforced, for example, by bounding the input of $G$, namely, by
%enforcing $\|z\|_2<M$ via the regularizer $H$ in program \eqref{eq:emp loss min}.
%\end{comment}
%
%For $G$ to satisfy the upper bound in \eqref{eq:lipsG}, it needs to be Lipschitz
%continuous, which holds for architectures with Lipschitz continuous activation
%functions, as is the case with the most common choices, see Section \ref{sec:experiments}. Moreover, the
%Lipschitz constant of $G$ can be controlled by regularizing the network
%\citep{raghunathan2018certified,tsuzuku2018lipschitz,yang2018diversity}.

%\begin{comment}
%As a consequence of Assumption \ref{assump:props_of_l}, we have that $L_m$ is
%convex. We additionally require $L_m$ to be strongly convex and smooth in the
%following restricted sense. Even though $L_m$ is random because of its
%dependence on the random training data $\{x_i\}_{i=1}^m$, we ensure in
%Section \ref{sec:guarantees2} that the next condition is indeed met with high
%probability when $m$ is large enough.
%\begin{definition}
%\label{defn:Lm_scvx}
%\textbf{\emph{(Restricted strong convexity / smoothness of empirical loss.) }}
%We say that $L_m$ is strongly convex and smooth on the set $W\subset\R^p$ if
%there exist $0<\mu_L\le \nu_L$ and $\ol{\mu}_L,\ol{\nu}_L\ge 0$ such that
%\begin{align}
%\D_{L_m}(w,w') &   \ge \frac{\mu_L}{2}\|w'-w\|_2^2 - \ol{\mu}_L, \nonumber\\
%\D_{L_m}(w,w')
%& \le \frac{\nu_L}{2}\|w'-w\|_2^2 + \ol{\nu}_L,
%\end{align}
%\begin{align*}
%\D_{L_m}(w,w') := L_m(w') - L_m(w) - \langle w' - w, \nabla L_m(w) \rangle,
%\end{align*}
%for every $w,w'\in W$.
%\end{definition}
%\end{comment}


%The main message of Theorem  \ref{thm:main} is simple: The
%optimization error $\|w_t-w^*\|_2$ and the {feasibility gap} $\|w_t - G(z_t)\|_2$
%rapidly reach a floor. Theorem \ref{thm:main} is
%immediately followed by a number of clarifying remarks.
%$\psi_\rho$ and $\mu_\rho \psi_\rho/\rho$ linearly, respectively.
%Here, $\rho$ is the penalty weight of the augmented Lagrangian and the quantities $\psi_\rho$ and $\mu_\rho$ are defined in the proof. 


%Moreover, in the convergence rate $1-\min(\frac{\mu_L}{\nu_L},\frac{\iota_G^2}{\kappa_G^2})$ in Theorem \ref{thm:main}, the  term $1-\frac{\mu_L}{\nu_L} $ is the standard linear
%convergence rate of a $\mu_L$ strongly convex and $\nu_L$ smooth
%function~\cite{nesterov2013introductory}, appearing here by the virtue of Assumption \ref{assump:risk} on $L$.
 

 

% \begin{comment}
% \paragraph{Trade-offs.}
% Even though problems \eqref{eq:emp loss min} and \eqref{eq:aug lagr} are equivalent for every penalty weight $\rho>0$, this parameter in Algorithm \ref{alg:admm} (or any other primal-dual optimization algorithm) balances the objective and feasibility gap. More specifically, if $\rho$ is too small ($\rho \ll \mu_L$), then Algorithm \ref{alg:admm} prioritizes reducing the objective of \eqref{eq:emp loss min} at the cost of possibly larger feasibility gap $\|w_t-G(z_t)\|_2$. In contrast, if the penalty weight $\rho$ is too large $(\rho \gg \nu_L)$, then Algorithm \ref{alg:admm} prioritizes reducing the feasibility gap at the cost of ignoring the objective value. 
% \end{comment}


% \begin{comment}
% \paragraph{Geometry of prior.}
%  At a high level, the more isometric and smooth $G$ is, the faster
%  Algorithm~\ref{alg:admm} would converge to a smaller neighborhood of
%  solutions. That is, smaller $\kappa_G / \iota_G, \nu_G,
%  \ol{\nu}_G,\ol{\iota}_G,\ol{\kappa}_G$ in Assumptions~\ref{assump:G_ssmth} and
%  \ref{defn:G_iso}  means that $G$ is more ``regular'' and this in turn leads to
%  smaller (faster) convergence rate $\eta_\rho$ and  optimization error
%  $\widetilde{\psi}_\rho$ in Theorem~\ref{thm:main}.
%  In other words, the performance of Algorithm~\ref{alg:admm} depends both on
%  the geometry of the ``manifold'' $G(\R^s)\subset \R^p$ and also on how $G$
%  maps different points in the latent space $\R^s$  to different points on
%  $G(\R^s)$. This dependence on the geometry of prior  and its parametrization
%  has precedent in the literature of
%  optimization~\cite{birgin2016evaluation,flores2012complete,cartis2018optimality}
%  and (manifold) embedding theory~\cite{eftekhari2015new,eftekhari2017happens}.
%  Based on this discussion  and in order to gain more insight, the simplified
%  expressions that will follow are derived for the idealistic scenario $\nu_G
%  \ll \iota_G \approx \kappa_G \ll \rho \ll \nu_L \approx \mu_L$, 
%  $\ol{\nu}_G=\ol{\iota}_G = \ol{\kappa}_G = \ol{\nu}_G = \ol{\mu}_L =0$, 
%  $\lambda_0 = 0\in \R^m$, and $\s_0 \approx 0$. 
%  %Our work appears to be the first to rigorously reveal this dependence in the context of learning with generative priors.
%  \end{comment}

% \paragraph{Step sizes.} Lower bounds on the primal step sizes, namely,
% $\widetilde{\alpha},\widetilde{\beta}$ in \eqref{eq:step_size_reqs_thm}, are a
% consequence of the restricted convexity and smoothness assumptions on $L_m$,
% see Definition~\ref{defn:Lm_scvx}. Indeed, such lower bounds have been reported
% before for both convex and nonconvex
% problems~\cite{agarwal2010fast,oymak2018sharp}.

% For step size $\a$ in $w$ variable, roughly speaking, $\a\approx
% \frac{1}{\nu_L}$, where $\nu_L$ quantifies the restricted strong smoothness of
% the empirical loss, see Definition~\ref{defn:Lm_scvx}.
% %See \cite{agarwal2010fast} for a precedent in the convex world.
% While $L_m$ and hence $\nu_L$ are both random because of their dependence on
% the training data, we will establish in Section~\ref{sec:guarantees2} that,
% with high probability, $\nu_L\approx \s_L$ if the number of training points $m$
% is large enough. Here, $\s_L$ is the smoothness parameter of the population
% risk, defined in  Assumption~\ref{assump:risk}.

% For the step size $\b$ in $z$ variable, loosely speaking, $\b \approx
% \frac{1}{2\rho \kappa_G^2}$, where $\kappa_G$ is the Lipschitz constant of $G$,
% see Assumption~\ref{defn:G_iso}.

% \paragraph{Convergence rate.} As specified in the proof,
% \begin{align}
% \eta_\rho \approx 1- \frac{\mu_L}{\nu_L} + \frac{C}{\widetilde{\psi}_\rho^2},
% \end{align}
% for a factor $C$. The  term $1-\frac{\mu_L}{\nu_L} $ is the standard linear
% convergence rate of a $\mu_L$ strongly convex and $\nu_L$ smooth
% function~\cite{nesterov2013introductory}, appearing here by the virtue of the
% assumptions on $L_m$, see Definition~\ref{defn:Lm_scvx}. Note the interesting
% tradeoff present here: Increasing $\widetilde{\psi}_\rho$ reduces $\eta_\rho$.
% That is,  Algorithm~\ref{alg:admm} converges faster to coarser estimates of
% solutions of Program~\eqref{alg:admm}. This  naturally leads us to the next
% remark.

% \paragraph{Optimization error.} Even as $t$ grows, the optimization error of
% Algorithm~\ref{alg:admm} does not vanish. In particular, it follows from
% \eqref{eq:linr_cvg_thm} that
% \begin{align}
% \lim_{t\rightarrow\infty} \|w_t - w^*\|_2^2 & \le \widetilde{\psi}_\rho, 
% \end{align}
% That is, according to Theorem \ref{thm:main}, the iterates $\{w_t,z_t\}_{t\ge
% 0}$ of Algorithm \ref{alg:admm} linearly converge to a neighborhood of
% solutions $(w^*,z^*)$ of Program \eqref{eq:emp loss min}, rather than
% converging to $(w^*,z^*)$ itself.

% Indeed, it is impossible to obtain linear convergence to solutions even for a
% convex but constrained optimization program \cite{ouyang2018lower}. While we
% are not aware of any general impossibility results for nonconvex problems such
% as Program \eqref{eq:emp loss min}, this observation suggests that
% Theorem \ref{thm:main} is sensible.

% Theorem \ref{thm:main} also agrees with earlier results for (convex)
% M-estimators~\cite{agarwal2010fast}. Later in Section \ref{sec:guarantees2},
% when bounding the generalization error, we will also see that this limited
% accuracy of Algorithm \ref{alg:admm} may not be consequential from a
% statistical viewpoint.

% \paragraph{Feasibility gap.} As with the optimization error,
% Algorithm \ref{alg:admm} is unable to reach exact feasibility, analogous to
% what happens for convex but constrained problems~\cite{ouyang2018lower}.
% Indeed, it follows from \eqref{eq:feas-thm} that
% \begin{align}
% \lim_{t\rightarrow\infty} \| w_t - G(z_t) \|_2^2 &  \le \mu_\rho \psi_\rho / \rho.
% \end{align}


==> neurips2019 copy/sections/guarantees2.tex <==

Building upon the results in Section~\ref{sec:guarantees1}, the main result in this section (Theorem~\ref{thm:main_stat}) quantifies the convergence of the iterates $\{w_t\}_{t\ge 0}$ of Algorithm~\ref{alg:admm} to the true parameter $w^\n$. 


In other words, Theorem~\ref{thm:main_stat} below controls the generalization error of Program~\eqref{eq:emp loss min}, namely, the error  incurred by using the empirical risk $L_m$ in lieu of the population risk $L$. Indeed, Theorem~\ref{thm:main} is  silent about $\|w_t - w^\n\|_2$.  We address this shortcoming with the following result, proved in Section~\ref{sec:proof of ws_to_wn} of the supplementary material.  
\begin{lemma}\label{lem:ws_to_wn}
Let $R=1_W$ be the indicator function on $W\subset\R^p$ and set $H=0$ in Program~(\ref{eq:emp loss min}).\footnote{To be complete, $1_W(w)=0$ if $w\in W$ and $1_W(w)=\infty$ otherwise. } Suppose that $w^*$ belongs to the relative interior of $W$. 
%\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ denotes the relative interior of the set $W$.  
Then it holds that 
\begin{align}
\|w^\n - w^*\|_2 \le \frac{1}{\zeta_L} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w) \|_2.
\label{eq:before_Upsilon}
\end{align}
\end{lemma}
Before bounding the right-hand side of \eqref{eq:before_Upsilon}, we remark that it is possible to extend Lemma~\ref{lem:ws_to_wn} to the case where the regularizer $R$ is a \emph{decomposable} norm, along the lines of~\cite{negahban2012unified}. We will however not pursue this direction in the present work. 
Next note that \eqref{eq:linr_cvg_thm} and Lemma~\ref{lem:ws_to_wn} together imply that 
\begin{align}
& \| w_t - w^\n\|_2^2  \nonumber\\
& \le ( \|w_t - w^*\|_2+ \|w^* - w^\n\|_2  )^2 
\qquad \text{(triangle inequality)} \nonumber\\
& \le 2 \|w_t - w^*\|_2^2 + 2 \|w^*-w^\n\|_2^2
\quad ( (a+b)^2 \le 2a^2+2b^2  )
 \nonumber\\
& \le 2\eta_{\rho}^t\widetilde{\Delta}_0 
+ 2\widetilde{\psi}_\rho \nonumber\\
& \qquad 
+ \frac{2}{\zeta_L^2} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w)\|_2^2. 
\label{eq:before_rademacher}
\end{align}
According to Theorem~\ref{thm:main}, the right-hand side of \eqref{eq:before_rademacher} depend on $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$, which were introduced in Definition~\ref{defn:Lm_scvx}, with the exact dependence specified in the proof of the theorem. Note that $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$  and the right-hand side of \eqref{eq:before_Upsilon} are all random variables because they depend on $L_m$ and thus on the randomly drawn training data $\{x_i\}_{i=1}^m$. To address this issue,  we apply a basic result in statistical learning theory as follows. For every $w\in \R^p$ and every pair $x,x'\in \mathbb{X}$, we use Assumption~\ref{assump:props_of_l} to write that 
\begin{align}
\| \nabla l(w,x) - \nabla l(w,x') \|_2 & \le \s_l \| x-x'\|_2
\qquad \text{(see \eqref{eq:props_of_l})} \nonumber\\
& \le \s_l \text{diam}(\mathbb{X}),
\end{align}
where $\text{diam}(\mathbb{X})$ denotes the diameter of the compact set $\mathbb{X}$. Note also that 
\begin{align}
\E_{\{x_i\}_i} \nabla L_m(w) = \nabla L(w), 
\qquad \forall w\in W,
\end{align}
where the expectation is over the training data $\{x_i\}_i$. 
Then, for $\varepsilon>0$ and except with a probability of at most $e^{-\varepsilon}$, it holds that 
\begin{align}
& \| \nabla L_m(w) - \nabla  L(w) \|_2  \nonumber\\
& \le 2 \mathcal{R}_W(x_1,\cdots,x_m) +3\s_l\text{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}} \nonumber\\
& =: \Upsilon_{m,W}(\varepsilon),
\label{eq:emp_proc}
\end{align}
for every $w\in W$~\cite{mohri2018foundations}. Above, 
\begin{align}
& \mathcal{R}_W(x_1,\cdots,x_m) \nonumber\\
& = 
\E_{E} \l[ \max_{w\in W}    \l \| \frac{1}{m} \sum_{i=1}^{m} e_i \nabla_w l(w,x_i)\r \|_2 \r],
\label{eq:emp rademach}
\end{align}
is the \emph{empirical Rademacher complexity} and $E=\{e_i\}_i$ is a Rademacher sequence, namely, a sequence of independent random variables taking $\pm 1$ with equal probabilities.  We can now revisit \eqref{eq:before_rademacher} and write that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le 2\eta_{\rho}^t\widetilde{\Delta}_0  + 
2\widetilde{\psi}_\rho + \frac{2\Upsilon_{m,W}^2(\varepsilon)}{\zeta_L^2},
\end{align}
which holds except with a probability of at most $e^{-\varepsilon}$. In addition, for every $w,w'\in W$, we may write that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \le   \| \nabla L(w) - \nabla L(w')\|_2+ \| \nabla L_m(w) - \nabla L(w) \|_2\nonumber\\
& \qquad  + \| \nabla L_m(w') - \nabla L(w')\|_2
\quad \text{(triangle inequality)} \nonumber\\
& \le  \s_L\|w-w'\|_2+  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx},\ref{eq:emp_proc} ))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. 
Likewise, for every $w,w'\in W$, we have that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \ge \| \nabla L_m(w) - \nabla L_m(w) \|_2  -  \| \nabla L_m(w) - \nabla L(w)\|_2\nonumber\\
& \qquad - \| \nabla L_m(w') - \nabla L(w')\|_2
\qquad \text{(triangle inequality)} \nonumber\\
& \ge  \zeta_L\|w-w'\|_2-  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx},\ref{eq:emp_proc} ))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. Therefore, $L_m$ satisfies the restricted strong convexity and smoothness in Definition~\ref{defn:Lm_scvx} with
\begin{align}
\mu_L = \s_L,
\qquad 
\nu_L = \zeta_L,
\nonumber\\
\ol{\mu}_L = \ol{\zeta}_L =  2\Upsilon_{m,W}(\varepsilon). 
\end{align}
%Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold. These findings are summarized below in our second main result.  For a convex set $W\subset\R^p$, let  $R=1_W$  be the (convex) indicator function on $W$ and set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of Program~(\ref{eq:emp loss min}) satisfies $w^*\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ is the relative interior of the set $W$.  
Our findings in this section are summarized below. 
\begin{theorem} \label{thm:main_stat}\textbf{\emph{(Generalization error)}} 
Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold and recall that the training samples $\{x_i\}_{i=1}^m$ are drawn independently from the probability space $(\mathbb{X},\chi)$ for a compact set $\mathbb{X} \subset \R^d$  with diameter $\operatorname{diam}(\mathbb{X})$.   

For a set $W\subset\R^p$, let  $R=1_W$  be the indicator function on $W$, and set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of Program~(\ref{eq:emp loss min}) belongs to the relative interior of $W$. 
For $\varepsilon>0$, evaluate the quantities in Theorem~\ref{thm:main} with 
\begin{align}
\mu_L & = \s_L,
\qquad 
\nu_L = \zeta_L, \nonumber\\
\ol{\mu}_L & = \ol{\zeta}_L =   
4 \mathcal{R}_W(x_1,\cdots,x_m) \nonumber\\
& \qquad +6\s_l\operatorname{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}},
\end{align}
where $\mathcal{R}_W(x_1,\cdots,x_m)$ in the empirical  Rademacher complexity defined in (\ref{eq:emp loss min}). If the requirements on the step sizes in~(\ref{eq:step_size_reqs_thm}) hold, we then have that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le   2\eta_{\rho}^t\widetilde{\Delta}_0   + 
2\psi_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2  \nonumber\\
& \qquad +  \frac{18\s_l^2 \operatorname{diam}(\mathbb{X})^2( \varepsilon+2)}{m}, 
\end{align}
 except with a probability of at most $e^{-\varepsilon}$. 
\end{theorem}
Most of the remarks about Theorem~\ref{thm:main} also apply to Theorem~\ref{thm:main_stat} and we note that $\|w_t-w^\n\|_2$ reduces by increasing the number of training samples $m$, before asymptotically reaching the generalization error
\begin{align}
2\psi_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2.
\label{eq:statistical ball}
\end{align}
Computing the Rademacher complexity above for specific choices of the network structure and loss is itself potentially a complicated task, which we will not pursue by the virtue of the generality of our results so far. The key technical challenge there is computing the corresponding \emph{entropy integral}, which involves estimating the \emph{covering numbers} of the set $W$ \cite{mohri2018foundations}. One last takeaway point from the statistical accuracy in \eqref{eq:statistical ball} is the following. If  
\begin{align}
\psi_\rho=O(\mathcal{R}_W(x_1,\cdots,x_m)^2/\zeta_L^2),
\label{eq:statistacll ball 2}
\end{align}
the asymptotic optimization error  in Theorem~\ref{thm:main} does not play an important role in determining the generalization error above. In words, i \eqref{eq:statistacll ball 2} holds, then Algorithm~\ref{alg:admm} converges to the ball of statistical accuracy around $w^\n$. Here, $O$ stands for the standard Big-O notation. 





==> neurips2019 copy/sections/guarantees_temp.tex <==
\section{Convergence Rate \label{sec:cvg rate}}

In this section, we investigate the convergence rate of our algorithm for finding first-order and second-order stationary points, along with iteration complexity results.
The proofs are deferred to Appendix~\ref{sec:theory} for clarity of exposition.

\subsection{Complexity results for first-order stationarity}
Theorem~\ref{thm:main} characterizes the convergence rate of Algorithm~\ref{Algo:2} for finding first-order stationary points in terms of the number of outer iterations.\\
{\color{red}{Ahmet: I think that it is possible to remove sufficiently large k0 assumption here. }}
\begin{theorem}
\label{thm:main}
In addition to the smoothness of $f$ and $A$ as in (\ref{eq:smoothness basic}) and for $\rho'>0$, let us define 
\begin{align}
\lambda'_f = \max_{\|x\|\le \rho'} \|\nabla f(x)\|,
~~
\lambda'_A = \max_{\|x\| \le \rho'} \|DA(x)\|,
\end{align}
to be the (restricted) Lipschitz constants of $f$ and $A$, respectively. 
 For sufficiently large integers $k_0\le k_1$, consider the interval $K=[k_0:k_1]$.  Let $\{x_k\}_{k\in K}$ be the output sequence of Algorithm~\ref{Algo:2} and, for $\nu>0$, assume that 
 \begin{align}
\nu \|A(x_k)\|  
& \le \dist\left( -DA(x_k)^\top A(x_k) , \frac{\partial g(x_k)}{ \b_{k-1}}  \right), 
\label{eq:regularity}
\end{align}
for every $k\in K$. 
Then the output of Algorithm~\ref{Algo:2} satisfies 
\begin{align}
& \dist^2( -\nabla_x \L_{\b_{k-1}}(x_k,y_k),\partial g(x_k)) + \| A(x_k)\|^2   \nonumber\\
& = \frac{1}{\b_{k-1}^2}\left( \frac{8 \lambda'_A\s_k^2 + 4}{ \nu^2} ( \lambda'_f+\lambda'_A y_{\max})^2 + 2\right) \nonumber \\ 
&=: \frac{Q}{\beta_{k-1}^2}. 
\end{align}
\end{theorem}
A few remarks are in order about Theorem~\ref{thm:main}. 

\textbf{Tradeoff.}
Roughly speaking, Theorem~\ref{thm:main} states that the iterates of Algorithm~\ref{Algo:2} approach first-order stationarity for~\eqref{prob:01} at the rate of $1/{\b_k}$, where $\b_k$ is the penalty weight in AL in iteration $k$ as in~\eqref{eq:Lagrangian}. Note the inherent tradeoff here: For a faster sequence $\{\b_k\}_k$, the iterates approach stationarity faster but the computational cost of the inexact primal subroutine (Step 2) increases since a higher accuracy is required and Lipschitz constant of the unconstrained problem is also affected by $\beta_k$. In words, there is a tradeoff between the number of outer and inner loop iterations of Algorithm~\ref{Algo:2}. We highlight this tradeoff for a number of subroutines below.

First, we characterize the iteration complexity of Algorithm~\ref{Algo:2} for finding a first-order stationary point of~\eqref{prob:01}.
We propose to use the standard accelerated proximal method (APGM), guarantees of which are analyzed in~\cite{ghadimi2016accelerated} for nonconvex problems of the form~\eqref{e:exac}.
They show that APGM can find $\epsilon$ first-order stationary point in 
\begin{equation}
\mathcal{O}\left ( \frac{\lambda_\beta^2\left( \|x^\star \|^2 + M^2 \right)}{\epsilon} \right)
\end{equation}
iterations, where $\lambda_\beta$ denotes the Lipschitz constant of the gradient of ${\mathcal{L}_{\beta}(x, y)}$ as in~\eqref{eq:smoothness of Lagrangian} and $M$ is defined with the following bound:
%
\begin{equation}
\min_{\text{dom}\{g\}}\|x\| \leq M.
\end{equation}
%
Using this result, we can get the following corollary describing the iteration complexity in terms of the calls to the first-order oracle:

\begin{corollary}\label{cor: first_order}
Let us use the following form for $\beta$
\begin{equation*}
\beta_k = \alpha^k, ~~ \alpha > 1.
\end{equation*}

If we use APGM from~\cite{ghadimi2016accelerated} for step 2 in Algorithm~\ref{Algo:2}, it finds an $\epsilon$-first-order stationary point in the sense that
\begin{equation}
\dist(-\nabla_x \mathcal{L}_\beta(x,y), \partial g(x)) \leq \epsilon, ~~~~
A(x) = 0 \leq \epsilon,
\end{equation}
in $T_K$ number of calls to the first-order oracle, where

\begin{equation}
T_K \leq \tilde{\mathcal{O}} \left( \frac{Q^{\frac{3}{2}}(\|x^\star\|^2 + M^2)}{\epsilon^{3}} \right).
\end{equation}
\end{corollary}


\subsection{Complexity results for second-order stationarity}
{\color{red}{Ahmet (note to myself): not sure of the constants of trust-region, check again}} \\
In this subsection, we focus on finding second-order stationary points of~\eqref{prob:01}.
For this purpose, we need to use a subroutine in Step 2 of Algorithm~\ref{Algo:2} to find approximate second-order stationary points of the subproblem~\eqref{e:exac}.
As shown in~\cite{nouiehed2018convergence}, finding approximate second-order stationary points for constrained problems is in general NP-hard.
For this reason, we focus on the special case of~\eqref{prob:01} with $g=0$ in this section.

In this case, we focus on find second-order stationary points of~\eqref{prob:01} in the sense of~\eqref{eq:sec_opt}.

We first give a theorem to show the convergence rate of the algorithm for second order stationarity: \\
{\color{red}{Ahmet: I think that it is possible to remove sufficiently large k0 assumption here. }} 
\begin{corollary}
\label{thm:main_second}
Under the assumptions of Theorem~\ref{thm:main}, the output of Algorithm~\ref{Algo:2} satisfies 
\begin{align}
%& \dist^2( -\nabla_x \L_{\b_{k-1}}(x_k,y_k),\partial g(x_k)) + \| A(x_k)\|^2   \nonumber\\
%& = \frac{1}{\b_{k-1}^2}\left( \frac{8 \lambda'_A\s_k^2 + 4}{ \nu^2} ( \lambda'_f+\lambda'_A y_{\max})^2 + 2\right) \nonumber \\ 
%&=: \frac{Q}{\beta_{k-1}^2}. 
\lambda_{\text{min}}(\nabla _{xx}\mathcal{L}_{\beta_{k-1}}(x_k, y_k)) \geq - \frac{C}{\beta_{k-1}} - \epsilon_{k-1}.
\end{align}
\end{corollary}
%
We now focus on total complexity of finding second-order stationary points of~\eqref{prob:01} in terms of calls to the second-order oracle.
We consider using trust region method for Step 2 of Algorithm~\ref{Algo:2} developed in~\cite{cartis2012complexity}.
In~\cite{cartis2012complexity}, the complexity for finding the second order stationary points of an unconstrained problem is derived to be
%
\begin{equation}
\mathcal{O}\left ( \frac{\lambda_{\beta, H}^2 (\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y))}{\epsilon^3} \right),
\end{equation}
%
where $\lambda_{\beta, H}$ is the Lipschitz constant of the Hessian of the augmented Lagrangian, which is of the order of $\beta$.
In~\cite{cartis2012complexity}, the term $\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y)$ is bounded by a constant independent of $\epsilon$.
We have a similar assumption for this quantity $\forall \beta_k$.

Consequently, we get the following result:
%
\begin{corollary}\label{cor: second_order}
Let us use the following form for $\beta$
\begin{equation*}
\beta_k = \alpha^k, ~~ \alpha > 1.
\end{equation*}
%
We use the trust region method from~\cite{cartis2012complexity} for step 2 in Algorithm~\ref{Algo:2} and assume that 
\begin{equation}
\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y)
\end{equation}
is upper bounded by a constant independent of $\epsilon$.
Algorithm~\ref{Algo:2} then finds an $\epsilon$-second-order stationary point of~\eqref{prob:01} in $T_K$ total number of calls to the second order oracle where
%
\begin{equation}
T_K \leq \tilde{\mathcal{O}}\left( \frac{Q^{\frac{5}{2}}}{\epsilon^{5}} \right).
\end{equation}
\end{corollary}
%
{\color{red} Ahmet: I'll check again the constants of the corollaries, eps dependence should be correct.}\\
%
\textbf{Regularity.}  The key condition in Theorem~\ref{thm:main} is \eqref{eq:regularity}. As the penalty weight $\b_k$ grows, the primal subroutine (Step 2) places an increasing emphasis on reducing the feasibility gap and \eqref{eq:regularity} formalizes this intuition. We verify this condition rigorously in several examples in Section~\ref{sec:experiments}. 

We argue that such a condition is necessary for controlling the feasibility gap of~\eqref{prob:01} and ensuring the success of Algorithm~\ref{Algo:2}. To motivate this condition, recall the Slater's condition for $g(\cdot) = \delta_{\mathcal{X}}(\cdot)$ which states that
\begin{equation}
\text{relint} (\mathcal{X}) \cap \{ x\in\mathbb{R}^d: A(x) = b \} \neq \emptyset.
\end{equation}
This condition plays a key role in convex optimization since it is a sufficient condition for strong duality. 
As a result, Slater's condition guarantees the success of a variety of primal-dual algorithms for linearly constrained convex optimization.

As a visual example, in~\eqref{prob:01}, we consider the case where $f=0$,  $g=\delta_\mathcal{X}$ where $\mathcal{X}$ is a convex set, and $A$ is a linear  operator. 
Slater's condition removes any pathological cases by ensuring that the affine subspace is not tangent to $\mathcal{X}$, see Figure~\ref{fig:convex_slater}.  
In such pathological cases, finding a feasible point of~\eqref{prob:01} is particularly difficult. 
For example, the iterates of the alternating projection algorithm (which iteratively projects onto $\null(A)$ and $\mathcal{X}$) have arbitrarily slow convergence, as show in Figure~\ref{fig:conve_slater}.

{\color{red}{We should add a figure here with circle and line.}}




==> neurips2019 copy/sections/introduction.tex <==
Generative Adversarial Networks (GANs) \citep{Goodfellow2014} show great promise for faithfully modeling complex  data distributions, 
such as natural images \citep{Radford2015,brock2018large} or audio signals
\citep{engel2018gansynth,donahue2019wavegan}. Understanding and improving the theoretical and
practical aspects of their training has thus attracted significant interest~\citep{Lucic2018,Mescheder2018,daskalakis2018training,Hsieh2018,Gidel2019}.
%More recently, the question of how to leverage the modeling power of GANs to improve
%or devise new applications has seen positive and encouraging answers in tasks

Researchers have also begun to leverage the modeling power of GANs  in applications ranging from compressive sensing \citep{Bora2017}, to image denoising
\citep{Lipton2017,Tripathi2018}, to robustness against adversarial examples
\citep{Ilyas2017,Samangouei2018}.

These and other \citep{Dhar2018,Ulyanov2018}  applications  model high-dimensional data as the output of the generator network associated with a GAN, and often lead to a highly non-convex optimization problem of the form $\min_z f(G(z))$, where the the generator $G$ is  nonlinear and $f$ is  convex. We then find the optimal \textit{latent vector} $z$, as illustrated in Section \ref{sec:experiments} with several examples. 
% such that $G(z)$ minimizes certain convex
%functional. 
%This gives rise to a poorly understood highly non-convex
%optimization problem due to the presence of the non-linear map $G$.


This GAN-based optimization problem poses various difficulties for existing first-order algorithms.  Indeed, to our knowledge, the only existing provable algorithm for solving \eqref{eq:emp loss min} relies  on  the existence of a projection oracle, and is limited to  the special case of \emph{compressive sensing} with a generative prior~\citep{Shah2018,Hegde2018}, see Section \ref{sec:related_works} for the details. 
%. More specifically, in the context of compressive sensing with a generative prior,  \citet{Shah2018,Hegde2018} proves linear convergence for the Projected Gradient Descent (PGD) in the presence of a projection oracle and in special case of $F(w,z)=\normb{Aw-b}_2^2$ for some \textit{measurement matrix}
%$A$ in \eqref{eq:emp loss min}. 
The main computational bottleneck is of course the non-convex projection step, %constraints set in \eqref{eq:emp loss min}, 
%oracle corresponding to the solution of \eqref{eq:emp loss min} with $F(w,z)
%=\normb{w - w^\natural}_2^2$. Even in this simple case, 
for which {no convergence analysis in terms of the geometry of the underlying  generator $G$ currently exists.}

On the other hand, Gradient Descent (GD) and its adaptive variants \citep{Kingma2014}  cannot efficiently handle non-smooth objective functions, as they are entirely oblivious to the composite structure of the problem \citep{nesterov2013gradient}. A simple example is denoising with the $\ell_\infty$-norm, for which subgradient descent (as the standard non-smooth alternative to GD) fails in practice, as observed in Section
\ref{sec:experiments}.
%In order
%to profit from the well-understood analysis of such c
%In analogy with composite convex optimization \citep{nesterov2013gradient},
%it is therefore imperative to design a flexible class of algorithms that efficiently handle non-smooth objectives.
%different breed of algorithms that {decouple} the
%convex objective function and the non-convex constraint in \eqref{eq:emp loss
%min}. 

With the explosion of GANs in popularity, there is consequently a pressing need
for provable and flexible optimization algorithms to solve the resulting
non-convex and (possibly) non-smooth problems. The present work addresses this need by focusing on the
general optimization template
\begin{align}
\begin{array}{lll}
    \underset{w, z}{\text{minimize}} & & F(w,z) := L(w) + R(w) + H(z) \\
\text{subject to } & & w = G(z),
\end{array}
\label{eq:emp loss min}
\end{align}
where $L:\R^d \rightarrow \R$ is  convex and smooth, $R:\R^d \rightarrow \R$ and
$H: \R^s \rightarrow \R$ are convex but not necessarily smooth, and
$G:\R^s\rightarrow\R^d$ is differentiable but often non-linear, corresponding to the generator network associated with  a GAN.
Even though $R$ and $H$ might not be smooth, we assume throughout that their
proximal mappings can be efficiently computed \citep{Parikh2014}.  

For brevity,
we refer to~\eqref{eq:emp loss min} as \textit{optimization with a generative
prior} whenever $G$ is given by the generator neural network associated with a GAN
\citep{Goodfellow2014}. In this context, we make three key contributions, summarized below:
%Our contributions can be summarized as


%is that they are oblivious to the
%particular composite structure of the objective, and might handle the possibly
%nonsmooth components $R$ and $H$ inefficiently. 

%Let us summarize the main contributions of this work. 

\textbf{1. Algorithm:} We propose an efficient and scalable (linearized)
Alternating Direction Method-of-Multipliers (ADMM) framework  to
solve \eqref{eq:emp loss min}, see Algorithm \ref{alg:admm}. To our
knowledge, this is the first non-convex and linearized ADMM algorithm for nonlinear constraints with provable fast
rates to solve problem \eqref{eq:emp loss min}, see
Section~\ref{sec:related_works} for a detailed literature review.

We evaluate this algorithm numerically in the context of denoising with GANs in
the presence of  adversarial or stochastic noise, as well as compressive
sensing~\citep{Bora2017}. In particular, Algorithm~\ref{alg:admm} allows for
efficient denoising with the $\ell_{\infty}$- and $\ell_1$-norms, with applications
in defenses against adversarial examples \citep{Szegedy2013} and signal
processing, respectively. 
%the numerical evidence suggests
%denoising with $\ell_\infty$ or $\ell_1$ norms is both efficient and also
%improves over iterative descent methods. 

\textbf{2. Optimization guarantees:} We prove  fast approximate convergence for
Algorithm~\ref{alg:admm} under the assumptions of smoothness and near-isometry
of $G$, as well as strong convexity of $L$.
%, as detailed in Section
%\ref{sec:guarantees1}.  % (supplementary \ref{sec:rsc}).
That is, we distill the key geometric attributes of the generative
network $G$  responsible for the success of Algorithm~\ref{alg:admm}.
We then show how some common neural network architectures 
satisfy these geometric assumptions. 

{We also establish a close relation between a variant of Algorithm~\ref{alg:admm} and the gradient descent in \citep{Bora2017} and, in this sense, provide the first rates for it, albeit in a limit case detailed in Section~\ref{sec:guarantees1}. Indeed, one key advantage of the primal-dual formulation studied in this paper is exactly this versatility, as well as the efficient handling of non-smooth objectives.} Lastly, we later relax the assumptions on $L$ to
\textit{restricted} strong convexity/smoothness, thus extending our results to
the broader context of statistical learning with generative priors, which includes
compressive sensing \citep{Bora2017} as a special case. 
%\label{pr:G-assumptions}.

\textbf{3. Statistical guarantees:} In the context of statistical learning with generative priors, where $L$ in~\eqref{eq:emp loss min} is replaced with an 
%$L(w)=\E_{x \sim \mu_m}
%l(w;x)$ 
\textit{empirical risk},
% where $\mu_m$ is an empirical
%distribution corresponding to a sample from $\mu$ and $\hat{L}(w)=\E_{x \sim
%\mu} l(w;x)$ is the \textit{population risk}, our main theoretical result is
%\ref{thm:main2} 
we provide the generalization error associated with Algorithm~\ref{alg:admm}. That is, we use the standard notion of Rademacher complexity~\citep{mohri2018foundations} to quantify the number of training data points required for Algorithm~\ref{alg:admm} to learn the true underlying parameter $w^\natural$. 

%Even though a thorough understanding of the non-linear geometry of generative
%priors remains an open problem and active research topic, we carefully justify
%these geometric requirements with the current tools and results. 
%To our
%knowledge, there is no non-convex nor linearized ADMM algorithm with rigorous
%rates to solve problem \eqref{eq:emp loss min}, see
%Section~\ref{sec:related_works} for a detailed review.


%\marginnote{\edita{\textbf{should we mention DARN here? if not, then we should remove the other appearances of DARN later in the paper.}}} Despite their remarkable success, deep neural network classifiers are 
%dangerously susceptible to adversarial attacks, in which a small (often
%imperceptible) perturbation of the network's input leads to erroneous
%classification \citep{Szegedy2013}. 
%\edita{\textbf{AE: please add a sentence here that says the problem is open, hence the need for new work and its importance.}}
%In order to thwart the attack
%and accurately classify an adversarially perturbed sample
%$w^\natural=w^\star + \xi$ with a bounded perturbation $\norm{\xi} \leq \epsilon$,  %for a given norm
%%$\norm{\cdot}$ and perturbation size $\epsilon$, 
%\citet{Samangouei2018,
%Ilyas2017} recently proposed to first denoise $w^\natural$ by projecting it onto
%the manifold of natural examples, which is encoded by a Generative Adversarial
%Network (GAN) \citep{Goodfellow2014},
%%\footnote{\edita{Training GANs is commonly modeled as a minimax game with an
%%adversary, hence the namesake, and should not be confused with adversarial
%%attacks to a network in our context.}}
%and then feed the denoised sample to a classifier. \edita{\textbf{AE: please add a sentence that says their method has a lot of potential and has successful preliminary results, so we're not extending a dead end result.}}
%More precisely, given
%an input $w^\natural \in \R^d$ and a generative network $G:\R^s\to \R^d$, the authors
%proposed to approximately solve the  optimization problem
%%gradient descent iterations
%%\edita{DARN sets}
%\begin{equation}
%    \label{eq:l2-denoising}
%    z^* := \argmin_{z\in \R^s} \norm{w^\natural - G(z)}_2^2,
%\end{equation}
%and use $w^*:=G(z^*)$ as the input to the classifier.
%Program \eqref{eq:l2-denoising} is non-convex because the generator $G$
%is often a highly nonlinear map \edita{\textbf{AE: is it possible to add a reference here?}}. In practice, \eqref{eq:l2-denoising} is solved
%to (approximate) first-order stationarity with the gradient descent algorithm
%or other first-order algorithms such as ADAM \citep{Kingma2014} \edita{\textbf{AE: is it possible to name one more 1st order algorithm in addition to adam?}}. The  
%performance of \eqref{eq:l2-denoising} in the absence adversarial noise has also been studied empirically in 
%\cite{Lipton2017,Tripathi2018}.\edita{\textbf{AE: it seems inconsistent to switch between cite and citep. shouldn't we use just one?}} 
%
%%We now pinpoint certain drawbacks of the the optimization objective
%%\eqref{eq:l2-denoising} as used in such applications. 
%
%The main drawback of \eqref{eq:l2-denoising} is that, in the adversarial setting,
%there is often a mismatch between the norm $\norm{\cdot}$ used by the attacker---often $\ell_\infty$ norm \citep{Madry2018}---and the $\ell_2$ norm in \eqref{eq:l2-denoising}.
%To realize the full potential of generative denoising as a defense mechanism,
%it appears natural to instead solve \eqref{eq:l2-denoising} with $\ell_2$ replaced
%by the attacker's norm $\|\cdot\|$.
%%same norm that bounds the adversarial perturbation. 
%Beyond successful defense, the flexibility in the choice of norm in \eqref{eq:l2-denoising} is valuable in denoising. \edita{\textbf{AE: somewhat not clear what you mean in this next sentence.}} In the presence
%of stochastic noise, it is well known that the $\ell_2$ loss is more sensitive
%to outliers when compared its $\ell_1$ counterpart, and could potentially
%provide better reconstruction when denoising with GANs.
%
%
%However, unlike \eqref{eq:l2-denoising}, the resulting optimization problems
%would be both non-smooth and non-convex, and consequently \emph{cannot} be
%solved efficiently  with available algorithms such as gradient descent or
%ADAM. Moreover, these algorithms in general do not offer any theoretical
%guarantees, see Section
%\ref{sec:related_works} for a detailed review of the literature and Section .
%
%This need for new algorithms and theory for efficient generative denoising
%%To summarize, new algorithms and theory are required for efficiently denoising
%%with GANs, which in particular would allow us to overcome the drawbacks
%%mentioned above.  This work precisely addresses this issue and 
%motivates us to consider the
%non-convex program
%\begin{align}
%\begin{array}{lll}
%\underset{w, z}{\text{minimize}} & & L(w) + R(w) + H(z) \\
%\text{subject to } & & w = G(z),
%\end{array}
%\label{eq:emp loss min}
%\end{align}
%where $L:\R^d \rightarrow \R$ is a  smooth function, $R:\R^d
%\rightarrow \R$ and $H: \R^s \rightarrow \R$ are convex but not
%necessarily smooth, and $G(z)$ is a differentiable but often non-linear constraint %on the parameter $w \in \R^d$ 
%with the latent variable $z \in\R^s$. Even though
%$R$ and $H$ might not be smooth, we assume that their proximal mappings
%can be efficiently computed \citep{Parikh2014}. Such a template covers generative denoising
%as a special case by choosing $L(w)=0$, $R(w)=\|w^\natural -
%w\|$, and $G:\R^s\rightarrow\R^d$ a generative network with smooth activation
%functions. 

%Beyond generative denoising, \eqref{eq:emp loss min} covers a wide range of
%optimization problems, such as \textit{compressive sensing} with generative
%prior as introduced by \citet{Bora2017} and, more broadly, statistical
%learning with generative priors. 

%Our numerical evidence illustrates that not only the $\ell_\infty$-DARN-GAN
%problem can be efficiently solved, but also it shows noticeable improvement
%over existing $\ell_2$-DARN-GAN proposals. We also compare our proposed
%approach for compressive sensing and other signal processing tasks with
%generative priors, to show that it is either competitive or outperforms common
%baselines in practice.

%\edita{Beyond DARN and denoising with a generative prior,} the general template in \eqref{eq:emp loss min} \edita{can be applied to} other problems such as \textit{compressive sensing with generative priors} \citep{Bora2017} \edita{and, broadly-speaking statistical learning with generative priors}, which might of independent interest, \edita{see Section \ref{sec:related_works} for more details.}
%To our knowledge, \edita{there is no non-convex nor linearized ADMM algorithm with rigorous rates to solve problem \eqref{eq:emp loss min}, see Section~\ref{sec:related_works} for a detailed review. In this sense, our findings might also have a significant impact on these problems.}


==> neurips2019 copy/sections/learning.tex <==

So far, we have assumed $L$ to be strongly convex in \eqref{eq:emp loss min}, see Assumption \ref{assump:risk} and Theorem \ref{thm:main}. In this section, we relax this assumption on $L$ in the context of  statistical learning with generative priors, thus extending Theorem \ref{thm:main} to applications such as compressive sensing. We also provide the corresponding generalization error in this section. 

Here, we follow the standard setup in learning theory~\cite{mohri2018foundations}. 
Consider the probability space $(\mathbb{X}, \chi)$, where
$\mathbb{X} \subset \R^d$ is a compact set, equipped with the Borel sigma
algebra, and $\chi$ is the corresponding probability measure. To learn an
unknown parameter $w^\n \in \R^d$, consider the optimization program
\begin{align}
\underset{w\in \R^p}{\text{min}} \,\,  L(w),
\qquad
L(w) := \E_{x \sim \chi} l(w,x),
\label{eq:pop loss min}
\end{align}
where $L:\R^p\rightarrow \R$ is the differentiable \textit{population risk}
and $l:\R^d \times \R^p \rightarrow\R$ is the corresponding \emph{loss function}. We
also assume that Program \eqref{eq:pop loss min} has a unique solution $w^\n\in
\R^p$. The probability measure $\chi$ above is itself often unknown and we instead
have access to $m$ samples drawn independently from $\chi$, namely,
$\{x_i\}_{i=1}^m \sim \chi$. This allows us to form the \emph{empirical loss}
\begin{align}
L_m(w) := \frac{1}{m} \sum_{i=1}^m l(w,x_i).
\label{eq:emp loss defn supp}
\end{align}
Often, $m \ll p$ and to avoid an ill-posed problem, we must leverage any
inherent structure in $w^\n$. In this work, we consider a differentiable map
$G: \R^s \to \R^d$ and we assume that $w^\n \in G(\R^s)$.  That is,
there exists $z^\n \in \R^s$ such that $w^\n = G(z^\n)$. While not necessary, we limit ourselves in this section to the important case where $G$ corresponds to a  GAN, see Section \ref{sec:introduction}. 

%The defferentiability assumption on $G$ is not
%restrictive. For example, the non-differentiable ReLU activation function in a GAN can be  replaced with its smooth alternative ELU \citep{clevert2015fast}, which only differs
% from ReLU near the origin. In our experiments, we were able to succesfully train GANs with ELU activation function. \citet{gulrajani2017improved} also reports
%successful training of GANs with another differentiable activation function. See also the discussion after Assumption~\ref{assump:G_ssmth}. 

To learn $w^\n$ with the generative prior $w^\n=G(z^\n)$,  we propose
to solve the program
\begin{align}
\begin{array}{lll}
\underset{w,z}{\text{minimize}} & & L_m(w) + R(w) + H(z)\\
\text{subject to } & & w = G(z),
\end{array}
\label{eq:emp loss min supp}
\end{align}
where $R:\R^p \rightarrow \R$ and $H: \R^s \rightarrow \R$ are convex but not
necessarily smooth. Depending on the specific problem at hand, the \emph{regularizers}
$R$ and $H$ allow us to impose  additional structure on $w$ and
$z$, such as sparsity or set inclusion. Throughout, we again require that
the {proximal maps} \citep{Parikh2014} for $R$ and $H$ can be computed
efficiently, as detailed in Section \ref{sec:algorithm}. 
%Several examples of
%this broad learning framework are discussed in Section \ref{sec:experiments},
%including \emph{compressive sensing} with deep-net priors.

%\subsection{\edita{Empirical Risk }Minimization}
%\label{sec:error_min}
%\notea{Changing $x$ to $u$ for parameter. $u$ could be the labels, could be the image itself. This is to cover the general learning with GAN prior rather than just inverse problems.}
%We consider the optimization problem
%\begin{equation}
%\begin{array}{llll}
%& \underset{\up}{\text{minimize}}
%& & \loss(\up) \\
%& \text{subject to}
%& & \up \in \bigcup_{k=1}^K G_k(\Sprior)
%\end{array}
%\label{eq:problem_general}
%\end{equation}
%where we assume that the objective function $\loss$ as well as each $G_k$ for
%$k \in [K]$ are differentiable. The measurement error minimization problem
%corresponds to $\loss(\up)=\norm{A\up - b}_2^2$.  
%Finally, each constraint of the form $\up_k \in G_k(\Sprior)$ can be rewritten as
%$\up_k = G_k(\prior_k)$ for every $ \prior_k \in \Sprior$. 
%Writing $\Prior=[\prior_1, \ldots,
%\prior_K]$ we arrive at the optimization problem





%Let us now study the convergence of  Algorithm \ref{alg:admm} when solving
%problem \eqref{eq:emp loss min}. As detailed in Supplementary
%\ref{sec:relations}, our result includes as a special case the
%convergence rate of the algorithm proposed in \citep{Bora2017} without
%convergence analysis.
% Our characterizations are based on the precise adaptive update rules on the penalty parameters, as described in Section 2. 

%To the best of our knowledge, in the context of learning
%with deep-net priors, the only existing convergence rate appears in
%\cite{Shah2018, Hegde2018} for the special case of linear regression and relies on a
%projection oracle onto a non-convex set. Establishing the accuracy of the
%numerical approach used in \cite{Shah2018, Hegde2018} in lieu of this oracle is
%an open question and arguably a daunting task in itself. In this sense,
%Theorem \ref{thm:main} below provides the first convergence rate for solving
% \eqref{eq:emp loss min} and its equivalent formulations. See Section \ref{sec:related_works} for a more detailed review of the literature. 

%Let $(w^*,z^*)$ be solutions of  \eqref{eq:emp loss min} and let
%$\lambda^*$ be a corresponding optimal dual variable. Let also
%$\{w_t,z_t,\lambda_t\}_{t\ge 0}$ denote the output sequence of Algorithm~\ref{alg:admm}. Our first characterization in this paper, Theorem
%\ref{thm:main} below, establishes the linear convergence of Algorithm~\ref{alg:admm}
%to a neighborhood of solutions $(w^*,z^*)$ under certain technical assumptions,
%described below.

Let us now state our assumptions, some of which differ from Section \ref{sec:guarantees1}. 
\begin{assumption}
\label{assump:props_of_l_supp}
\textbf{\emph{Convexity / strong smoothness of loss: }}
We assume that $\lossf(\cdot, \cdot)$ is convex in both of its arguments.
Moreover, we assume that $\lossf(w, \cdot)$ is strongly smooth, namely, there
exists $\s_\lossf \ge 0$ such that for every $x,x'\in \mathbb{X}$
\begin{align}
    \D_\lossf(x,x';w) \le \dfrac{\s_\lossf}{2}\norm{x-x'}_2^2,
\label{eq:props_of_l_supp}
\end{align}
where $\D_\lossf$ stands for the \emph{Bregman divergence} associated with $l(w,\cdot)$,
\begin{align*}
\D_l(x,x';w) = l(w,x') - l(w,x) - \langle x'-x, \nabla_x l(w,x) \rangle .
\end{align*}
\end{assumption}
\begin{assumption}\textbf{\emph{Strong convexity / smoothness of the population risk:}}\label{assump:risk_supp}
We assume that the population risk $L$ defined as
\begin{equation}
    \label{eq:poploss_supp}
L(w) := \E_{x \sim \chi} l(w,x),
\end{equation}
is both strongly convex and smooth, i.e., there exist $0<\zeta_L\le \sigma_L$
such that
\begin{align*}
\frac{\zeta_L}{2} \| w-w'\|^2&  \le {D}_L(w,w') \le \frac{\sigma_L}{2} \| w-w'\|^2,
\end{align*}
\begin{align}
D_L(w,w') & = L(w') - L(w) - \langle w'-w,\nabla L(w) \rangle,
\label{eq:L_str_cvx_supp}
\end{align}
for every $w, w'\in \R^d$. In the following we denote by $w^\n$
the minimizer of (\ref{eq:poploss_supp}). In view of our assumption,
such minimizer is unique.
% NOTE BY FABIAN: here w^\n has not been properly introduced
% In particular, it follows that $w^\n$ is the unique
% minimizer of the population loss.
\end{assumption}
Assumptions~\ref{assump:props_of_l_supp} and \ref{assump:risk_supp}
 are standard in statistical learning~\cite{mohri2018foundations}. For example, in linear regression, we might take
 \[
 l(w,x)= \frac{1}{2}|\langle w-w^\n,x \rangle|^2,
 \]
 \[
 L_m(w) = \frac{1}{2m} \sum_{i=1}^m |\langle w-w^\n,x_i \rangle|^2,
 \]
for which both Assumptions \ref{assump:props_of_l_supp} and \ref{assump:risk_supp} are met. Lastly, we require that the Assumptions \ref{assump:G_ssmth} and \ref{defn:G_iso} on $G$ hold in this section, see and Proposition~\ref{pr:G-assumptions} for when these assumptions hold for generative priors. 
%\begin{assumption}
%\label{assump:G_ssmth}
%\textbf{\emph{(Strong smoothness of the prior)}}
%We say that $G$ is strongly smooth if there exist $\nu_G\ge 0$ such that
%\begin{align}
%& \| G(z') - G(z) - DG(z) (z'-z) \|_2  \nonumber\\
%& \le \frac{\nu_G}{2} \|z'-z\|_2^2
%\end{align}
%for every $z,z'\in \R^s$. Above, $DG$ is the Jacobian of $G$.
%\end{assumption}
%\begin{assumption}
%\label{defn:G_iso}
%\textbf{\emph{(Near-isometry of prior)}}
%We say that $G$ is a near-isometric map if there exist
%$\iota_G,\kappa_G> 0$ such that
%\begin{align}
%\iota_G \|z' - z\|_2 \le  \|G(z') - G(z)\|_2
%\le  \kappa_G \|z' - z\|_2,
%\label{eq:lipschitz of G statement}
%\end{align}
%for every $z,z'\in \R^s$.
%\end{assumption}

%For $G$ to satisfy \eqref{eq:lipsG} it suffices that it be Lipschitz
%continuous, which holds for architectures with Lipschitz continuous activation
%functions, as is the case with the most common choices. Moreover, the
%Lipschitz constant of $G$ can be controlled by regularizing the network
%\citep{raghunathan2018certified,tsuzuku2018lipschitz,yang2018diversity}.
%
%Condition \eqref{eq:lipschitz of G statement} means that $G$ must be
%\emph{stably} injective: faraway inputs should remain mapped to faraway outputs
%under $G$. Consider the parametrization of a circle $z\mapsto (\sin(z),
%\cos(z)), z \in \R$ as a pathological example. Stable injectivity is necessary
%for the success of Algorithm \ref{alg:admm} and is not an artifact of our proof
%techniques. Indeed, without this condition, the $z$ updates in Algorithm
%\ref{alg:admm}
%might not reduce the feasibility gap $\norm{w-G(z)}_2$ (see Steps 1 and 3 of Algorithm
%\ref{alg:admm}). Geometric assumptions on nonconvex constraints are commonplace
%in optimization literature
%\citep{birgin2016evaluation,flores2012complete,cartis2018optimality} and have a
%few precedents in the literature of neural networks too
%\citep{hand2017global,ma2018invertibility}, which we discuss in Section
%\ref{sec:related_works}.
% NOTE BY FABIAN: THIS IS NOT TRUE
%\emph{Mode collapse}, in which a trained generator $G$ fails to imitate some
%of modes of the original multi-modal distribution, is a notable pathological
%case for which $G$ would not be stably injective. There are various guidelines
%in the literature to protect against mode collapse \cite{che2016mode,
%metz2016unrolled, nguyen2017dual, lin2018pacgan}
%%Mode collapse, in which the trained generator collapses to a singleton is a notable pathological case for which $G$ would not be stably injective; there are various guidelines in the literature to protect against mode collapse~\cite{lin2018pacgan}.\textbf{Note: Fabian, Chen, is this description of mode collapse correct? If not, please correct. Add citation too.}. 


As a consequence of Assumption \ref{assump:props_of_l_supp}, we have that $L_m$ is
convex. We additionally require $L_m$ to be strongly convex and smooth in the
following restricted sense. Even though $L_m$ is random because of its
dependence on the random training data $\{x_i\}_{i=1}^m$, we ensure later in this section that the next condition is indeed met with high
probability when $m$ is large enough.
\begin{definition}
\label{defn:Lm_scvx}
\textbf{\emph{Restricted strong convexity / smoothness of empirical loss: }}
We say that $L_m$ is strongly convex and smooth on the set $W\subset\R^p$ if
there exist $0<\mu_L\le \nu_L$ and $\ol{\mu}_L,\ol{\nu}_L\ge 0$ such that
\begin{align}
\D_{L_m}(w,w') &   \ge \frac{\mu_L}{2}\|w'-w\|_2^2 - \ol{\mu}_L, \nonumber\\
\D_{L_m}(w,w')
& \le \frac{\nu_L}{2}\|w'-w\|_2^2 + \ol{\nu}_L,
\end{align}
\begin{align*}
\D_{L_m}(w,w') := L_m(w') - L_m(w) - \langle w' - w, \nabla L_m(w) \rangle,
\end{align*}
for every $w,w'\in W$.
\end{definition}
%Under the above assumptions, our first main result is that
%Algorithm \ref{alg:admm} converges linearly to a neighborhood of the solution, see Supplementary \ref{sec:theory} for the proof.

%While there are numerous quantities involved in the above assumptions and
%consequently in Theorem \ref{thm:main}, the main message is simple: The
%optimization error $\|w_t-w^*\|_2$ and the \emph{feasibility gap} $\|w_t - G(z_t)\|_2$
%converge linearly to reach a certain accuracy. Theorem \ref{thm:main} is
%immediately followed by a number of clarifying remarks.
%$\psi_\rho$ and $\mu_\rho \psi_\rho/\rho$ linearly, respectively.
%Here, $\rho$ is the penalty weight of the augmented Lagrangian and the quantities $\psi_\rho$ and $\mu_\rho$ are defined in the proof. 

Under the above assumptions, a result similar to Theorem \ref{thm:main} holds, which we state without proof.
\begin{theorem}
\label{thm:main-stat-learn}

\textbf{\emph{(guarantees for Algorithm \ref{alg:admm})}}
Suppose that Assumptions~\ref{assump:G_ssmth}-\ref{assump:risk_supp} hold. 
Let $(w^*,z^*)$ be a solution of program (\ref{eq:emp loss min}) and let $\lambda^*$ be a corresponding optimal dual variable.  Let also
$\{w_t,z_t,\lambda_t\}_{t\ge 0}$ denote the output sequence of
Algorithm~\ref{alg:admm}. 
Suppose that $L_m$
satisfies the restricted strong convexity and smoothness in
Definition~\ref{defn:Lm_scvx} for a set $W\subset \R^p$ that contains a
solution $w^*$ of  (\ref{eq:emp loss min}) and all the iterates
$\{w_t\}_{t\ge 0}$ of Algorithm \ref{alg:admm}.\footnote{If necessary, the inclusion
$\{w_t\}_{t\ge 0}\subset W$ might be enforced by adding the indicator function
of the convex hull of $W$ to $R$ in  \eqref{eq:emp loss min}, similar
to \cite{agarwal2010fast}.} Suppose also that the primal step sizes $\a,\b$ in  Algorithm~\ref{alg:admm} satisfy
\begin{align}
\a  \le  \frac{1}{\nu_\rho},
%\widetilde{\alpha},%(\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
\qquad
\b \le \frac{1}{\xi_\rho + 2\a\tau_\rho^2}.
%\frac{\xi_\rho}{2}+\a \tau_\rho^2 \le \frac{1}{2\b}, 
%\widetilde{\beta},%(\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,%\lambda_0),
%,(\a,\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
\qquad \s_0 \le \s_{0,\rho}, 
\label{eq:step_size_reqs_thm}
\end{align}
Then  it holds that
\begin{align}
\frac{\|w_t-\wh{w}\|_2^2}{\a}+\frac{\|z_t-\wh{z}\|_2^2}{\b} \le 2(1-\eta_{\rho})^t \Delta_{0} +
\frac{\ol{\eta}_\rho}{\rho},
\label{eq:linr_cvg_thm}
\end{align}
\begin{align}
\label{eq:feas-thm}
\|w_t - G(z_t)\|_2^2 \le 
\frac{4(1-\eta_\rho)^t\Delta_0}{\rho}+ \frac{\widetilde{\eta}_\rho}{\rho^2}
,
\end{align}
for every iteration $t$. Above, $\Delta_0 = \mathcal{L}_\rho(w_0,z_0,\lambda_0)- \mathcal{L}_\rho(w^*,z^*,\lambda^*)$ is the initialization error, see~(\ref{eq:defn_aug_lagr}).
The convergence rate $ 1-\eta_\rho\in (0,1)$ and the quantities  $\nu_\rho,\xi_\rho,\tau_\rho,\s_{0,\rho},\ol{\eta}_\rho,\widetilde{\eta}_\rho$ above depend on the parameters in the Assumptions \ref{assump:G_ssmth}-\ref{assump:risk_supp} and on $\lambda_0,\s_0$. 
%As an example,  in the regime where $\mu_L \gg \rho$ and $\iota_G^2 \gg \nu_G$, we can take 
%\begin{align*}
%\a \approx \frac{1}{\nu_L}, \qquad \b\approx \frac{1}{\rho \kappa_G^2},
%\qquad \frac{\rho \nu_G}{\kappa_G^2}\lesssim\s_0 \lesssim \rho\min \l(\frac{\mu_L^2}{\nu_L^2},\frac{\iota_G^4}{\kappa_G^4}\r),
%\end{align*}
%\begin{align}
%\eta_\rho \approx \min\l(\frac{\mu_L}{\nu_L}, \frac{\iota_G^2}{\kappa_G^2}  \r),
%\qquad 
%\ol{\eta}_\rho \approx \widetilde{\eta}_\rho \approx  \max\l(\frac{\nu_L}{\mu_L}, \frac{\kappa_G^2}{\iota_G^2}  \r),
%\label{eq:step-sizes-example}
%\end{align}
%where  $\approx$ and $\lesssim$   suppress the universal constants and dependence on $\lambda^*$ for the sake of clarity. Note that, in this regime, $\eta_\rho,\ol{\eta}_\rho,\widetilde{\eta}_\rho$ are nearly independent of $\rho$.
%


%--=s-----------------
%\textbf{\emph{(Convergence rate)}}
%Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold and $L_m$
%satisfies the restricted strong convexity and smoothness in
%Definition~\ref{defn:Lm_scvx} for a set $W\subset \R^p$ that contains a
%solution $w^*$ of  (\ref{eq:emp loss min}) and all the iterates
%$\{w_t\}_{t\ge 0}$ of Algorithm \ref{alg:admm}.\footnote{If necessary, the inclusion
%$\{w_t\}_{t\ge 0}\subset W$ might be enforced by adding the indicator function
%of the convex hull of $W$ to $R$ in  \eqref{eq:emp loss min}, similar
%to \cite{agarwal2010fast}.}
%Suppose also that the step sizes of Algorithm \ref{alg:admm} satisfy
%\begin{align}
%\a  \in (\widetilde{\a},   1/\nu_\rho],
%%\widetilde{\alpha},%(\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
%\qquad
%\b  \in ( \widetilde{\b}, 1/\xi_\rho],
%%\widetilde{\beta},%(\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,%\lambda_0),
%\qquad
%\s_0  < \widetilde{\s}_0,%,(\a,\b,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0),
%\label{eq:step_size_reqs_thm}
%\end{align}
%for every iteration $t$. Then it holds that
%\begin{align}
%\|w_t-\wh{w}\|_2^2+\|z_t-\wh{z}\|_2^2 \le \eta_{\rho}^t \widetilde{\Delta}_0 +
%\widetilde{\psi}_\rho,
%\label{eq:linr_cvg_thm}
%\end{align}
%\begin{align}
%\label{eq:feas-thm}
%\|w_t - G(z_t)\|_2^2 \le    \frac{2\eta_{\rho}^t \Delta_0}{\rho} +
%\frac{\mu_\rho{\psi}_\rho}{\rho},
%\end{align}
%for every iteration $t$. The quantities
%$\widetilde{\alpha}$,$\xi_\rho$,$\widetilde{\beta}$,$\nu_\rho$,$\widetilde{\s}_0$,$\eta_{\rho}$,$\widetilde{\Delta}_0$,$
%\Delta_0$,$\mu_\rho$,$\widetilde{\psi}_\rho$,$\psi_\rho$  above depend on the
%parameters
%$\rho$,$\s_l$,$\zeta_L$,$\s_L$,$\nu_G$,$\iota_G$,$\kappa_G$,$\mu_L$,$\ol{\mu}_L$,$\nu_L$,$\ol{\nu}_L$,$\lambda_0$
%and specified at the end of the proof.
\end{theorem}

The remarks after Theorem \ref{thm:main} apply here too.

%Because of the nature of the problem and various assumptions involved, the
%exact expressions for the quantities appearing in Theorem \ref{thm:main} are
%somewhat complicated. Let us however provide a simplified overview of the
%result.
%
%\paragraph{Geometry of prior.}
% At a high level, the more isometric and smooth $G$ is, the faster
% Algorithm~\ref{alg:admm} would converge to a smaller neighborhood of
% solutions. That is, smaller $\kappa_G / \iota_G, \nu_G,
% \ol{\nu}_G,\ol{\iota}_G,\ol{\kappa}_G$ in Assumptions~\ref{assump:G_ssmth} and
% \ref{defn:G_iso}  means that $G$ is more ``regular'' and this in turn leads to
% smaller (faster) convergence rate $\eta_\rho$ and  optimization error
% $\widetilde{\psi}_\rho$ in Theorem~\ref{thm:main}.
%
% In other words, the performance of Algorithm~\ref{alg:admm} depends both on
% the geometry of the ``manifold'' $G(\R^s)\subset \R^p$ and also on how $G$
% maps different points in the latent space $\R^s$  to different points on
% $G(\R^s)$. This dependence on the geometry of prior  and its parametrization
% has precedent in the literature of
% optimization~\cite{birgin2016evaluation,flores2012complete,cartis2018optimality}
% and (manifold) embedding theory~\cite{eftekhari2015new,eftekhari2017happens}.
% Based on this discussion  and in order to gain more insight, the simplified
% expressions that will follow are derived for the idealistic scenario $\nu_G
% \ll \iota_G \approx \kappa_G \ll \rho \ll \nu_L \approx \mu_L$, 
% $\ol{\nu}_G=\ol{\iota}_G = \ol{\kappa}_G = \ol{\nu}_G = \ol{\mu}_L =0$, 
% $\lambda_0 = 0\in \R^m$, and $\s_0 \approx 0$. 
% %Our work appears to be the first to rigorously reveal this dependence in the context of learning with generative priors.
%
%\paragraph{Step sizes.} Lower bounds on the primal step sizes, namely,
%$\widetilde{\alpha},\widetilde{\beta}$ in \eqref{eq:step_size_reqs_thm}, are a
%consequence of the restricted convexity and smoothness assumptions on $L_m$,
%see Definition~\ref{defn:Lm_scvx}. Indeed, such lower bounds have been reported
%before for both convex and nonconvex
%problems~\cite{agarwal2010fast,oymak2018sharp}.
%
%For step size $\a$ in $w$ variable, roughly speaking, $\a\approx
%\frac{1}{\nu_L}$, where $\nu_L$ quantifies the restricted strong smoothness of
%the empirical loss, see Definition~\ref{defn:Lm_scvx}.
%%See \cite{agarwal2010fast} for a precedent in the convex world.
%While $L_m$ and hence $\nu_L$ are both random because of their dependence on
%the training data, we will establish in Section~\ref{sec:guarantees2} that,
%with high probability, $\nu_L\approx \s_L$ if the number of training points $m$
%is large enough. Here, $\s_L$ is the smoothness parameter of the population
%risk, defined in  Assumption~\ref{assump:risk_supp}.
%
%For the step size $\b$ in $z$ variable, loosely speaking, $\b \approx
%\frac{1}{2\rho \kappa_G^2}$, where $\kappa_G$ is the Lipschitz constant of $G$,
%see Assumption~\ref{defn:G_iso}.
%
%\paragraph{Convergence rate.} As specified in the proof,
%\begin{align}
%\eta_\rho \approx 1- \frac{\mu_L}{\nu_L} + \frac{C}{\widetilde{\psi}_\rho^2},
%\end{align}
%for a factor $C$. The  term $1-\frac{\mu_L}{\nu_L} $ is the standard linear
%convergence rate of a $\mu_L$ strongly convex and $\nu_L$ smooth
%function~\cite{nesterov2013introductory}, appearing here by the virtue of the
%assumptions on $L_m$, see Definition~\ref{defn:Lm_scvx}. Note the interesting
%tradeoff present here: Increasing $\widetilde{\psi}_\rho$ reduces $\eta_\rho$.
%That is,  Algorithm~\ref{alg:admm} converges faster to coarser estimates of
%solutions of ~\eqref{alg:admm}. This  naturally leads us to the next
%remark.
%
%\paragraph{Optimization error.} Even as $t$ grows, the optimization error of
%Algorithm~\ref{alg:admm} does not vanish. In particular, it follows from
%\eqref{eq:linr_cvg_thm} that
%\begin{align}
%\lim_{t\rightarrow\infty} \|w_t - w^*\|_2^2 & \le \widetilde{\psi}_\rho, 
%\end{align}
%That is, according to Theorem \ref{thm:main}, the iterates $\{w_t,z_t\}_{t\ge
%0}$ of Algorithm \ref{alg:admm} linearly converge to a neighborhood of
%solutions $(w^*,z^*)$ of  \eqref{eq:emp loss min}, rather than
%converging to $(w^*,z^*)$ itself.
%
%Indeed, it is impossible to obtain linear convergence to solutions even for a
%convex but constrained optimization  \cite{ouyang2018lower}. While we
%are not aware of any general impossibility results for nonconvex problems such
%as  \eqref{eq:emp loss min}, this observation suggests that
%Theorem \ref{thm:main} is sensible.
%
%Theorem \ref{thm:main} also agrees with earlier results for (convex)
%M-estimators~\cite{agarwal2010fast}. Later in Section \ref{sec:guarantees2},
%when bounding the generalization error, we will also see that this limited
%accuracy of Algorithm \ref{alg:admm} may not be consequential from a
%statistical viewpoint.
%
%\paragraph{Feasibility gap.} As with the optimization error,
%Algorithm \ref{alg:admm} is unable to reach exact feasibility, analogous to
%what happens for convex but constrained problems~\cite{ouyang2018lower}.
%Indeed, it follows from \eqref{eq:feas-thm} that
%\begin{align}
%\lim_{t\rightarrow\infty} \| w_t - G(z_t) \|_2^2 &  \le \mu_\rho \psi_\rho / \rho.
%\end{align}
%
%===========================

\subsection{Generalization Error \label{sec:gen-err}}
Building upon the optimization guarantee in Theorem~\ref{thm:main_stat}, our next result in this section is Theorem~\ref{thm:main_stat}, which quantifies the convergence of the iterates $\{w_t\}_{t\ge 0}$ of Algorithm~\ref{alg:admm} to the true parameter $w^\n$. 


In other words, Theorem~\ref{thm:main_stat} below controls the generalization error of~\eqref{eq:emp loss min}, namely, the error  incurred by using the empirical risk $L_m$ in lieu of the population risk $L$. Indeed, Theorem~\ref{thm:main} is  silent about $\|w_t - w^\n\|_2$.  We address this shortcoming with the following result, proved in Section~\ref{sec:proof of ws_to_wn} of the supplementary material.  
\begin{lemma}\label{lem:ws_to_wn}
Let $R=1_W$ be the indicator function on $W\subset\R^p$ and set $H=0$ in ~(\ref{eq:emp loss min}).\footnote{To be complete, $1_W(w)=0$ if $w\in W$ and $1_W(w)=\infty$ otherwise. } Suppose that $w^*$ belongs to the relative interior of $W$. 
%\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ denotes the relative interior of the set $W$.  
Then it holds that 
\begin{align}
\|w^\n - w^*\|_2 \le \frac{1}{\zeta_L} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w) \|_2.
\label{eq:before_Upsilon}
\end{align}
\end{lemma}
Before bounding the right-hand side of \eqref{eq:before_Upsilon}, we remark that it is possible to extend Lemma~\ref{lem:ws_to_wn} to the case where the regularizer $R$ is a \emph{decomposable} norm, along the lines of~\cite{negahban2012unified}. We will however not pursue this direction in the present work. 
Next note that \eqref{eq:linr_cvg_thm} and Lemma~\ref{lem:ws_to_wn} together imply that 
\begin{align}
 \frac{\| w_t - w^\n\|_2^2}{\a^2} 
& \le \l( \frac{\|w_t - w^*\|_2}{\a}+ \frac{\|w^* - w^\n\|_2}{\b} \r )^2 
\qquad \text{(triangle inequality)} \nonumber\\
& \le \frac{2 \|w_t - w^*\|_2^2}{\a^2} + \frac{2 \|w^*-w^\n\|_2^2}{\b^2}
\quad ( (a+b)^2 \le 2a^2+2b^2  )
 \nonumber\\
& \le 
4(1-\eta_\rho)^t \Delta_0 + \frac{2\ol{\eta}_\rho}{\rho}
+ \frac{2}{\zeta_L^2} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w)\|_2^2. 
\label{eq:before_rademacher}
\end{align}
According to Theorem~\ref{thm:main}, the right-hand side of \eqref{eq:before_rademacher} depends on $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$, which were introduced in Definition~\ref{defn:Lm_scvx}. 
%with the exact dependence specified in the proof of the theorem. 
Note that $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$  and the right-hand side of \eqref{eq:before_Upsilon} are all random variables because they depend on $L_m$ and thus on the randomly drawn training data $\{x_i\}_{i=1}^m$. To address this issue,  we apply a basic result in statistical learning theory as follows. For every $w\in \R^p$ and every pair $x,x'\in \mathbb{X}$, we use Assumption~\ref{assump:props_of_l_supp} to write that 
\begin{align}
\| \nabla l(w,x) - \nabla l(w,x') \|_2 & \le \s_l \| x-x'\|_2
\qquad \text{(see \eqref{eq:props_of_l_supp})} \nonumber\\
& \le \s_l \text{diam}(\mathbb{X}),
\end{align}
where $\text{diam}(\mathbb{X})$ denotes the diameter of the compact set $\mathbb{X}$. Note also that 
\begin{align}
\E_{\{x_i\}_i} \nabla L_m(w) = \nabla L(w), 
\qquad \forall w\in W,
\end{align}
where the expectation is over the training data $\{x_i\}_i$. 
Then, for $\varepsilon>0$ and except with a probability of at most $e^{-\varepsilon}$, it holds that 
\begin{align}
& \| \nabla L_m(w) - \nabla  L(w) \|_2  \nonumber\\
& \le 2 \mathcal{R}_W(x_1,\cdots,x_m) +3\s_l\text{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}} \nonumber\\
& =: \Upsilon_{m,W}(\varepsilon),
\label{eq:emp_proc}
\end{align}
for every $w\in W$~\citep{mohri2018foundations}. Above, 
\begin{align}
 \mathcal{R}_W(x_1,\cdots,x_m)  = 
\E_{E} \l[ \max_{w\in W}    \l \| \frac{1}{m} \sum_{i=1}^{m} e_i \nabla_w l(w,x_i)\r \|_2 \r],
\label{eq:emp rademach}
\end{align}
is the \emph{empirical Rademacher complexity} and $E=\{e_i\}_i$ is a Rademacher sequence, namely, a sequence of independent random variables taking $\pm 1$ with equal probabilities.  We can now revisit~\eqref{eq:before_rademacher} and write that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le 4\a^2 (1-\eta_\rho)^t \Delta_0 + \frac{2\a^2 \ol{\eta}_\rho}{\rho}  + \frac{2\a^2\Upsilon_{m,W}^2(\varepsilon)}{\zeta_L^2},
\end{align}
which holds except with a probability of at most $e^{-\varepsilon}$. In addition, for every $w,w'\in W$, we may write that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \le   \| \nabla L(w) - \nabla L(w')\|_2+ \| \nabla L_m(w) - \nabla L(w) \|_2\nonumber\\
& \qquad  + \| \nabla L_m(w') - \nabla L(w')\|_2
\quad \text{(triangle inequality)} \nonumber\\
& \le  \s_L\|w-w'\|_2+  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx_supp},\ref{eq:emp_proc}))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. 
Likewise, for every $w,w'\in W$, we have that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \ge \| \nabla L_m(w) - \nabla L_m(w) \|_2  -  \| \nabla L_m(w) - \nabla L(w)\|_2\nonumber\\
& \qquad - \| \nabla L_m(w') - \nabla L(w')\|_2
\qquad \text{(triangle inequality)} \nonumber\\
& \ge  \zeta_L\|w-w'\|_2-  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx_supp},\ref{eq:emp_proc} ))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. Therefore, $L_m$ satisfies the restricted strong convexity and smoothness in Definition~\ref{defn:Lm_scvx} with
\begin{align}
\mu_L = \s_L,
\qquad 
\nu_L = \zeta_L,
\nonumber\\
\ol{\mu}_L = \ol{\zeta}_L =  2\Upsilon_{m,W}(\varepsilon). 
\end{align}
%Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold. These findings are summarized below in our second main result.  For a convex set $W\subset\R^p$, let  $R=1_W$  be the (convex) indicator function on $W$ and set $H=0$ in ~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of ~(\ref{eq:emp loss min}) satisfies $w^*\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ is the relative interior of the set $W$.  
Our findings in this section are summarized below. 
\begin{theorem} \label{thm:main_stat}\textbf{\emph{(generalization error)}} 
Suppose that Assumptions~\ref{assump:G_ssmth}-\ref{assump:risk_supp} hold and recall that the training samples $\{x_i\}_{i=1}^m$ are drawn independently from the probability space $(\mathbb{X},\chi)$ for a compact set $\mathbb{X} \subset \R^d$  with diameter $\operatorname{diam}(\mathbb{X})$.   

For a set $W\subset\R^p$, let  $R=1_W$  be the indicator function on $W$, and set $H\equiv 0$ in ~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of ~(\ref{eq:emp loss min}) belongs to the relative interior of $W$. 
For $\varepsilon>0$, evaluate the quantities in Theorem~\ref{thm:main-stat-learn} with 
\begin{align}
\mu_L & = \s_L,
\qquad 
\nu_L = \zeta_L, \nonumber\\
\ol{\mu}_L & = \ol{\zeta}_L =   
4 \mathcal{R}_W(x_1,\cdots,x_m) \nonumber\\
& \qquad +6\s_l\operatorname{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}},
\end{align}
where $\mathcal{R}_W(x_1,\cdots,x_m)$ in the empirical  Rademacher complexity defined in (\ref{eq:emp rademach}). If the requirements on the step sizes in~(\ref{eq:step_size_reqs_thm}) hold, we then have that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le   4\a^2(1-\eta_\rho)^t \Delta_0 + \frac{2\a^2 \ol{\eta}_\rho}{\rho}+ \frac{8\a^2 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2  \nonumber\\
& \qquad +  \frac{18\a^2\s_l^2 \operatorname{diam}(\mathbb{X})^2( \varepsilon+2)}{m}, 
\end{align}
except with a probability of at most $e^{-\varepsilon}$. 
\end{theorem}
Most of the remarks about Theorem~\ref{thm:main} also apply to Theorem~\ref{thm:main_stat} and we note that $\|w_t-w^\n\|_2$ reduces by increasing the number of training samples $m$, before asymptotically reaching the generalization error
\begin{align}
2\psi_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2.
\label{eq:statistical ball}
\end{align}
Computing the Rademacher complexity above for specific choices of the network structure and loss is itself potentially a complicated task, which we will not pursue by the virtue of the generality of our results so far. The key technical challenge there is computing the corresponding \emph{entropy integral}, which involves estimating the \emph{covering numbers} of the set $W$ \cite{mohri2018foundations}. One last takeaway point from the statistical accuracy in \eqref{eq:statistical ball} is the following. If  
\begin{align}
\ol{\eta}_\rho =O(\rho \cdot \mathcal{R}_W(x_1,\cdots,x_m)^2/\zeta_L^2),
\label{eq:statistacll ball 2}
\end{align}
the asymptotic optimization error  in Theorem~\ref{thm:main} does not play an important role in determining the generalization error above. In words, if  \eqref{eq:statistacll ball 2} holds, then Algorithm~\ref{alg:admm} converges to the ball of statistical accuracy around $w^\n$. Here, $O$ stands for the standard Big-O notation. 






==> neurips2019 copy/sections/proposition.tex <==
The feedforward network $G=G_\Xi:\R^s
\to \R^d$ is a composition of linear maps and entry-wise applications of
the activation functions, and hence is also of class $C^1$. Its Jacobian $DG:\R^s \to \R^{d \times s}$
is thus a continuous function and its restriction
to the compact subset $\Dom \subseteq \R^s$ is Lipschitz-continuous. Therefore, there exists
$\nu_G \geq 0$ such that
\[
    \norm{DG(z') - DG(z)}_2 \leq \nu_G \norm{z'-z}, \qquad \forall z, z' \in \Dom.
\]
From standard arguments it then follows that Assumption \ref{assump:G_ssmth} holds in the sense that 
\begin{align*}
\norm{G(z') - G(z) - DG(z)(z'-z)}_2 &= \norm{\int_{0}^1 (DG(tz' + (1-t)z) - DG(z))(z'-z) dt}_2 \\
&\leq \int_{0}^1 \norm{DG(tz' + (1-t)z) - DG(z)}_2 \norm{z' - z}_2 dt \\
&\leq \nu_G \int_0^1 t\norm{z' - z}^2 dt = \dfrac{\nu_G}{2} \norm{z'-z}_2^2,
\end{align*}
for every $z,z'\in \R^s$. 

In order to show that Assumption \ref{defn:G_iso} (near-isometry) also holds, we will require the following simple fact:

\begin{lemma}
\label{lem:inv_lips}
Let $G:\Dom \subseteq \R^s \to \R^d$ have a left inverse $H:G(\Dom) \subseteq \R^d \to \R^s$
which is Lipschitz-continuous with constant $\iota_G > 0$. Then  it holds
that
\[
    \dfrac{1}{\iota_G} \norm{z'-z} \leq \norm{G(z') - G(z)},
    \qquad \forall z', z \in \D.
\]
\begin{proof}
\[
\norm{z' - z} = \norm{H(G(z')) - H(G(z))} \leq \iota_G \norm{G(z') - G(z)}. 
\]
\end{proof}
\end{lemma}
We now proceed to show that Assumption \ref{defn:G_iso} holds. We suppose $G$ is of the form
\[
    G(z) = \omega_k W_k (\omega_{k-1} W_{k-1}\ldots (\omega_1 W_1 z)\ldots),
\]
for weight matrices $\{W_k\}_k$. 
First note that, by the compactness of the domain of $G$, 
the values of the hidden layers are always contained in a product of compact
intervals, and so we can replace $\omega_i$ by its restriction to such sets.
Each $\omega_i$ is continuous, defined on a product of intervals, and
is stricly increasing so that they have a continuous left inverse $\omega_i^{-1}$
\citep[Proposition 6.4.5]{garling_2014}. The
assumption of non-decreasing layer sizes implies that the $W_i$ are tall
matrices of dimensions $(m_i, n_i)$ with $m_i \geq n_i$, whose columns are
almost surely linearly independent after an arbitrarily small perturbation. In such case they have a
left matrix inverse $W_i^{-1}$, which as a {bounded} linear map, is continuous.
It then follows that $G$ has a continuous left inverse of the form
\[
    G^{-1}=W_1^{-1} \circ \omega_1^{-1} \ldots W_k^{-1} \circ \omega_k^{-1},
\]
which is a continuous mapping and is defined on $G(\Dom)$ which by continuity
of $G$ is compact, hence $G^{-1}$ is Lipschitz-continuous. The result then
follows by the Lipschitz continuity of the map $G$ (restricted to the compact domain $\Dom$)
and Lemma \ref{lem:inv_lips}. 


==> neurips2019 copy/sections/related_work.tex <==
\cite{Bora2017}  empirically tune gradient descent for compressive sensing with a
{generative prior}  
\begin{align}
 \underset{z}{\min}\,\,
 \norm{A\cdot G(z)-b}^2_2, 
 %\qquad b:=Aw^\natural + \eta
\label{eq:intro_pr2}
\end{align}
which is a particular case of
template \eqref{eq:emp loss min} (without splitting). They also provide a
statistical generalization error dependent on a certain \textit{set restricted isometry property}
on the matrix $A$. More generally, Theorem \ref{thm:main_stat}
in Supplementary~\ref{sec:statLearn} provides statistical guarantees for
Algorithm \ref{alg:admm} using the standard  notion of empirical Rademacher
complexity~\citep{mohri2018foundations}.
%
%Despite the success of first order methods like
%gradient descent in minimizing such objective, much of the literature regarding
%this problem has focused on the statistical guarantees of either an exact or
%approximate solution of \eqref{eq:intro_pr2}. Theorem 1.1 and 1.2 in
%\citet{Bora2017} exploit the Lipschitzness of the generator $G$ and a certain
%\textit{set-restricted eigenvalue condition} to derive sample complexity
%estimates for the approximate recovery of the underlying true signal
%$w^\natural$. In stark contrast our derived statistical guarantee
%\ref{thm:main2} is given in terms of the standard statistical notion of
%empirical Rademacher complexity \citep{mohri2018foundations}, moreover such
%generalization bounds are given for the iterates of our algorithm
%\ref{alg:admm}.

\citet{hand2017global} analyze the optimization landscape of
\eqref{eq:intro_pr2} under the assumption that $G$ $(i)$ is composed of linear
layers and ReLU activation functions, $(ii)$ is sufficiently expansive at each
layer and $(iii)$ the network's weights have a Gaussian distribution or an
equivalent deterministic \textit{weight distribution condition}. Under such
conditions, they show global existence of descent directions outside small
neighborhoods around two points, but do not provide algorithmic convergence rates.  Their analysis requires ReLU activation in all layers of the
generator $G$, including the last one, which is  often not met in practice.
%whereas the common
%GANs trained in practice use sigmoid or Tanh.

On the other hand, our framework is not restricted to a particular network
architecture and instead isolates the necessary assumptions on the network $G$
for the success of Algorithm~\ref{alg:admm}. In doing so, we effectively
decouple the learning task from the network structure $G$ and study them
separately in Theorem \ref{thm:main} and Proposition \ref{pr:G-assumptions},
respectively. In particular, our theory in Section~\ref{sec:guarantees1} 
(Supplementary~\ref{sec:statLearn}) applies broadly to any nonlinear map $G$ that
meets Assumptions~\ref{assump:risk}-\ref{defn:G_iso} (Assumptions~\ref{assump:G_ssmth}-\ref{assump:risk_supp}), respectively. In turn, Proposition~\ref{pr:G-assumptions} establishes that the standard feed forward network with
common differentiable activation functions almost surely meets these assumptions. In this sense, let us also point to the work of~\citet{oymak2018sharp}, which is limited to linear regression with a nonlinear constraint, with its convex analogue studied
in~\citep{agarwal2010fast,giryes2016tradeoffs}. 

\citet{Heckel2019} provides a convergence proof for a modified version of
gradient descent, limited to \eqref{eq:intro_pr2} and without specifying a rate. We provide
the convergence rate for a  broad range of learning problems, and study the
statistical generalization. \citet{Hand2018} studied the \textit{phase
retrieval} problem, with a non-convex objective function that is not directly
covered by  \eqref{eq:emp loss min}. 

For the problem \eqref{eq:intro_pr2}, \citet{Shah2018, Hegde2018} proposed to
use Projected Gradient Descent (PGD) after splitting in a manner similar to our
template \eqref{eq:emp loss min}. If the projection (onto the range of the
prior $G$) is successful, and under certain additional conditions, the authors
establish linear convergence of PGD to a minimizer of \eqref{eq:intro_pr2}.
However, the projection onto the nonlinear range of $G$ is itself a
difficult non-convex program without any theoretical guarantees. In contrast,
we can solve the same problem without any projections while still providing a
convergence rate.

From an optimization perspective, there are no fast rates for linearized ADMM
with nonlinear constraints to our knowledge, but convergence to a first-order
stationary point and special cases in a few different settings have been
studied~\citep{liu2017linearized,shen2016square,chen2014convergence,qiao2016linearized}.
Let us again emphasize that
Assumptions~\ref{assump:G_ssmth}~and~\ref{defn:G_iso} extract the key
attributes of $G$ necessary for the success of Algorithm \ref{alg:admm}, which
is therefore not limited to a generator network.  It is also worth noting
another line of work that applies tools from statistical physics to inference
with deep neural networks, see~\citep{manoel2017multi,rezende2014stochastic}
and the references therein.


==> neurips2019 copy/sections/relations.tex <==
This section uncovers the relation between several first-order algorithms that have been proposed in the literature to solve Program~\eqref{eq:emp loss min}. Loosely speaking, we will establish that Algorithm~\ref{alg:admm} is closely related to previous algorithms, and that our convergence analysis in Section~\ref{sec:guarantees1} also applies to the algorithm proposed in \cite{Bora2017} without rates. We caution the reader that the discussion in this section is less formal by its nature. 

Let us now turn to the details. 
Throughout this section, we set $R=H=0$ in Program~\eqref{eq:emp loss min} since the current literature for deep-net priors in unable to provably and efficiently handle nonsmooth regularizers, to the best of our knowledge, unlike Algorithm~\ref{alg:admm}. Instead of the (linearized) updates in Algorithm~\ref{alg:admm}, consider the updates 
\begin{equation}
\begin{split}
    z_{ t+1} &=  z_{ t} - \b \grad_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) , \\
    w_{ t+1} &\in \underset{w}{\operatorname{argmin}} \,\, \Lagr_\rho(w,z_{t+1},\lambda_t), \\
    \lambda_{t+1} &= \lambda_{ t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1})).
\end{split}
\label{eq:aug lagr alg full}
\end{equation}
From \eqref{eq:defn_aug_lagr}, recall that $\Lagr_\rho(w,z,\lambda)$ is convex in $w$ and the second step in \eqref{eq:aug lagr alg full} is therefore often easy to implement  with any over-the-shelf standard convex solver. 
 Recalling~(\ref{eq:defn_aug_lagr}), note also that the optimality condition for $w_{t+1}$ in \eqref{eq:aug lagr alg full} is  
\begin{align}
w_{t+1} - G(z_{t}) & = -\frac{1}{\rho}(\nabla L_m(w_{t+1})+ \lambda_t).
\label{eq:feas_to_grads}
\end{align}
Using \eqref{eq:defn_aug_lagr} again, we also write that 
\begin{align}
& \nabla_z \Lagr_\rho(w_{t+1},z_t,\lambda_t) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t +\rho (w_{t+1}-G(z_t)) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t  - \lambda_{t-1}- \nabla L_m(w_t)  ) \nonumber\\
& = - DG(z_t)^\top  ( \s_t (w_t - G(z_t)) - \nabla L_m(w_t)  ) ,
\end{align}
where the last two lines above follow from (\ref{eq:feas_to_grads},\ref{eq:aug lagr alg full}), respectively. When $t\gg 1$, the choice of dual step sizes in Algorithm~\ref{alg:admm} satisfies $\s_t\|w_t - G(z_t)\|_2 \approx 0$. Therefore, the $z$ update in \eqref{eq:aug lagr alg full} simplifies to 
\begin{align}
z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(w_t),
\label{eq:z_approx}
\end{align}
provided that $G$ is sufficiently smooth. 
In addition, when $\rho \gg 1$, the $w$ update in \eqref{eq:aug lagr alg full} ensures that $w_t \approx G(z_t)$ which, together with \eqref{eq:z_approx},  implies that 
\begin{align}
z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(G(z_t)), 
\label{eq:grad_step}
\end{align}
if the  prior $G$ and empirical loss $L_m$ are sufficiently smooth. Note that \eqref{eq:grad_step} corresponds to one step of gradient descent (GD) with step size $\b$ applied to the program 
\begin{align}
\min_z \,\,L_m(G(z)),
\label{eq:parameter_space}
\end{align}
which is equivalent to Program~\eqref{eq:emp loss min} with $R=H=0$. That is, for a sufficiently large penalty weight, the updates in \eqref{eq:aug lagr alg full} approximately coincide  with those in GD applied to  Program~\eqref{eq:parameter_space}. Since the updates in \eqref{eq:aug lagr alg full} can only improve over Algorithm~\ref{alg:admm}, the convergence rate in Section~\ref{sec:guarantees1} also applies to GD for Program~\eqref{eq:parameter_space}, thereby providing convergence rate as a special case for the algorithm introduced in~\citet{Bora2017} without supporting theory. 


The next observation highlights the relation between GD in \eqref{eq:grad_step} (with exact equality therein) and the Projected Gradient Descent (PGD) applied to Program~\eqref{eq:emp loss min}. Indeed, with  the step size $\alpha_{\operatorname{pgd}}>0$, an iteration of PGD is specified as 
\begin{align}
w_{t+1} & \in  \Proj_G(w_t - \a_{\operatorname{pgd}} \nabla L_m(w_t) ) \nonumber\\
& = \Proj_G( G(z_t) - \alpha_{\operatorname{pgd}} \nabla L_m(G(z_t)) ), 
\label{eq:PGD update}
\end{align}
where the possibly set-valued operator $\Proj_G:\R^p\rightarrow\R^p$ denotes the projection onto the  prior, taking $w\in \R^p$ to 
\begin{align}
\Proj_G(w) & = 
\underset{z}{\operatorname{argmin}}\,\, \frac{1}{2}\| w - G(z)\|^2_2,
\label{eq:proj_gan}
\end{align}
and $z_t$ satisfies $w_t = G(z_t)$. 
Program~\eqref{eq:proj_gan} can be solved numerically by GD, for instance, to first-order stationarity. Initialized at $z_t$ and with the step size of $\alpha_{\operatorname{proj}}>0$,  the first iterate of gradient descent for computing $w_{t+1}$ in \eqref{eq:PGD update}  takes $z_t$ to 
\begin{align}
z_t - \alpha_{\operatorname{proj}} \alpha_{\operatorname{pgd}} DG(z_t)^\top 
 \nabla L_m (G(z_t)), 
\end{align}
which coincides with the right-hand side of \eqref{eq:grad_step} with the choice of $\b= \alpha_{\operatorname{proj}}\alpha_{\operatorname{pgd}}$. That is, the first iterate of PGD for solving Program~\eqref{eq:emp loss min} matches the first GD update for Program~\eqref{eq:parameter_space}.



==> neurips2019 copy/sections/setup.tex <==
For the sake of completeness, in this section we provide a more detailed problem formulation, which follows the standard setup in learning theory~\cite{mohri2018foundations}. 
Consider the probability space $(\mathbb{X}, \chi)$, where
$\mathbb{X} \subset \R^d$ is a compact set, equipped with the Borel sigma
algebra, and $\chi$ is the corresponding probability measure. To learn an
unknown parameter $w^\n \in \R^d$, consider the optimization program
\begin{align}
\underset{w\in \R^p}{\text{min}} \,\,  L(w),
\qquad
L(w) := \E_{x \sim \chi} l(w,x),
\label{eq:pop loss min}
\end{align}
where $L:\R^p\rightarrow \R$ is the differentiable \textit{population risk}
and $l:\R^d \times \R^p \rightarrow\R$ is the corresponding \emph{loss function}. We
also assume that Program \eqref{eq:pop loss min} has a unique solution $w^\n\in
\R^p$. The probability measure $\chi$ above is itself often unknown and we instead
have access to $m$ samples drawn independently from $\chi$, namely,
$\{x_i\}_{i=1}^m \sim \chi$. This allows us to form the \emph{empirical loss}
\begin{align}
L_m(w) := \frac{1}{m} \sum_{i=1}^m l(w,x_i).
\label{eq:emp loss defn supp}
\end{align}
Often, $m \ll p$ and to avoid an ill-posed problem, we must leverage any
inherent structure in $w^\n$. In this work, we consider a differentiable map
$G: \R^s \to \R^d$ and we assume that $w^\n \in G(\R^s)$.  That is,
there exists $z^\n \in \R^s$ such that $w^\n = G(z^\n)$. While not necessary, we limit ourselves in this paper to the important case where $G$ corresponds to a deep neural network, a GAN for instance. 

The defferentiability assumption on $G$ is not
restrictive. For example, the non-differentiable ReLU activation function in a GAN can be  replaced with its smooth alternative ELU \citep{clevert2015fast}, which only differs
 from ReLU near the origin. In our experiments, we were able to succesfully train GANs with ELU activation function. \citet{gulrajani2017improved} also reports
successful training of GANs with another differentiable activation function. See also the discussion after Assumption~\ref{assump:G_ssmth}. 

To learn $w^\n$ with the deep-net prior $w^\n=G(z^\n)$,  we propose
to solve the program
\begin{align}
\begin{array}{lll}
\underset{w,z}{\text{minimize}} & & L_m(w) + R(w) + H(z)\\
\text{subject to } & & w = G(z),
\end{array}
\label{eq:emp loss min supp}
\end{align}
where $R:\R^p \rightarrow \R$ and $H: \R^s \rightarrow \R$ are convex but not
necessarily smooth. Depending on the specific problem at hand, the \emph{regularizers}
$R$ and $H$ allow us to impose  additional structure on $w$ and
$z$, such as sparsity or set inclusion. Throughout, we only require that
the \emph{proximal maps} \citep{Parikh2014} for $R$ and $H$ can be computed
efficiently, as detailed in Section \ref{sec:algorithm}. Several examples of
this broad learning framework are discussed in Section \ref{sec:experiments},
including \emph{compressive sensing} with deep-net priors.

%\subsection{\edita{Empirical Risk }Minimization}
%\label{sec:error_min}
%\notea{Changing $x$ to $u$ for parameter. $u$ could be the labels, could be the image itself. This is to cover the general learning with GAN prior rather than just inverse problems.}
%We consider the optimization problem
%\begin{equation}
%\begin{array}{llll}
%& \underset{\up}{\text{minimize}}
%& & \loss(\up) \\
%& \text{subject to}
%& & \up \in \bigcup_{k=1}^K G_k(\Sprior)
%\end{array}
%\label{eq:problem_general}
%\end{equation}
%where we assume that the objective function $\loss$ as well as each $G_k$ for
%$k \in [K]$ are differentiable. The measurement error minimization problem
%corresponds to $\loss(\up)=\norm{A\up - b}_2^2$.  
%Finally, each constraint of the form $\up_k \in G_k(\Sprior)$ can be rewritten as
%$\up_k = G_k(\prior_k)$ for every $ \prior_k \in \Sprior$. 
%Writing $\Prior=[\prior_1, \ldots,
%\prior_K]$ we arrive at the optimization problem


==> neurips2019 copy/sections/stat_guarantees_main_body.tex <==
Building upon the results in Section~\ref{sec:guarantees1}, the main result in
this section (Theorem \ref{thm:main_stat}) quantifies the convergence of the
iterates $\{w_t\}_{t\ge 0}$ of Algorithm~\ref{alg:admm} to the true parameter
$w^\n$.

In other words, Theorem~\ref{thm:main_stat_body} below controls the generalization
error of Program~\eqref{eq:emp loss min}, namely, the error  incurred by using
the empirical risk $L_m$ in lieu of the population risk $L$. Indeed,
Theorem \ref{thm:main} is silent about $\|w_t - w^\n\|_2$. Our findings in this
section are summarized below.
\begin{theorem}
\label{thm:main_stat_body}
\textbf{\emph{(Generalization error) }}
Suppose that Assumptions \ref{defn:Lm_scvx}-\ref{defn:G_iso} hold and recall
that the training samples $\{x_i\}_{i=1}^m$ are drawn independently from the
probability space $(\mathbb{X},\chi)$ for a compact set $\mathbb{X} \subset
\R^d$ with diameter $\operatorname{diam}(\mathbb{X})$.

For a set $W\subset\R^p$, let  $R=1_W$  be the indicator function on $W$, and
set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of
Program \eqref{eq:emp loss min} belongs to the relative interior of $W$.
For $\varepsilon>0$, evaluate the quantities in Theorem \ref{thm:main} with
\begin{align}
    \mu_L = \s_L, \qquad&
    \nu_L = \zeta_L, \qquad &
\ol{\mu}_L = \ol{\zeta}_L =
4 \mathcal{R}_W(x_1,\cdots,x_m) +6 \s_l\operatorname{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}}
\end{align}
where $\mathcal{R}_W(x_1,\cdots,x_m)$ in the empirical  Rademacher complexity
defined in (\ref{eq:emp loss min}). If the requirements on the step sizes
in~(\ref{eq:step_size_reqs_thm}) hold, we then have that
\begin{align}
\|w_t- w^\n \|_2^2
\le   2\eta_{\rho}^t\widetilde{\Delta}_0 +
2\widetilde{\psi}_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2
+ \frac{18\s_l^2 \operatorname{diam}(\mathbb{X})^2( \varepsilon+2)}{m}
\end{align}
 except with a probability of at most $e^{-\varepsilon}$.
\end{theorem}
Most of the remarks about Theorem~\ref{thm:main} also apply to
Theorem~\ref{thm:main_stat} and we note that $\|w_t-w^\n\|_2$ reduces by
increasing the number of training samples $m$, before asymptotically reaching
the generalization error
\begin{align}
2\widetilde{\psi}_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2.
\label{eq:statistical ball_body}
\end{align}
Computing the Rademacher complexity above for specific choices of the network
structure and loss is itself potentially a complicated task, which we will not
pursue by the virtue of the generality of our results so far. The key technical
challenge there is computing the corresponding \emph{entropy integral}, which
involves estimating the \emph{covering numbers} of the set $W$
\cite{mohri2018foundations}. One last takeaway point from the statistical
accuracy in \eqref{eq:statistical ball_body} is the following. If
\begin{align}
\widetilde{\psi}_\rho=O(\mathcal{R}_W(x_1,\cdots,x_m)^2/\zeta_L^2),
\label{eq:statistacll ball 2_body}
\end{align}
the asymptotic optimization error  in Theorem~\ref{thm:main} does not play an
important role in determining the generalization error above. In words, if
\eqref{eq:statistacll ball 2_body} holds, then Algorithm \ref{alg:admm} converges to
the ball of statistical accuracy around $w^\n$. Here, $O$ stands for the
standard Big-O notation. An extended version of this section that includes the proof of Theorem~\ref{thm:main_stat_body} appears in the supplementary material. 


==> neurips2019 copy/sections/theory.tex <==
It is convenient throughout the supplementary material  to use a slightly different notation for Lagrangian, compared to the body of the paper. 
To improve the readability of the proof, let us  list here the assumptions on the empirical loss $L$ and prior $G$ that are used throughout this proof. For every iteration $t$, we assume that 
\begin{align}
& L(w_{t}) - L(\wh{w}) - \langle w_{t}-\wh{w} , \nabla L(\wh{w}) \rangle \nonumber\\
& \ge \frac{\mu_L}{2}\|w_{t}-\wh{w}\|_2^2 , 
\qquad \l(\text{strong convexity of }L  \r)
\label{eq:str cvx of L}
\end{align}
\begin{align}
& L(w_{t+1}) - L(w_{t}) - \langle w_{t+1}-w_{t} , \nabla L(w_{t}) \rangle  \nonumber\\
& \le \frac{\nu_L}{2}\|w_{t+1}-w_{t}\|_2^2 , 
\qquad \l(\text{strong smoothness of } L \r)
\label{eq:smoothness of L}
\end{align}
\begin{align}
& \| G(z') - G(z) - DG(z) \cdot (z'-z) \|_2 \nonumber\\
& \le \frac{\nu_G}{2} \|z'-z\|_2^2,
\qquad \l(\text{strong smoothness of } G\r)
\label{eq:smoothness of G} 
\end{align}
\begin{align}
{\iota}_G \|z' - z\|_2   \le  \|G(z') - G(z)\|_2 \le \kappa_G \|z'- z\|_2,
\qquad \l( \text{near-isometry of } G \r)
\label{eq:lipschitz of G 2}
\end{align}
%\begin{align}
%\|G(z')-G(z)\|_2 \le \kappa_G \|z'-z\|_2+\ol{\kappa}_G,
%\qquad \l( \text{Lipschitz continuty of } G \r)
%\label{eq:lipschitz of G}
%\end{align}
\begin{align}
\|DG(z)\cdot (z'-z)\|_2 \le \kappa_G \|z'-z\|_2,
\qquad \l( \text{Lipschitz continuty of } G \r)
\label{eq:smoothness of G 2}
\end{align}
For the sake of brevity, let us set 
\begin{align*}
v = (w,z) \in \R^{p+s},
\end{align*}
\begin{align}
& \Lagr_\rho(v,\lambda) := \Lagr_\rho(w,z,\lambda)   := L(w) + R(w)+H(z)+ \langle w - G(z), \lambda \rangle \nonumber\\
& \qquad \qquad \qquad \qquad \qquad + \frac{\rho}{2}\|w-G(z)\|_2^2, 
\qquad \text{(augmented Lagrangian)}
\label{eq:ind Lagr}
\end{align}
\begin{align}
\Lagr_\rho'(v,\lambda) := \Lagr'_\rho(w,z,\lambda) = L(w)+\langle w - G(z),\lambda\rangle + \frac{\rho}{2}\|w-G(z)\|_2^2, 
\label{eq:ind Lagr prime}
\end{align}
\begin{align}
A(v) = A(w,z) := w - G(z).
\qquad \text{(feasibility gap)}
\label{eq:A_shorhtand}
\end{align}
Let also $v^*=(\wh{w},\wh{z})$ be a solution of \eqref{eq:emp loss min} and let $\wh{\lambda}$ be a corresponding optimal dual variable. The first-order necessary optimality conditions for \eqref{eq:emp loss min} are 
\begin{align}
\begin{cases}
- \nabla_v \Lagr'_\rho(\wh{v},\wh{\lambda}) \in \partial R(w^*)\times \partial H(z^*),\\
\wh{w} = G(\wh{z}),
\end{cases}
\label{eq:opt cnds}
\end{align}
where $\partial R(w^*)$ and $\partial H(z^*)$ are the  subdifferentials of $R$ and $H$, respectively, at $w^*$ and $z^*$.  
Throughout the proof, we will also often use the notation
\begin{align}
\Delta_{t} := \Lagr_\rho(v_{t},\lambda_{t}) - \Lagr_\rho(\wh{v},\wh{\lambda}), 
\label{eq:defn of Delta}
\end{align}
\begin{align}
\Delta'_t := \Lagr'_\rho(v_t,\lambda_t) - \Lagr'_\rho(v^*,\lambda^*),
\end{align}
\begin{align}
\delta_{t} := \| w_{t}-w^*\|_2,
\qquad 
\delta'_t := \| z_t - z^*\|_2,
\label{eq:defn of delta}
\end{align}
\begin{align}
A_{t} := A(v_t) = w_{t} - G(z_{t}).
\label{eq:defn of A}
\end{align}
In particular, with this new notation, the dual update can be rewritten as 
\begin{align}
\lambda_{t+1} = \lambda_t + \sigma_{t+1} A_{t+1}.
\qquad \text{(see Algorithm \ref{alg:admm})}
\label{eq:dual update proof}
\end{align}
First, in Appendix \ref{sec:smoothness}, we control the smoothness of $\Lagr'_\rho$ over the trajectory of the algorithm.
\begin{lemma}\label{lem:smoothness}
For every iteration $t$, it holds that 
\begin{align}
&  \Lagr'_\rho (w_{t+1},z_{t+1},\lambda_{t}) - \Lagr'_\rho (w_{t},z_{t+1},\lambda_{t}) - 
\langle w_{t+1}-w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t})  \rangle \nonumber\\
& \le \frac{\nu_\rho  }{2}\|w_{t+1}-w_t\|_2^2,
\label{eq:smoothness lemma w}
\end{align}
\begin{align}
& \Lagr'_\rho (w_{t},z_{t+1}\lambda_{t}) - \Lagr'_\rho (w_{t},z_{t},\lambda_{t}) - 
\langle z_{t+1}-z_{t}, \nabla_z \Lagr'_\rho(w_{t},z_{t},\lambda_{t})  \rangle \nonumber\\
& \le \frac{\xi_\rho }{2}\|z_{t+1}-z_t\|_2^2,
\label{eq:smoothness lemma z}
\end{align}
\begin{align}
\| \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \nabla_w \Lagr'_\rho(w_t,z_{t},\lambda_t)  \|_2 & \le \tau_\rho \|z_{t+1}-z_t\|_2^2 ,
\label{eq:smoothness lemma zw}
\end{align}
where 
\begin{align}
\nu_\rho := \nu_L+\rho.
\end{align}
\begin{align}
\xi_\rho  := \nu_G (\lambda_{\max}+\rho \max_i \|A_i\|_2 ) + 2\rho \kappa_G^2,   
\label{eq:xi rho bar raw}
\end{align}
\begin{align}
\tau_\rho := \rho \kappa_G.
\end{align}
\end{lemma}
Second, in the following result we ensure that $\Lagr_\rho$ and $\Lagr_\rho'$ are sufficiently regular along the trajectory of our algorithm, see  Appendix  \ref{sec:str cvx} for the proof. 
%, as a consequence of (\ref{eq:smoothness of L},\ref{eq:smoothness of G},\ref{eq:lipschitz of G 2}).
\begin{lemma}\label{lem:str cvx}
For every iteration $t$, it holds that 
\begin{align}
\Delta_{t} \ge \frac{\mu_\rho \d_t^2}{2} + \frac{\mu_\rho' \d_t'^2}{2}  - \ol{\mu}_\rho,
\label{eq:str cvx lemma 1}
\end{align}
\begin{align}
 \Delta'_{t}+ \langle v^* - v_{t} , \nabla_v \Lagr'_\rho (v_{t}) \rangle 
\le  \frac{\omega_\rho \d_t^2}{2} + \frac{\omega'_\rho \d_t^{'2}}{2},
\label{eq:smoothness lemma 2}
\end{align}
where 
\begin{align}
\mu_\rho :=  \mu_L - 2\rho,
\qquad 
\mu'_\rho := \frac{\rho \iota^2_G}{2}-\nu_G\|\lambda^*\|_2,
\end{align}
\begin{align}
\ol{\mu}_\rho := 
\frac{3}{\rho}\l( \lambda_{\max}^2 + \|\lambda^*\|_2^2\r), 
\end{align}
\begin{align}
\omega_\rho := 0,
\qquad 
\omega'_\rho :=
\frac{\nu_G  }{2} \l(\lambda_{\max}+ \rho   \r).
\end{align}
\end{lemma}
Having listed all the necessary technical lemmas above, we now proceed to prove Theorem \ref{thm:main}. Using the smoothness of $\Lagr'_\rho$, established in Lemma \ref{lem:smoothness}, we argue that 
\begin{align}
& \Lagr'_\rho(v_{t+1},\lambda_{t+1}) \nonumber\\
& = L(w_{t+1})+ \langle A_{t+1}, \lambda_{t+1} \rangle + \frac{\rho}{2}\| A_{t+1}\|_2^2 
\qquad \text{(see \eqref{eq:ind Lagr prime})}
\nonumber\\
& = L(w_{t+1})+ \langle A_{t+1}, \lambda_{t} \rangle + \l(\frac{\rho}{2}+ \sigma_{t+1} \r) \| A_{t+1}\|_2^2 
\qquad \text{(see \eqref{eq:dual update proof})}
\nonumber\\
& = \Lagr'_\rho(w_{t+1},z_{t+1},\lambda_{t}) +  \sigma_{t+1}  \| A_{t+1}\|_2^2 
\qquad \text{(see (\ref{eq:ind Lagr}))}
\nonumber\\
& \le \Lagr'_\rho (w_t,z_{t+1},\lambda_t) + \langle w_{t+1}-w_t, \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) \rangle +  \frac{\nu_\rho}{2}\|w_{t+1}-w_t\|_2^2 \nonumber\\
& \qquad + \ol{\nu}_\rho + \s_{t+1}\|A_{t+1}\|_2^2 
\qquad \text{(see (\ref{eq:smoothness lemma w}))}\nonumber\\
& \le \Lagr'_\rho (w_t,z_{t+1},\lambda_t) + \langle w_{t+1}-w_t, \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) \rangle +  \frac{1}{2\a}\|w_{t+1}-w_t\|_2^2\nonumber\\
& \qquad  + \ol{\nu}_\rho+ \s_{t+1}\|A_{t+1}\|_2^2  ,
\label{eq:proof 0}
\end{align}
where the last line above holds if the step size $\a$ satisfies 
\begin{align}
\a \le \frac{1}{\nu_\rho}.
\label{eq:first-step-size-assump}
\end{align}
According to Algorithm~\ref{alg:admm}, we can equivalently write the $w$ updates as 
\begin{align}
w_{t+1} = \arg\min_w \l\langle w - w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t})  \r\rangle + \frac{1}{2\a}\|w-w_{t} \|_2^2+ R(w).
\label{eq:equiv rep of w update}
\end{align}
In particular, consider above the choice of $w=\t w^*+(1-\t) w_t$ for $\t\in [0,1]$ to be set later. We can then bound the last line of \eqref{eq:proof 0} as 
\begin{align}
& \Lagr'_\rho(v_{t+1},\lambda_{t+1}) + R(w_{t+1}) \nonumber\\
& = \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t})  +  
\min_{w}  \langle w - w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t}) \rangle \nonumber\\
& \qquad +  \frac{1}{2\a}\|w-w_{t} \|_2^2 + R(w) + \sigma_{t+1} \|A_{t+1}\|_2^2
\qquad \text{(see (\ref{eq:proof 0},\ref{eq:equiv rep of w update}))}
 \nonumber\\
& \le \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t}) +  
\t \langle w^* - w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t}) \rangle
+  \frac{\t^2 \d_t^2}{2\a} \nonumber\\
& \qquad + \t R(w^*)+ (1-\t) R(w_t) + \sigma_{t+1} \|A_{t+1}\|_2^2 
\qquad (\text{convexity of } R  )\nonumber\\
& = \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t})  +  
 \t \langle w^* - w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t},\lambda_{t}) \rangle
+  \frac{\t^2\d_t^2}{2\a}\nonumber\\
& \qquad 
+ \t \langle w^* - w_t, \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \nabla_w \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle \nonumber\\
& \qquad + \t R(w^*)+ (1-\t) R(w_t) +  \sigma_{t+1} \|A_{t+1}\|_2^2 . 
\label{eq:proof 1}
\end{align}
The last inner product above can be controlled as 
\begin{align}
& \t \langle w^* - w_t , \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \nabla_w \Lagr'_\rho(w_t,z_{t},\lambda_t) \rangle  \nonumber\\
& \le \frac{\t^2 \d_t^2}{2\a} + \frac{\a}{2}\| \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \nabla_w \Lagr'_\rho(w_t,z_{t},\lambda_t)  \|_2^2 
\qquad ( 2\langle a, b\rangle \le \|a\|_2^2+\|b\|_2^2 \text{ and (\ref{eq:defn of delta})})
\nonumber\\
& \le \frac{\t^2\d_t^2}{2\a} +  \a \tau^2_\rho \|z_{t+1}-z_t\|_2^2,
\qquad \text{(see (\ref{eq:smoothness lemma zw}))}
\end{align}
which, after substituting in \eqref{eq:proof 1}, yields that 
\begin{align}
& \Lagr'_\rho(v_{t+1},\lambda_{t+1}) + R(w_{t+1})  \nonumber\\
& \le \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t}) +  
 \t \langle w^* - w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t},\lambda_{t}) \rangle
+  \frac{\t^2\d_t^2}{\a} \nonumber\\
& \qquad + \a\tau_\rho^2 \|z_{t+1}-z_t\|_2^2  + \t R(w^*) + (1-\t) R(w_t)+  \sigma_{t+1} \|A_{t+1}\|_2^2. 
\label{eq:proof 1.1}
\end{align}
Regarding the right-hand side above, the smoothness of $\Lagr'_\rho$ in Lemma \ref{lem:smoothness} allows us to write that 
\begin{align}
& \Lagr'_\rho(w_t,z_{t+1},\lambda_t)
+ \a\tau_\rho^2 \|z_{t+1}-z_t\|_2^2 
\nonumber\\
& \le \Lagr'_\rho(w_t,z_t,\lambda_t) + 
\langle z_{t+1}-z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t)\rangle \nonumber\\
& \qquad + 
\l( \frac{\xi_\rho}{2} + \a\tau_\rho^2  \r)
 \|z_{t+1}-z_t\|_2^2.
\qquad \text{(see (\ref{eq:smoothness lemma z}))} 
\label{eq:proof 1.2}
\end{align}
If we assume that the primal step sizes $\alpha,\b$ satisfy
\begin{align}
\frac{\xi_\rho}{2}+ \a\tau_\rho^2 \le \frac{1}{2\b},
\label{eq:step size assump}
\end{align}
we can simplify \eqref{eq:proof 1.2} as 
\begin{align}
& \Lagr'_\rho(w_t,z_{t+1},\lambda_t) + \a\tau_\rho^2 \|z_{t+1}-z_t\|_2^2  \nonumber\\
& \le \Lagr'_\rho(w_t,z_t,\lambda_t) + 
\langle z_{t+1}-z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t)\rangle +
\frac{1}{2\b} \|z_{t+1}-z_t\|_2^2 . 
\qquad \text{(see (\ref{eq:step size assump}))}
\label{eq:proof 1.3}
\end{align}
From Algorithm~\ref{alg:admm}, recall the equivalent expression of the $z$ updates as 
\begin{align}
z_{t+1} = \arg\min_z \langle z - z_t , \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle + \frac{1}{2\b}\|z-z_t\|_2^2 + H(z),
\label{eq:equiv_rep_of_z_updates}
\end{align}
and consider the choice of $z=\t z^* + (1-\t) z_t$ above, with $\t\in[0,1]$ to be set later.   Combining (\ref{eq:proof 1.3},\ref{eq:equiv_rep_of_z_updates}) leads us to 
\begin{align}
& \Lagr'_\rho(w_t,z_{t+1},\lambda_t ) + \a \tau_\rho^2 \|z_{t+1}-z_t\|_2^2 + H(z_{t+1})  \nonumber\\
& = \Lagr'_\rho(w_t,z_t,\lambda_t) + \min_z
\langle z - z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle + 
\frac{1}{2\b}\|z-z_t\|_2^2
+ H(z) 
\qquad \text{(see (\ref{eq:proof 1.3},\ref{eq:equiv_rep_of_z_updates}))}
\nonumber\\
& \le 
\Lagr'_\rho(w_t,z_t,\lambda_t) + 
\t \langle z^* - z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle + 
\frac{\t^2\d_t^{'2}}{2\b}
+ H(\t z^* + (1-\t) z_{t})
\nonumber\\
& 
\le \Lagr'_\rho(w_t,z_t,\lambda_t) + 
\t \langle z^* - z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle + 
\frac{\t^2 \d_t^{'2}}{2\b} \nonumber\\
& \qquad + \t H(z^*) + (1-\t) H(z_t) .
\qquad (\text{convexity of } H ) 
\label{eq:proof 1.4}
\end{align} 
By combining (\ref{eq:proof 1.1},\ref{eq:proof 1.4}), we reach 
\begin{align}
& \Lagr_\rho(v_{t+1},\lambda_{t+1}) \nonumber\\
& = \Lagr'_\rho(v_{t+1},\lambda_{t+1}) + R(w_{t+1}) + H(z_{t+1}) 
\qquad \text{(see (\ref{eq:ind Lagr},\ref{eq:ind Lagr prime}))}
\nonumber\\
& \le \Lagr'_\rho(w_t,z_{t+1},\lambda_t) +
\t \langle w^* - w_t, \nabla_w \Lagr'_\rho(w_t,z_t,\lambda_t) \rangle + \frac{\t^2\d_t^2}{\a} 
+ \a\tau_\rho^2\|z_{t+1}-z_t\|_2^2 \nonumber\\
& \qquad + \t R(w^*) +(1-\t) R(w_t) + H(z_{t+1}) + \s_{t+1}\|A_{t+1}\|_2^2  
\qquad 
\text{(see (\ref{eq:proof 1.1}))}  \nonumber\\
& \le \Lagr'_\rho(v_t,\lambda_t)+ \t \langle v^* - v_t, \nabla_z \Lagr'_\rho(v_t,\lambda_t) \rangle  + \frac{\t^2\d_t^2}{\a}  + \frac{\t^2\d_t^{'2}}{2\b} \nonumber\\
& \qquad  + \t R(z^*)+ (1-\t) R(z_t) + \t H(z^*) + (1-\t) H(z_t) \nonumber\\
& \qquad + \s_{t+1}\|A_{t+1}\|_2^2 
\qquad \text{(see (\ref{eq:proof 1.4}))} 
 \nonumber\\
& = \Lagr_\rho(v_t,\lambda_t) + \t \langle v^* - v_t, \nabla_z \Lagr'_\rho(v_t,\lambda_t) \rangle + \frac{\t^2\d_t^2}{\a}+  \frac{\t^2\d_t^{'2}}{2\b} 
\nonumber\\
&\qquad + \t (R(z^*) + H(z^*)- R(z_t) - H(z_t)  ) 
+ \s_{t+1}\|A_{t+1}\|_2^2 
\qquad \text{(see (\ref{eq:ind Lagr},\ref{eq:ind Lagr prime}))} \nonumber\\
& \le \Lagr_\rho(v_t,\lambda_t) + \t \l( \frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^{'2}}{2}-\Delta'_t  \r)  + \frac{\t^2 \d_t^2}{\a} + \frac{\t^2 \d_t^{'2}}{2\b}
\nonumber\\
& \qquad  
+ \t (R(z^*) + H(z^*)- R(z_t) - H(z_t)  ) 
+ \s_{t+1}\|A_{t+1}\|_2^2 
\qquad \text{(see \eqref{eq:smoothness lemma 2})}
\nonumber\\
& = \Lagr_\rho(v_t,\lambda_t) + \t \l( \frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^{'2}}{2}-\Delta_t  \r) + \frac{\t^2 \d_t^{2}}{\a} + \frac{\t^2  \d_t^{'2}}{2\b}  \nonumber\\
& \qquad + \s_{t+1}\|A_{t+1}\|_2^2 
\qquad \text{(see (\ref{eq:ind Lagr},\ref{eq:ind Lagr prime}))}
\label{eq:proof 1.45}
\end{align}
%where we conveniently defined the shorthand 
%\begin{align}
%\g := \min(\b,\a). 
%\end{align}
After recalling (\ref{eq:defn of Delta}) and by subtracting $\Lagr_\rho(v^*,\lambda^*)$ from both sides,  \eqref{eq:proof 1.45} immediately implies that 
\begin{align}
 \Delta_{t+1}  & \le \Delta_t 
 + \frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^{'2}}{2}+ 
 \t \l(  \ol{\omega}_\rho-\Delta_t  \r) 
+ \frac{\t^2 \d_t^2 }{\a} + \frac{\t^2 \d_t^{'2} }{2\b} \nonumber\\
& \qquad  + \s_{t+1}\|A_{t+1}\|_2^2 ,
 \quad \text{(see (\ref{eq:defn of Delta},\ref{eq:proof 1.45}))}
\label{eq:proof 1.5}
\end{align}
where we also used the assumption that $\t\le 1$ above. 
%Assuming that 
%\begin{align}
%\b < \frac{1}{\xi_\rho},
%\label{eq:step size z cnd}
%\end{align}
%Let us set 
%\begin{align}
%\t_0 = \sqrt{\frac{2\a\b\tau_\rho^2}{1-\b\xi_\rho}},
%\end{align}
%assuming that $\b < 1/\xi_\rho$. 
To remove the feasibility gap $\|A_{t+1}\|_2$ from the right-hand side above, we write that 
\begin{align}
\|A_{t+1}\|_2 & = \| w_{t+1}-G(z_{t+1})\|_2 
\qquad \text{(see \eqref{eq:defn of A})}
\nonumber\\
& = \| w_{t+1}- w^* - (G(z_{t+1}) - G(z^*)) \|_2 
\qquad ( (w^*,z^*) \text{ is a solution of \eqref{eq:emp loss min}} )
\nonumber\\
& \le  \|w_{t+1}-w^*\|_2 + \| G(z_{t+1}) - G(z^*)\|_2 
\qquad \text{(triangle inequality)}
\nonumber\\
& \le  \|w_{t+1}-w^*\|_2 + \kappa_G \| z_{t+1} - z^*\|_2 
\qquad \text{(see \eqref{eq:lipschitz of G 2})}
\nonumber\\ 
& = \d_{t+1} + \k_G \d'_{t+1},
\qquad \text{(see \eqref{eq:defn of delta})}
\label{eq:bnd-on-At}
\end{align}
which, after substituting in \eqref{eq:proof 1.5}, yields that 
\begin{align}
\Delta_{t+1}  & \le \Delta_t 
 + \frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^{'2}}{2}+ 
 \t \l(  \ol{\omega}_\rho-\Delta_t  \r) 
+ \frac{\t^2 \d_t^2 }{\a} + \frac{\t^2 \d_t^{'2} }{2\b}+ 2\s_{t+1}\d_{t+1}^2  + 2\s_{t+1}\k_G^2 \d'^2_{t+1} \nonumber\\
& \qquad  
\qquad (\text{see \eqref{eq:bnd-on-At} and } (a+b)^2\le 2a^2+2b^2)  \nonumber\\
& \le \Delta_t 
 + \frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^{'2}}{2}+ 
 \t \l(  \ol{\omega}_\rho-\Delta_t  \r) 
+ \frac{\t^2 \d_t^2 }{\a} + \frac{\t^2 \d_t^{'2} }{2\b} + 2\s_0 \d_{t+1}^2  + 2\s_0 \k_G^2 \d'^2_{t+1}. \nonumber\\
& \qquad  .
\qquad (\s_{t+1} \le \s_0 \text{ in Algorithm \ref{alg:admm}})
\label{eq:bnd-for-all-thetas}
\end{align}
For  every iteration $t$, suppose that 
\begin{align}
\frac{\d_t^2}{\a} + \frac{\d_t^{'2}}{\b}  \ge \ol{\eta}_\rho \ge 
\frac{\ol{\mu}_\rho  }{ \min\l( \frac{\a \mu_\rho }{4}, \frac{\b\mu'_\rho}{2}  \r) - \sqrt{\max\l(\frac{\a}{2}(\omega_\rho+4\s_0), \b (\omega'_\rho+4\s_0 \k_G^2)\r)}}
,
\label{eq:thresh}
\end{align}
for $\ol{\eta}_\rho$ to be set later. Consequently, it holds that 
\begin{align}
\frac{\Delta_t }{\frac{2\d_t^2}{\a}+ \frac{\d'^2_t }{\b}} & \ge \frac{\frac{\mu_\rho \d_t^2}{2}+ \frac{\mu'_\rho \d'^2_t}{2} - \ol{\mu}_\rho }{ \frac{2\d_t^2}{\a}+ \frac{\d'^2_t}{\b} }
\qquad \text{(see \eqref{eq:str cvx lemma 1})} \nonumber\\
& \ge \min\l( \frac{\a\mu_\rho}{4}, \frac{\b\mu'_\rho}{2}  \r) - \frac{\ol{\mu}_\rho }{\frac{2\d_t^2}{\a}+ \frac{\d'^2}{\b}} \nonumber\\
&\ge  \min\l( \frac{\a\mu_\rho}{4}, \frac{\b\mu'_\rho}{2}  \r) - \frac{\ol{\mu}_\rho }{\ol{\eta}_\rho} 
\qquad \text{(see \eqref{eq:thresh})} 
\nonumber\\
& \ge \sqrt{\max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b (\omega'_\rho+4\s_0 \k_G^2)\r)}. 
\qquad \text{(see \eqref{eq:thresh})}
\label{eq:show-well-defn}
\end{align}
We now set 
\begin{align}
\widehat{\theta}_t := \min\l(  
\sqrt{
\frac{\Delta_t ^2}{\l( \frac{2\d_t^2}{\a} + \frac{\d'^2_t}{\b} \r)^2}
- \max\l( \frac{\a}{2}\l( \omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)}
, 1
 \r),
\label{eq:thetahat}
\end{align}
which is well-defined, as verified in  \eqref{eq:show-well-defn}. 
From (\ref{eq:show-well-defn},\ref{eq:thetahat}), it also immediately follows that 
\begin{align}
%\widehat{\theta}_t \in [\t_0,1],
 \widehat{\theta}_t \in [0,1], 
\qquad \forall t, 
\label{eq:range_of_theta}
\end{align}
\begin{align}
\Delta_t \ge0, \qquad \forall t,
\label{eq:admissible}
\end{align} 
which we will use later on in the proof. 
%where we use the convention that $[\t_0,1]=\{1\}$ if $\t_0 >1$. 
Consider first the case where $\widehat{\t}_t <1$. To study  the choice of $\theta = \widehat{\theta}_t$ in \eqref{eq:proof 1.5}, we will need the bound 
\begin{align}
& -\widehat{\t}_t\Delta_t + \widehat{\t}_t^2 \l( \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{2\b} \r)  \nonumber\\
& = - \sqrt{
\frac{\Delta_t ^4}{\l( \frac{2\d_t^2}{\a} + \frac{\d'^2_t}{\b} \r)^2}
- \Delta_t^2 \max\l( \frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)} \nonumber\\
& \qquad + \frac{ \Delta_t^2}{\frac{4\d_t^2}{\a}+ \frac{2\d'^2_t}{\b} } - \max\l(\frac{\a}{2}\l(\omega_\rho +4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r) \l( \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{2\b} \r) 
\qquad \text{(see \eqref{eq:admissible})}
\nonumber\\
& \le - \frac{\Delta_t^2}{\frac{4\d_t^2}{\a}+\frac{2\d'^2}{\b}} + \Delta_t  \sqrt{\max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)} \nonumber\\
& \qquad - \max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r) \l( \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{2\b} \r),
\label{eq:nec-calc}
\end{align}
where the inequality above uses $\sqrt{a-b}\ge \sqrt{a}-\sqrt{b}$. Substituting  \eqref{eq:nec-calc} back into \eqref{eq:bnd-for-all-thetas}, we reach 
\begin{align}
\Delta_{t+1} & \le \Delta_t - \frac{\Delta_t^2}{\frac{4\d_t^2}{\a}+\frac{2\d'^2}{\b}} + \Delta_t  \sqrt{\max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)} 
\qquad \text{(see (\ref{eq:bnd-for-all-thetas},\ref{eq:nec-calc}))}
\nonumber\\
& \le \Delta_t - \l( \min\l( \frac{\a\mu_\rho}{4}, \frac{\b\mu'_\rho}{2 } \r) - \frac{\ol{\mu}_\rho}{\ol{\eta}_\rho}  \r) \frac{\Delta_t }{2} \nonumber\\
& \qquad + \Delta_t  \sqrt{\max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)} 
\qquad \text{(see third line of \eqref{eq:show-well-defn} and (\ref{eq:admissible}))}
\nonumber\\
& \le  \l(1 - \min\l( \frac{\a\mu_\rho}{8}, \frac{\b\mu'_\rho}{4 } \r) + \frac{\ol{\mu}_\rho}{2\ol{\eta}_\rho}  +
\sqrt{\max\l(\frac{\a}{2}\l(\omega_\rho+4\s_0 \r), \b\l(\omega'_\rho+4\s_0 \k_G^2 \r)  \r)}
\r) \Delta_t  \nonumber\\
%& \qquad + \min\l( \frac{\a \mu_\rho}{8},\frac{\b\mu'_\rho}{4} \r) \ol{\omega}_\rho+\a \ol{\tau}^2_\rho + \ol{\nu}_\rho + \ol{\xi}_\rho  \nonumber\\
& =: \eta_{\rho,1} \Delta_t ,
\qquad 
\text{if } \Delta_t  < \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{\b}. 
\label{eq:contraction}
\end{align}
%
%
%
%we arrive at 
%\begin{align} 
%&  \Delta_{t+1}  - \a\ol{\tau}^2_\rho - \ol{\nu}_\rho 
%- \ol{\xi}_\rho
% \nonumber\\
%& \le \Delta_{t} - 
%\frac{ (\Delta_{t}  - \ol{\omega}_\rho)^2}{\frac{2\d_t^2}{\a}+ \frac{2\d_t^{'2}}{\b}  } 
%\qquad \text{(see \eqref{eq:proof 1.5})} 
%\nonumber\\
%& \le \Delta_{t} +  \frac{\omega_\rho \d_t^2}{2}  +  \frac{\omega'_\rho \d_t^{'2}}{2} 
%- \frac{ \Delta^2_{t}}{\frac{4\d_t^2}{\a}+ \frac{4\d_t^{'2}}{\b}} 
%+ \frac{ \ol{\omega}_\rho^2}{\frac{2\d_t^2}{\a}+ \frac{2\d_t^{'2}}{\b}} 
%\qquad \l( (a-b)^2 \ge \frac{a^2}{2}-b^2 \r) \nonumber\\
%& \le  \Delta_{t} 
% +  \frac{\omega_\rho \d_t^2}{2}  +  \frac{\omega'_\rho \d_t^{'2}}{2} 
%- 
%\frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{ \frac{\delta_t^2}{\a}+ \frac{\delta_t^{'2}}{\b} }  \r) 
%\Delta_t
%+ \frac{ \ol{\omega}_\rho^2}{\frac{2\d_t^2}{\a}+ \frac{2\d_t^{'2}}{\b}} 
%\qquad \text{(see (\ref{eq:str cvx lemma 1},\ref{eq:admissible}))}
%\nonumber\\
%& \le  \Delta_{t} 
%+  \frac{\omega_\rho \d_t^2}{2}  +  \frac{\omega'_\rho \d_t^{'2}}{2} 
%- 
%\frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) 
%\Delta_t
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2}. 
%\qquad \text{(see (\ref{eq:thresh}))}
%\label{eq:delta'-to-be-removed}
%\end{align}
%To remove the feasibility gap $A_{t+1}$ from the first line above, let us assume that 
%\begin{align}
%\|A_t\|_2 \le \d_t, \qquad \forall t.
%\label{eq:feas-to-delta}
%\end{align}
%we write that 
%\begin{align}
%\|A_{t+1}\|_2^2 & = \| w_{t+1} - G(z_{t+1}) \|_2^2 \qquad \text{(see \eqref{eq:defn of A})} \nonumber\\
%& = \| w_{t+1} - G(z_{t+1}) - (w^* - G(z^*)) \|_2^2 
%\qquad ((w^*,z^*) \text{ is a solution of (\ref{eq:emp loss min})})
%\nonumber\\
%& = \| (w_{t+1} - w^*) - (G(z_{t+1}) - G(z^*))\|_2^2 \nonumber\\
%& \le 2 \|w_{t+1} - w^*\|_2^2 + 2 \|G(z_{t+1}) - G(z^*)\|_2^2 
%\qquad (\|a+b\|_2^2 \le 2\|a\|_2^2 + 2\|b\|_2^2)
%\nonumber\\
%& \le  2 \| w_{t+1} - w^* \|_2^2 + 2 (\kappa_G \| z_{t+1} - z^*\|_2^2 + \overline{\kappa}_G)^2 
%\qquad \text{(see \eqref{eq:lipschitz of G 2})} \nonumber\\
%& \le 2 \delta_{t+1}^2 + 4 \k_G^2 \d'^2_{t+1}  + 4 \ol{\k}_G^2. 
%\qquad ( \text{(\ref{eq:defn of A})  and } (a+b)^2 \le 2a^2 +2b^2)
%% \nonumber\\
%%& \le  2 \max\l( \frac{2}{\mu_\rho}, \frac{4\k_G^2}{\mu'_\rho}  \r) \l( \frac{\mu_\rho \d_{t+1}^2}{2}+ \frac{\mu_\rho' \d'^2_{t+1}}{2}    \r) + 4  \ol{\k}_G^2 \nonumber\\
%%& \le 4 \max\l( \frac{1}{\mu_\rho}, \frac{2\k_G^2}{\mu'_\rho}  \r) \l( \Delta_{t+1} + \ol{\mu}_\rho   \r) + 4  \ol{\k}_G^2,
%%\qquad \text{(see (\ref{eq:str cvx lemma 1}))} 
%\label{eq:feas-to-delta}
%\end{align}
%which, after substituting in \eqref{eq:delta'-to-be-removed}, yields that 
%\begin{align}
%\Delta_{t+1} & \le \l( 1- \frac{1}{8} \min (\mu_\rho \alpha, \mu'_\rho \beta) - \frac{2\ol{\mu}_\rho}{\psi_\rho^2} \r) \Delta_t + \frac{\omega_\rho\delta_t^2}{2}+ \frac{\omega_\rho'\delta'^2_t}{2} 
%+ 2 \d_{t+1}^2 + 4 \kappa_G^2 \d'^2_{t+1} 
%\nonumber\\
%& \qquad + \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2} + \alpha \ol{\tau}_\rho^2 + \ol{\nu}_\rho +\ol{\xi}_\rho+ 4\ol{\kappa}_G^2.
%\qquad \text{(see (\ref{eq:delta'-to-be-removed},\ref{eq:feas-to-delta}))}
%\end{align}
%To remove $\d_t$ and $\d'_t$ above, we write that 
%\begin{align}
%\frac{\omega_\rho \d_t^2}{2}+ \frac{\omega'_\rho \d_t^2}{2} & 
%\end{align}
%Let us now remove $\d'_t$  from the last line of \eqref{eq:delta'-to-be-removed}. Using the near-isometry property of $G$, we write that  
%\begin{align}
%\d'_t & = \| z_t - z^*\|_2
%\qquad \text{(see \eqref{eq:defn of delta})}
% \nonumber\\
%& \le \frac{\|G(z_t) - G(z^*)\|_2}{\iota_G} 
%\qquad \text{(see \eqref{eq:lipschitz of G 2})}
%\nonumber\\
%& \le \frac{\|w_t - G(z_t)\|_2}{\iota_G} +\frac{ \| w_t - w^*\|_2}{\iota_G} + \frac{\|w^*-G(z^*)\|_2}{\iota_G}
%\qquad \text{(triangle inequality)}
%\nonumber\\
%& =  \frac{\|A_t\|_2}{\iota_G} +\frac{ \d_t}{\iota_G} 
%\qquad ( \text{feasibility of } w^* \text{ and (\ref{eq:defn of delta})}) \nonumber\\
%& \le \frac{ 2\d_t}{\iota_G} .
%\qquad \text{(see \eqref{eq:feas-to-delta})}
%\label{eq:near-iso-used}
%\end{align}
%In the same spirit as \eqref{eq:thresh}, we assume for every $t$ that 
%\begin{align}
% \d_t \ge \psi'_\rho ,
% \label{eq:new_thresh}
%\end{align}
%for $\psi'_\rho$ to be set later, and suppose that $\psi'_\rho$ satisfies
%\begin{align}
%\psi'_\rho \ge \max_t \|A_t\|_2.
%\label{eq:slater_lin}
%\end{align} 
%Under \eqref{eq:slater_lin}, we may simplify \eqref{eq:near-iso-used} to read as 
%\begin{align}
%\d'_t & \le \frac{2\d_t + \ol{\iota}_G}{\iota_G},
%\qquad \text{(see (\ref{eq:near-iso-used},\ref{eq:new_thresh},\ref{eq:slater_lin}))}
%\label{eq:upp-bnd-delta'}
%\end{align}
%Above, we have replaced $A_{t+1}$ and $\d'_t$, respectively, with $\d_{t+1}$ and $\d_t$. In turn, $\d_{t+1}$ and  $\d_t$ above can be related back to $\Delta_t$ by noting that 
%\begin{align}
%\d_t^2 \le \frac{2}{\mu_\rho}(\Delta_t + \ol{\mu}_\rho ). 
%\qquad \text{(see \eqref{eq:str cvx lemma 1})}
%\label{eq:delta-to-Delta}
%\end{align}
%With (\ref{eq:feas-to-delta}-\ref{eq:delta-to-Delta}) at hand, we revisit \eqref{eq:delta'-to-be-removed} to write that 
%\begin{align}
%\Delta_{t+1} & \le \Delta_t + \frac{\omega_\rho \d_t^2}{2} + \frac{2 \omega'_\rho \d_t^2 }{\iota_G^2} - \frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) \Delta_t \nonumber\\
%& \qquad + \s_{t+1} \d_{t+1}^2 + \a \ol{\tau}_\rho^2 + \ol{\nu}_\rho + \ol{\xi}_\rho 
%+ \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2} \qquad \text{(see (\ref{eq:feas-to-delta},\ref{eq:delta-to-Delta}))} \nonumber\\
%& \le \Delta_t + \frac{ ( \omega_\rho \iota_G^2 + 4 \omega'_\rho ) \d_t^2}{2\iota_G^2} 
%- \frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) \Delta_t + \s_{t+1}\d_{t+1}^2 
%\nonumber\\
%& \qquad 
%+ \a \ol{\tau}_\rho^2 + \ol{\nu}_\rho + \ol{\xi}_\rho 
%+ \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2} \nonumber\\
%& \le \Delta_t +  \frac{  ( \omega_\rho \iota_G^2 + 4 \omega'_\rho ) (\Delta_t + \ol{\mu}_\rho)}{\iota_G^2 \mu_\rho} - \frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) \Delta_t \qquad \nonumber\\
%& \qquad + \frac{2\s_{t+1} }{\mu_\rho} (\Delta_{t+1} + \ol{\mu}_\rho )
%+  \a \ol{\tau}_\rho^2 + \ol{\nu}_\rho + \ol{\xi}_\rho 
%+ \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2}
%\qquad \text{(see \eqref{eq:delta-to-Delta})} \nonumber\\
%& = \l(1 - \frac{1}{8}\min(\mu_\rho \a,\mu'_\rho\b ) + \frac{\ol{\mu}_\rho}{4\psi_\rho^2} 
%+ \frac{\omega_\rho \iota_G^2 + 4\omega'_\rho}{\iota_G^2\mu_\rho}
% \r) \Delta_t + \frac{2\s_{t+1} \Delta_{t+1} }{\mu_\rho} \nonumber\\
%& \qquad  + \frac{2\s_{t+1}\ol{\mu}_\rho}{\mu_\rho} +  \a \ol{\tau}_\rho^2 + \ol{\nu}_\rho + \ol{\xi}_\rho 
%+ \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2} . 
%\label{eq:before-rearranging}
%\end{align}
%For a sufficiently small $\s_0$, we have that $\s_{t+1}\le \s_0 \le \rho/2$, see Algorithm \ref{alg:admm}. Taking this into account and rearranging \eqref{eq:before-rearranging}, we reach 
%\begin{align}
%\Delta_{t+1} & \le \l(1- \frac{\rho }{\mu_\rho}\r)^{-1} \Bigg(  \l(1 - \frac{1}{8}\min(\mu_\rho \a,\mu'_\rho\b ) + \frac{\ol{\mu}_\rho}{4\psi_\rho^2} 
%+ \frac{\omega_\rho \iota_G^2 + 4\omega'_\rho}{\iota_G^2\mu_\rho}
% \r) \Delta_t  \nonumber\\
%&  \qquad  + \frac{\rho\ol{\mu}_\rho}{\mu_\rho} +  \a \ol{\tau}_\rho^2 + \ol{\nu}_\rho + \ol{\xi}_\rho 
%+ \frac{\ol{\omega}_\rho^2}{2\psi_\rho^2} \Bigg)  \nonumber\\
%& =: {\eta}_{\rho,1} \Delta_t + \ol{\eta}_{\rho,1},
%\qquad \text{if } \Delta_t - \ol{\omega}_\rho < \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{\b}.
%\label{eq:contraction}
%\end{align}
%and, in turn, rewrite \eqref{eq:delta'-to-be-removed} as 
%\begin{align}
%& \Delta_{t+1} - \sigma_{t+1} \|A_{t+1}\|_2^2 - \a\ol{\tau}^2_\rho - \ol{\nu}_\rho 
%- \ol{\xi}_\rho 
%\nonumber\\
%& \le  \Delta_{t} 
%+  \frac{\omega_\rho \d_t^2}{2}  +  \frac{\omega'_\rho (2\d_t + \ol{\iota}_G)^2 }{2} 
%- 
%\frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) 
%\Delta_t
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} 
%\qquad \text{(see (\ref{eq:delta'-to-be-removed},\ref{eq:upp-bnd-delta'}))}
%\nonumber\\
%& \le    \l( 1 -  \frac{1}{8}\min(\mu_\rho\a, \mu'_\rho \b ) + \frac{\ol{\mu}_\rho }{4\psi_\rho^2 }  \r)\Delta_{t} 
%+  \frac{(\omega_\rho + 8\omega'_\rho )\d_t^2}{2}  
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} + \omega'_\rho \ol{\iota}_G^2 
%\qquad ( (a+b)^2 \le 2a^2 +2b^2) 
%\nonumber\\
%& \le  \l( 1 -  \frac{1}{8}\min(\mu_\rho\a, \mu'_\rho \b ) + \frac{\ol{\mu}_\rho }{4\psi_\rho^2 }   +  \frac{\omega_\rho + 8\omega'_\rho }{\mu_\rho} \r)\Delta_{t} 
%+  \frac{(\omega_\rho + 8\omega'_\rho ) \ol{\mu}_\rho}{\mu_\rho} 
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} + \omega'_\rho \ol{\iota}_G^2 
%\qquad \text{(see \eqref{eq:str cvx lemma 1})} \nonumber\\
%& =: \widetilde{\eta}_{\rho,1} \Delta_t + \frac{(\omega_\rho+8\omega'_\rho)\ol{\mu}_\rho}{\mu_\rho} 
%   + \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} + \omega'_\rho \ol{\iota}_G^2.
%\label{eq:proof 3}
%\end{align}
%
%
%\begin{align}
%&  \le \Delta_{t} 
%+ \frac{\omega_\rho \d_t^2 + \omega'_\rho \d_t^{'2}}{\mu_\rho\d_t^2 + \mu'_\rho\d_t^{'2}} 
%(\Delta_t + \ol{\mu}_\rho)
%- 
%\frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) 
%\Delta_t 
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2}  
%\qquad \text{(see \eqref{eq:str cvx lemma 1})}
%\nonumber\\
%&  \le \Delta_{t} 
%+ \frac{\omega_\rho  + \omega'_\rho \Phi_T}{\mu_\rho } 
%(\Delta_t + \ol{\mu}_\rho)
%- 
%\frac{1}{8} \l( \min(\mu_\rho\a, \mu'_\rho \b ) - \frac{2\ol{\mu}_\rho }{\psi_\rho^2 }  \r) 
%\Delta_t 
%+ \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2}  
%\qquad \text{(see \eqref{eq:slater})}
%\nonumber\\
%& = \l( 1 + \frac{\omega_\rho+\omega'_\rho \Phi_T}{\mu_\rho } 
%-\frac{1}{8} \min(\mu_\rho\a, \mu'_\rho \b ) + \frac{\ol{\mu}_\rho }{4\psi_\rho^2 }  
%   \r)\Delta_t + 
%   \frac{(\omega_\rho+\omega'_\rho\Phi_T)\ol{\mu}_\rho}{\mu_\rho} 
%   + \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2}  
%\nonumber\\
%& =: \widetilde{\eta}_{\rho,1} \Delta_t + \frac{(\omega_\rho+\omega'_\rho\Phi_T)\ol{\mu}_\rho}{\mu_\rho} 
%   + \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} .
%\label{eq:proof 3}
%\end{align}
%Substituting \eqref{eq:feas-to-delta} back into \eqref{eq:proof 3} yields that 
%\begin{align}
% \Delta_{t+1} 
%& \le \l(1 - 4 \s_{t+1} \max\l( \frac{1}{\mu_\rho}, \frac{2\k_G^2}{\mu'_\rho}  \r)  \r)^{-1} \nonumber\\
%& \qquad \cdot \l( \widetilde{\eta}_{\rho,1} \Delta_t+ \alpha  \overline{\tau}_\rho^2 + \overline{\nu}_\rho + \overline{\xi}_\rho  + 
%\frac{(\omega_\rho + 8 \omega'_\rho) \overline{\mu}_\rho}{\mu_\rho} +  \frac{\overline{\omega}_\rho^2}{2\psi_\rho^2} + \omega'_\rho \ol{\iota}_G^2 \r). 
%\end{align}
%
%
%The above bound also controls the feasibility gap at the iteration $t+1$. Indeed, note that 
%\begin{align}
% \frac{\rho}{2}\|A_{t+1}\|_2^2 & 
% \le \mathcal{L}_\rho(v_{t+1},\lambda_{t+1}) 
% \qquad \text{(see (\ref{eq:ind Lagr}))}
% \nonumber\\
%& = \Delta_{t+1}
%+  \mathcal{L}_\rho(v^*,\lambda^*) 
%\qquad \text{(see \eqref{eq:defn of Delta})} \nonumber\\
%& 
%\le \Delta_{t+1}
%\qquad 
%\text{(see (\ref{eq:ind Lagr},\ref{eq:defn of Delta},\ref{eq:admissible}))}
%\nonumber\\
%& \le 
%\widetilde{\eta}_{\rho,1}
%\Delta_t 
%+ \sigma_{t+1} \|A_{t+1}\|_2^2 +
%\a\ol{\tau}^2_\rho + \ol{\nu}_\rho 
%+ \ol{\xi}_\rho  + \frac{(\omega_\rho+4\omega'_\rho)\ol{\mu}_\rho}{\mu_\rho} 
%   + \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2} + \omega'_\rho \ol{\iota}_G^2
%\qquad \text{(see (\ref{eq:proof 3}))} \nonumber\\
%& =: \widetilde{\eta}_{\rho,1}
%\Delta_t + \s_{t+1}\|A_{t+1}\|_2^2 + \widehat{\eta}_{\rho,1}.
%\end{align}
%For sufficiently small $\sigma_0$, we have that $\sigma_{t+1}\le \sigma_0 \le \rho/2$, see Algorithm~\ref{alg:admm}. We can therefore simplify  the above bound as 
%\begin{align}
%\|A_{t+1}\|_2^2 \le \frac{2 \widetilde{\eta}_{\rho,1} }{\rho-2\sigma_{0}}
%\Delta_t + 
%\frac{2 \widehat{\eta}_{\rho,1} }{\rho-2\sigma_{0}}.\label{eq:proof 4} 
%\end{align}
%In turn, substituting \eqref{eq:proof 4} back into \eqref{eq:proof 3} yields that 
%\begin{align}
%\Delta_{t+1} & \le 
%\frac{\rho \widetilde{\eta}_{\rho,1} }{\rho-2\sigma_{0}}
%\Delta_t + 
%\frac{\rho \widehat{\eta}_{\rho,1} }{\rho-2\sigma_{0}}
%\qquad \text{(see (\ref{eq:proof 3},\ref{eq:proof 4}))}
%\nonumber\\
%& =: \eta_{\rho,1} \Delta_t + \ol{\eta}_{\rho,1},
%\qquad 
%\text{if } \Delta_t-\ol{\omega}_\rho  <  \frac{\d_t^2}{\a}+   \frac{\d_t^{'2}}{\b}. 
%\label{eq:contraction}
%\end{align}
Next consider the case where $\widehat{\theta}_t=1$. With the choice of $\theta = \widehat{\theta}_t=1$ in \eqref{eq:bnd-for-all-thetas}, we find that 
\begin{align}
\Delta_{t+1}  
& \le
 \l( \frac{\omega_\rho}{2} + \frac{1}{\a}+ \rho \r) \d_t^2 
+ \l( \frac{\omega'_\rho}{2} + \frac{1}{2\b}+ \rho \kappa_G^2 \r) \d'^2_t 
\qquad \text{(see \eqref{eq:bnd-for-all-thetas})}\nonumber\\
& \le \frac{1}{2} \l( 1+ \max\l(  \frac{\a}{2} (\omega_\rho +4\s_0)    , \b(\omega'_\rho+4\s_0 \kappa_G^2  ) \r) \r)\cdot  \l( \frac{2\d_t^2}{\a}+ \frac{\d'^2_t}{\b}  \r) \nonumber\\
& \le \frac{1}{2} \sqrt{ 1+ \max\l(  \frac{\a}{2} (\omega_\rho +4\s_0)    , \b(\omega'_\rho+4\s_0 \kappa_G^2  ) \r) } \Delta_t  
\qquad \text{(see \eqref{eq:thetahat})} \nonumber\\
& =: \eta_{\rho,2} \Delta_t ,
\qquad \text{if } \Delta_t \ge  \frac{\d_t^2}{\a}+ \frac{\d'^2_t}{\b}.
\label{eq:contraction 2} 
\end{align}
%Recalling \eqref{eq:feas-to-delta}, we may remove $A_{t+1}$ from the first line above and write that 
%\begin{align}
%\Delta_{t+1} & \le  \l(\frac{\omega_\rho}{2}+\frac{1}{2\alpha}+ \s_{t+1} \r) \delta_t^2 + 
%\l(\frac{\omega'_\rho}{2}+\frac{1}{2\b}\r) \delta_t^{'2} 
%+ \a\ol{\tau}_\rho^2 +\ol{\nu}_\rho + \ol{\xi}_\rho +  \ol{\omega}_\rho
%\nonumber\\
%& \le \max(\a\omega_\rho+1 +2\a\sigma_{t+1}, \b\omega'_\rho+1 ) \frac{\Delta_t}{2}
%+ \a\ol{\tau}_\rho^2 +\ol{\nu}_\rho + \ol{\xi}_\rho 
% + \ol{\omega}_\rho
%\qquad \text{(see \eqref{eq:thetahat})} \nonumber\\
%& =: \eta_{\rho,2} \Delta_{t} + \ol{\eta}_{\rho,2},
%\qquad
%\text{if } \Delta_t-\ol{\omega}_\rho  \ge   \frac{\d_t^2}{\a}+   \frac{\d_t^{'2}}{\b}. 
%\label{eq:contraction 2}
%\end{align}
%
%
%As before, the above bound also controls the feasibility gap, namely, 
%\begin{align}
%\|A_{t+1}\|_2^2 & 
%\le\max(\a\omega_\rho+1 , \b\omega'_\rho+1 )   \frac{\Delta_t}{\rho-2\sigma_{0}}  + 
%\frac{2 }{\rho-2\sigma_{0}} \l(  \a\ol{\tau}^2_\rho + \ol{\nu}_\rho  
%+ \ol{\xi}_\rho   +\ol{\omega}_\rho\r) , 
%\end{align}
%which, after substituting in \eqref{eq:proof 5}, yields that
%\begin{align}
%\Delta_{t+1} & \le  
%\max(\a\omega_\rho+1 , \b\omega'_\rho+1 )  \frac{\rho \Delta_t}{2(\rho-2\sigma_0)} + \frac{\rho }{\rho-2\sigma_{0}} \l(  \a\ol{\tau}^2_\rho + \ol{\nu}_\rho  
%+ \ol{\xi}_\rho   +\ol{\omega}_\rho \r) \nonumber\\
%& =: \eta_{\rho,2} \Delta_{t} + \ol{\eta}_{\rho,2},
%\qquad
%\text{if } \Delta_t-\ol{\omega}_\rho  \ge   \frac{\d_t^2}{\a}+   \frac{\d_t^{'2}}{\b}. 
%\label{eq:contraction 2}
%\end{align}
\begin{comment}
Our assumptions in (\ref{eq:step size assump},\ref{eq:first-step-size-assump}) imply that
\begin{equation}
\a < \frac{1}{\omega_\rho},
\qquad 
\b < \frac{1}{\omega'_\rho}.
\label{eq:step-size-consq}
\end{equation}
Let us additionally assume that  
\begin{align}
\widetilde{\eta}_{\rho,1} <1,
\label{eq:cnd_on_psi_later}
\end{align}
\begin{align}
\s_0 < \widetilde{\s}_0:= \frac{\rho}{4}\min\l( 2-2\widetilde{\eta}_{\rho,1} , 1-\a\omega_\rho, 1-\b\omega'_\rho \r).
\label{eq:contraction cnds 2}
\end{align}
From (\ref{eq:step-size-consq},\ref{eq:cnd_on_psi_later},\ref{eq:contraction cnds 2}), 
\end{comment}
To simplify the above expressions, let us assume that
\begin{align}
\sqrt{\max\l(\frac{\a}{2}(\omega_\rho+4\s_0), \b(\omega'_\rho+4\s_0\kappa_G^2)  \r)} \le  \min\l(\frac{\a\mu_\rho}{16},\frac{\b\mu'_\rho}{8} \r) \le \frac{1}{2},
\label{eq:simp-assump-contraction}
\end{align}
from which it follows that 
\begin{align}
\max(\eta_{\rho,1},\eta_{\rho,2}) &\le 1-  \min\l(\frac{\a\mu_\rho}{16}, \frac{\b\mu'_\rho}{8}  \r)+  \frac{\ol{\mu}_\rho}{2\ol{\eta}_\rho} \nonumber\\
& \le 1-   \min\l(\frac{\a\mu_\rho}{32}, \frac{\b\mu'_\rho}{16}  \r) \nonumber\\
& =: 1-\eta_\rho \in [0,1),
\label{eq:defn-of-eta}
\end{align}
where the second line above holds if
\begin{align}
\ol{\eta}_\rho \ge \frac{\ol{\mu}_\rho}{ \min\l(\frac{\a\mu_\rho}{16},\frac{\b\mu'_\rho}{8}  \r)}.
\label{eq:second-req-for-etabar}
\end{align}
Then, by unfolding (\ref{eq:contraction},\ref{eq:contraction 2}), we reach
\begin{align}
\Delta_t & \le 
(1-\eta_\rho)^t \Delta_0 .
\label{eq:geo decay lagrangian}
\end{align}
Moreover, by combining (\ref{eq:str cvx lemma 1},\ref{eq:geo decay lagrangian}), we can bound the error, namely,
\begin{align} 
\frac{\d_t^2}{\a} + \frac{\d'^2_t}{\b} 
& \le \max(\alpha \mu_\rho, \beta \mu'_\rho ) \l( \mu_\rho \d_t^2+ \mu'_\rho \d'^2_t \r) \nonumber\\
& \le \mu_\rho \d_t^2 + \mu'_\rho \d'^2_t 
\qquad \text{(see (\ref{eq:first-step-size-assump},\ref{eq:step size assump}), Lemmas \ref{lem:smoothness} and \ref{lem:str cvx})}\nonumber\\
& \le 2(\Delta_t + \ol{\mu}_\rho) 
\qquad \text{(see \eqref{eq:str cvx lemma 1})}
\nonumber\\
& \le 
 2 (1-\eta_\rho)^t   \Delta_0  + 
\frac{2\ol{\mu}_\rho}{\eta_\rho }
%\qquad \text{(see first line of \eqref{eq:geo decay lagrangian})}
\nonumber\\
& \le 2 (1-\eta_\rho)^t \Delta_0 + \frac{2 \ol{\mu}_\rho}{ \min\l( \frac{\a\mu_\rho}{16},\frac{\b\mu'_\rho}{8} \r)}  
\qquad \text{(see (\ref{eq:defn-of-eta}))}
\nonumber\\
& =: 2 (1-\eta_\rho)^t \Delta_0 +\frac{\ol{\eta}_\rho}{\rho}.
\qquad \text{(this choice of }\ol{\eta}_\rho \text{ satisfies (\ref{eq:thresh},\ref{eq:second-req-for-etabar}))}.
\label{eq:geo decay dist}
\end{align}
\begin{comment}
In light of (\ref{eq:thresh},\ref{eq:proof 3},\ref{eq:cnd_on_psi_later},\ref{eq:geo decay dist}), we  select the threshold $\psi_\rho$ to satisfy 
\begin{align}
\psi_\rho  & \ge \max\Bigg(
\l(  \frac{1}{1-\eta_{\rho,1}}+   \frac{1}{1-\eta_{\rho,2}}\r)
\frac{2(\ol{\eta}_{\rho,1}+\ol{\eta}_{\rho,2}) +2\ol{\mu}_\rho}{\min(\mu_\rho,\mu'_\rho)} \nonumber\\
& \qquad\qquad\qquad   ,
\sqrt{\frac{2(\ol{\omega}_\rho + \ol{\mu}_\rho ) }{\min\l( \a(\mu_\rho - \omega_\rho ), \b (\mu'_\rho - \omega'_\rho ) \r) - 2\t_0}  }
\nonumber\\
& \qquad \qquad \qquad 
, \sqrt{2\ol{\mu}_\rho}\l(  \min(\mu_\rho \a, \mu'_\rho \b)  - \frac{8(\omega_\rho+4\omega_\rho')}{\mu_\rho} \r)^{-\frac{1}{2}}
\Bigg),
\label{eq:other cnd on tau}
\end{align}
which also simplifies \eqref{eq:geo decay dist} as 
\begin{align}
\|v_t-\wh{v}\|_2^2 \le \frac{2\max(\eta_{\rho,1}^t,\eta_{\rho,2}^t)  \Delta_0}{\min(\mu_\rho,\mu_\rho')}  + \psi_\rho. 
\label{eq:final-bnd-on-v}
\end{align}
In addition,  we can bound the  feasibility gap as 
\begin{align}
\|A_t\|_2^2 & \le \frac{2\Delta_t}{\rho} 
\qquad \text{(see (\ref{eq:ind Lagr},\ref{eq:defn of Delta},\ref{eq:admissible}))}
\nonumber\\
& \le 
\max(\eta_{\rho,1}^t,\eta_{\rho,2}^t) \frac{2\Delta_0}{\rho} + 
\l( \frac{1}{1-\eta_{\rho,1}}+ \frac{1}{1-\eta_{\rho,2}}  \r) \frac{2(\ol{\eta}_{\rho,1}+\ol{\eta}_{\rho,2})}{\rho }
\qquad \text{(see \eqref{eq:geo decay lagrangian})} \nonumber\\
& \le \max(\eta_{\rho,1}^t,\eta_{\rho,2}^t) \frac{2\Delta_0}{\rho} + 
\l( \frac{1}{1-\eta_{\rho,1}}+ \frac{1}{1-\eta_{\rho,2}}  \r) \frac{2  \min(\mu_\rho,\mu'_\rho) ( (\ol{\eta}_{\rho,1}+\ol{\eta}_{\rho,2})+\ol{\mu}_\rho)}{\rho\min(\mu_\rho,\mu_\rho')  } 
\nonumber\\
& \le 
\max(\eta_{\rho,1}^t,\eta_{\rho,2}^t) \frac{2\Delta_0}{\rho} + 
\frac{\min(\mu_\rho,\mu'_\rho) \psi_\rho}{\rho}.
\qquad \text{(see \eqref{eq:other cnd on tau})}
\label{eq:bnd on feas proof}
\end{align}
\end{comment}
It remains to bound the feasibility gap $\|A_t\|_2$, see \eqref{eq:defn of A}.
\begin{comment}
The naive way to do achieve this is via \eqref{eq:bnd-on-At}, which does not clearly reflect the role of penalty weight $\rho$. Indeed, increasing penalty weight $\rho$ must eventually derive  the feasibility gap to zero, which is not reflected by the right-hand side of  \eqref{eq:bnd-on-At}, as clear from  \eqref{eq:thresh}. 
\end{comment}
Instead of \eqref{eq:bnd-on-At}, we consider the following alternative approach to bound $\|A_t\|_2$. Using definition of $\Delta_t$ in  \eqref{eq:defn of Delta}, we write that 
\begin{align}
\Delta_t & = \mathcal{L}_\rho(v_t,\lambda_t) - \mathcal{L}_\rho(v^*,\lambda^* ) 
\qquad \text{(see \eqref{eq:defn of Delta})}
\nonumber\\
& = \mathcal{L}_\rho(v_t,\lambda_t) - \mathcal{L}_\rho(v_t,\lambda^*) + \mathcal{L}_\rho(v_t,\lambda^*) - 
\mathcal{L}_\rho(v^*,\lambda^* ) \nonumber\\
& = \langle A_t, \lambda_t - \lambda^* \rangle + \mathcal{L}(v_t,\lambda^*) - \mathcal{L}(v^*,\lambda^*) + \frac{\rho}{2}\|A_t\|_2^2 ,
\label{eq:Delta-to-A-1}
\end{align}
where 
\begin{align}
\mathcal{L}(v,\lambda)=\mathcal{L}(w,z,\lambda) := L(w) + R(w) + H(z) + \langle w- G(z), \lambda\rangle.
\end{align}
It is not difficult to verify that $\mathcal{L}(v^*,\lambda^*)=\mathcal{L}_\rho(v^*,\lambda^*)$ is the optimal value of problem \eqref{eq:emp loss min} and that $\mathcal{L}(v_t,\lambda^*)\ge \mathcal{L}(v^*,\lambda^*)$, from which it follows that 
\begin{align}
\Delta_t & \ge \langle A_t, \lambda_t - \lambda^* \rangle + \frac{\rho}{2}\|A_t\|_2^2 
\qquad \text{(see \eqref{eq:Delta-to-A-1})}
\nonumber\\
& \ge - \frac{\rho}{4}\|A_t\|_2^2- \frac{1}{\rho }\|\lambda_t - \lambda^*\|_2^2 + \frac{\rho}{2}\|A_t\|_2^2 
\qquad (\text{Holder's inequality and } 2ab\le a^2+b^2) \nonumber\\
& \ge - \frac{2}{\rho}\|\lambda_t\|_2^2 - \frac{2}{\rho}\|\lambda^*\|_2^2 + \frac{\rho}{4}\|A_t\|_2^2
\qquad ((a+b)^2 \le 2 a^2+2b^2) \nonumber\\
& \ge -\frac{2\lambda_{\max}^2}{\rho} - \frac{2\|\lambda^*\|_2^2}{\rho}  + \frac{\rho}{4}\|A_t\|_2^2,
\qquad \text{(see \eqref{eq:dual seq})}
\label{eq:Delta-to-A-2}
\end{align}
which, in turn, implies that 
\begin{align}
\|A_t\|_2^2 &\le \frac{4}{\rho}\l(\Delta_t +\frac{2\lambda_{\max}^2}{\rho} + \frac{2\|\lambda^*\|_2^2}{\rho}\r)
\qquad \text{(see \eqref{eq:Delta-to-A-2})} \nonumber\\
& \le \frac{4}{\rho}\l( (1-\eta_\rho)^t \Delta_0 + \frac{2(\ol{\eta}_{\rho,1}+ \ol{\eta}_{\rho,2})}{\eta_\rho}+\frac{2\lambda_{\max}^2}{\rho} + \frac{2\|\lambda^*\|_2^2}{\rho} \r)
\qquad \text{(see \eqref{eq:geo decay lagrangian})} \nonumber\\
& \le \frac{4}{\rho}\l( (1-\eta_\rho)^t \Delta_0 + \frac{\ol{\eta}_\rho +2\lambda_{\max}^2 + 2\|\lambda^*\|_2^2}{\rho} \r)
\qquad \text{(see \eqref{eq:geo decay dist})}\nonumber\\
& =: \frac{4(1-\eta_\rho)^t \Delta_0}{\rho }+ \frac{\widetilde{\eta}_\rho}{\rho^2}.
\label{eq:bnd on feas proof}
%\frac{4}{\rho}\l(\ol{\eta}_\rho + 2\lambda_{\max}^2+ 2\|\lambda^*\|_2^2\r) 
\end{align}
\begin{comment}
Recalling \eqref{eq:bnd-on-At}, we can also bound the feasibility gap as 
\begin{align}
\| A_t\|_2^2 & \le (\d_t + \kappa_G^2 \d'_t)^2 
\qquad \text{(see \eqref{eq:bnd-on-At})}
\nonumber\\
& \le 2\d_t^2 + 2 \kappa_G^2 \d'^2_t 
\qquad ((a+b)^2 \le 2a^2+2b^2) \nonumber\\
& \le 2\max(\a, \b\kappa_G^2) \l(\frac{\d_t^2}{\a}+ \frac{\d'^2_t}{\b} \r) \nonumber\\
& \le 2\max(\a, \b\kappa_G^2) (2 \eta_\rho^t {\Delta}_{0}+ \phi^2_\rho).
\qquad \text{(see \eqref{eq:geo decay dist})}
\label{eq:bnd on feas proof}
\end{align}
\end{comment}
\begin{comment}
In light of the bound on the feasibility gap in \eqref{eq:bnd on feas proof}, we revisit the expression in (\ref{eq:xi rho bar raw}) and simplify it as 
\begin{align}
\xi_\rho  & =  \nu_G (\lambda_{\max}+\rho \max_i \|A_i\|_2 ) + 2\rho \kappa_G^2 
\qquad \text{(see \eqref{eq:xi rho bar raw})}
\nonumber\\
& \le  
\nu_G \lambda_{\max}+ \rho \nu_G \sqrt{\frac{4\Delta_0}{\rho}+\frac{\widetilde{\eta}_\rho}{\g} } + 2\rho \kappa_G^2,
\qquad \text{(see \eqref{eq:bnd on feas proof})}
\label{eq:upp_bnd_on_xi}
\end{align}
and, to ease the notation, we redefine $\xi_\rho$  to match the upper bound in (\ref{eq:upp_bnd_on_xi}).
\end{comment}
\begin{comment}
Lastly, with \eqref{eq:bnd on feas proof} in hand, we revisit (\ref{eq:slater_lin}) to find that 
\begin{align}
\psi'_\rho \ge 
\frac{2\Delta_0 + \min(\mu_\rho,\mu'_\rho) \psi_\rho}{\rho}.
\end{align}
In light of \eqref{eq:new_thresh}, we can make a simple adjustment to \eqref{eq:final-bnd-on-v} as 
\begin{align}
\|v_t-\wh{v}\|_2^2 & \le \frac{2\max(\eta_{\rho,1}^t,\eta_{\rho,2}^t)  \Delta_0}{\min(\mu_\rho,\mu_\rho')}  + \psi_\rho + \psi'_\rho \nonumber\\ 
& =: \max(\eta_{\rho,1}^t,\eta_{\rho,2}^t)  \widetilde{\Delta}_0  + \widetilde{\psi}_\rho.
\end{align}
\end{comment}
This completes the proof of Theorem \ref{thm:main}. 


Let us also inspect the special case  where $\mu_L\gg \rho \gtrsim 1$ and $\iota_G^2 \gg \nu_G$, where $\approx$ and $\gtrsim$ suppress any universal constants and dependence on the dual optimal variable $\lambda^*$, for the sake of simplicity.   From Lemmas \ref{lem:smoothness} and \ref{lem:str cvx}, it is easy to verify that 
\begin{align*}
\nu_\rho \approx \nu_L,
\qquad \xi_\rho \approx \rho \kappa_G^2,
\qquad 
\tau_\rho = \rho \kappa_G,
\end{align*}
\begin{align}
\mu_\rho \approx \mu_L,
\qquad 
\mu'_\rho \approx \rho \iota_G^2,
\qquad 
\ol{\mu}_\rho \approx \rho^{-1},
\qquad 
\omega'_\rho \approx \rho \nu_G.
\end{align}
%\begin{align}
%\ol{\nu}_\rho = \ol{\xi}_\rho=\ol{\tau}_\rho = \omega_\rho = \ol{\omega}_\rho = 0.
%\end{align}
We can then take 
\begin{align}
\alpha & \approx \frac{1}{\nu_L}, \qquad \text{(see \eqref{eq:first-step-size-assump})} \nonumber\\
\beta & \approx \frac{1}{\xi_\rho} \approx \frac{1}{\rho \kappa_G^2},
\qquad \text{(see \eqref{eq:step size assump})} \nonumber\\
\eta_\rho &  \approx \min\l(\frac{\mu_L}{\nu_L}, \frac{\iota_G^2}{\kappa_G^2}  \r),
\qquad \text{(see \eqref{eq:defn-of-eta})}\nonumber\\
%\ol{\eta}_{\rho,1} &= \ol{\eta}_{\rho,2}  = 0,
%\qquad \text{(see (\ref{eq:contraction},\ref{eq:contraction 2}))}
%\nonumber\\
\ol{\eta}_\rho & \approx \frac{\rho \ol{\mu}_\rho}{\min\l(\a\mu_\rho, \b\mu'_\rho \r)} \approx \max\l( \frac{\nu_L}{\mu_L}, \frac{\kappa_G^2}{\iota_G^2}  \r),
\qquad \text{(see \eqref{eq:geo decay dist})} \nonumber\\
\widetilde{\eta}_\rho & \approx \ol{\eta}_\rho \approx   \max\l( \frac{\nu_L}{\mu_L}, \frac{\kappa_G^2}{\iota_G^2}  \r).
\qquad \text{(see \eqref{eq:bnd on feas proof})}
\end{align}
Lastly, for \eqref{eq:simp-assump-contraction} to hold, it suffices that 
\begin{align}
\s_0 \lesssim \rho  \min\l(\frac{\mu_L^2}{\nu_L^2}, \frac{\iota_G^4}{\kappa_G^4}  \r)=:\s_{0,\rho}.
\end{align}



\begin{comment}
To close, let us summarize the key quantities defined throughout  the proof:
\newpage
\begin{align}
 \a & \in  (\widetilde{\a}, 1/\nu_\rho],
 \qquad 
 \widetilde{ \alpha}:=\frac{8}{\mu_\rho^2}(\omega_\rho+ 4\omega'_\rho  ),
%\widetilde{\alpha}
%(\a,\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0)
\nonumber\\
\b  & \in   (\widetilde{\b}, 1/\xi_\rho],
\qquad 
\widetilde{\beta}:= \frac{8}{\mu_\rho \mu'_\rho}(\omega_\rho+4 \omega'_\rho  ) ,
%\widetilde{\a} 
%(\rho,\s_l,\zeta_L,\s_L,\nu_G,\iota_G,\kappa_G,\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L,\lambda_0)
 \nonumber\\
\s_0 & < \widetilde{\s}_0 :=  \frac{\rho}{4}\min\l( 2-2\widetilde{\eta}_{\rho,1} , 1-\a\omega_\rho, 1-\b\omega'_\rho \r), \nonumber\\
\widetilde{\eta}_{\rho,1} & := 
1 -  \frac{1}{8}\min(\mu_\rho\a, \mu'_\rho \b ) + \frac{\ol{\mu}_\rho }{4\psi_\rho^2 }   +  \frac{\omega_\rho + 4\omega'_\rho }{\mu_\rho} , \nonumber\\
\eta_{\rho} & := \max( \eta_{\rho,1}, \eta_{\rho,2}), \nonumber\\
\eta_{\rho,1} & =\frac{ \rho \widetilde{\eta}_{\rho,1}}{\rho - 2 \s_0} 
, \nonumber\\
\ol{\eta}_{\rho,1} & = 
\frac{\rho \widehat{\eta}_{\rho,1}}{\rho - 2\s_0}
, \nonumber\\
\widehat{\eta}_{\rho,1} & = 
\a\ol{\tau}^2_\rho + \ol{\nu}_\rho 
+ \ol{\xi}_\rho  + \frac{(\omega_\rho+4\omega'_\rho)\ol{\mu}_\rho}{\mu_\rho} 
   + \frac{ \ol{\omega}_\rho^2}{2\psi_\rho^2},
\nonumber\\
\eta_{\rho,2} & = \max(\a\omega_\rho+1 , \b\omega'_\rho+1 )  \frac{\rho }{2(\rho-2\sigma_0)},  \nonumber\\
\ol{\eta}_{\rho,2} & =  \frac{\rho }{\rho-2\sigma_{0}} \l( \a\ol{\tau}^2_\rho + \ol{\nu}_\rho 
+ \ol{\xi}_\rho  +  \frac{\omega_\rho \ol{\mu}_\rho}{2\mu_\rho} + \frac{\ol{\omega}_\rho}{2} \r),\nonumber\\
\psi_\rho  & \ge \max\Bigg(
\l(  \frac{1}{1-\eta_{\rho,1}}+   \frac{1}{1-\eta_{\rho,2}}\r)
\frac{2(\ol{\eta}_{\rho,1}+\ol{\eta}_{\rho,2}) +2\ol{\mu}_\rho}{\min(\mu_\rho,\mu'_\rho)} \nonumber\\
& \qquad\qquad\qquad   ,
\sqrt{\frac{2(\ol{\omega}_\rho + \ol{\mu}_\rho ) }{\min\l( \a(\mu_\rho - \omega_\rho ), \b (\mu'_\rho - \omega'_\rho ) \r) - 2\t_0}  }
\nonumber\\
& \qquad \qquad \qquad 
, \sqrt{2\ol{\mu}_\rho}\l(  \min(\mu_\rho \a, \mu'_\rho \b)  - \frac{8(\omega_\rho+4\omega_\rho')}{\mu_\rho} \r)^{-\frac{1}{2}}
\Bigg),
\nonumber\\
 \psi'_\rho & =
\frac{2\Delta_0 + \min(\mu_\rho,\mu'_\rho) \psi_\rho}{\rho}  \nonumber\\
\widetilde{\psi}_\rho & = \psi_\rho + \psi'_\rho \nonumber\\
\widetilde{\Delta}_0 & := \frac{2\Delta_0}{\min(\mu_\rho,\mu_\rho')}
\qquad \text{(see \eqref{eq:defn of Delta})}
 \nonumber\\
\t_0 & := \sqrt{\frac{2\a\b\tau_\rho^2}{1-\b\xi_\rho}},\nonumber\\
\nu_\rho & = \nu_L+\rho,
\qquad 
\ol{\nu}_\rho := \rho, \nonumber\\
\xi_\rho  & = \nu_G (\lambda_{\max}+\rho \max_i \|A_i\|_2 ) + 2\rho \kappa_G^2, \nonumber\\
\ol{\xi}_\rho & = \ol{\nu}_G( \lambda_{\max} + \rho \max_i \|A_i\|_2 ) + \rho \ol{\kappa}_G^2, \nonumber\\
\tau_\rho &  := \rho \kappa_G, 
\qquad 
\ol{\tau}_\rho := \rho \ol{\kappa}_G, \nonumber\\
\mu_\rho & := \mu_L - 2\rho,\qquad 
\mu'_\rho :=
 \frac{\rho \iota^2_G}{4}-\nu_G\|\lambda^*\|_2 ,\nonumber\\
\ol{\mu}_\rho &  = \ol{\mu}_L + \ol{\nu}_G\|\lambda^*\|_2 + \frac{\rho \ol{\iota}^2_G}{4} + 
\frac{3}{\rho}\l( \lambda_{\max}^2 + \|\lambda^*\|_2^2\r), \nonumber\\
\omega_\rho & := 0,
\qquad 
\omega'_\rho :=
\nu_G \lambda_{\max} + 2\rho\kappa^2_G,\nonumber\\
\ol{\omega}_\rho & = \ol{\nu}_G\lambda_{\max}+\rho\ol{\kappa}^2_G,  \nonumber\\
\lambda_{\max} & :=  \| \lambda_{0}\|_2 + c\sigma_0, 
\qquad 
c = \sum_{t=1}^{\infty} \frac{1}{t \log^2(t+1)}.
\end{align}

\end{comment}



\begin{comment}
%\section{Proof of Lemma \ref{lem:ws_to_wn} \label{sec:proof of ws_to_wn}}

Recall that $R=1_W$ and $H=0$ for this proof. Using the optimality of $w^*\in\text{relint}(W)$ in \eqref{eq:final_problem_k1}, we can write that 
\begin{align}
\| \nabla L(w^*) \|_2 & \le \| \nabla L(w^*) \|_2 + \| \nabla L(w^*) - \nabla L(w^*) \|_2
\qquad 
\text{(triangle inequality)} \nonumber\\
& =  \| \nabla L(w^*) - \nabla L(w^*) \|_2
\qquad \l( \nabla L(w^*) = 0  \r) \nonumber\\
& \le \max_{w\in W}\| \nabla L(w) - \nabla L(w) \|_2.
\label{eq:near_st}
\end{align}
On the other hand, using the strong convexity of $L$ in \eqref{eq:L_str_cvx}, we can write that 
\begin{align}
\| w^\n - w^* \|_2 &
\le \frac{1}{\zeta_L} \| \nabla L(w^\n) - \nabla L(w^*) \|_2 
\qquad \text{(see \eqref{eq:L_str_cvx})}
\nonumber\\
& = \frac{1}{\zeta_L} \|\nabla L(w^*) \|  
\qquad (\nabla L(w^\n) = 0 )
\nonumber\\
& \le \frac{1}{\zeta_L} \max_{w\in W}\| \nabla L(w) - \nabla L(w) \|_2,
\qquad \text{(see \eqref{eq:near_st})}
\end{align}
which completes the proof of Lemma \ref{lem:ws_to_wn}. 
\end{comment}


\section{Proof of Lemma \ref{lem:smoothness} \label{sec:smoothness}}


To prove \eqref{eq:smoothness lemma w}, we write that 
\begin{align}
&  \Lagr'_\rho (w_{t+1},z_{t+1},\lambda_{t}) - \Lagr'_\rho (w_{t},z_{t+1},\lambda_{t}) - 
\langle w_{t+1}-w_{t}, \nabla_w \Lagr'_\rho(w_{t},z_{t+1},\lambda_{t})  \rangle  \nonumber\\
& = L(w_{t+1}) - L(w_t) - \langle w_{t+1}-w_t , \nabla_w L(w_t) \rangle \nonumber\\
& \qquad+ \frac{\rho}{2}\|w_{t+1}-G(z_{t+1})\|_2^2 - \frac{\rho}{2}\|w_t - G(z_{t+1})\|_2^2 - 2\rho \langle w_{t+1}-w_t, w_t - G(z_{t+1}) \rangle  
\qquad \text{(see \eqref{eq:ind Lagr prime})}
\nonumber\\
& \le \frac{\nu_L}{2}\|w_{t+1}-w_t\|_2^2 + \ol{\nu}_L + \frac{\rho}{2}\| w_{t+1}-w_t \|_2^2 
\qquad \text{(see \eqref{eq:smoothness of L})} \nonumber\\
& =: \frac{\nu_\rho}{2}\|w_{t+1}-w_t\|_2^2 + \ol{\nu}_\rho.
\end{align}
To prove \eqref{eq:smoothness lemma z}, let us first control the dual sequence $\{\lambda_{t}\}_t$ by writing that 
\begin{align}
\|\lambda_{t}\|_2 & = 
\| \lambda_{0}+ \sum_{i=1}^t \sigma_{i} A_{i} \|_2 
\qquad \text{(see \eqref{eq:dual update proof})}
\nonumber\\
& \le \| \lambda_{0}\|_2 + \sum_{i=1}^t \sigma_{i} \|A_{i}\|_2 
\qquad \text{(triangle inequality)}
\nonumber\\
& \le \| \lambda_{0}\|_2 + \sum_{t'=1}^t \frac{\s_0}{i \log^2 (i+1)} \nonumber\\
& \le   \| \lambda_{0}\|_2 + c\sigma_0 \nonumber\\
& =: \lambda_{\max},
\label{eq:dual seq}
\end{align}
where 
\begin{align}
c \ge \sum_{t=1}^{\infty} \frac{1}{t \log^2(t+1)}. 
\end{align}
We now write that 
\begin{align}
& \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \Lagr'_\rho(w_t,z_{t},\lambda_t) - \langle z_{t+1}-z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \nonumber\\
& = -\langle G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) ,\lambda_t \rangle \nonumber\\
& \qquad + \frac{\rho}{2} \|w_t - G(z_{t+1})\|_2^2 - \frac{\rho}{2}\|w_t - G(z_t)\|_2^2 \nonumber\\
& \qquad + \rho \langle DG(z_t) (z_{t+1}-z_t) ,  w_t - G(z_t) \rangle .
\qquad \text{(see \eqref{eq:ind Lagr prime})}
\label{eq:lem proof 1}
\end{align}
To bound the first inner product on the right-hand side above, we write that 
\begin{align}
& \langle G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) ,\lambda_t \rangle \nonumber\\
& \le \| G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) \|_2 \cdot \|\lambda_t\|_2
\qquad \text{(Cauchy-Shwartz's inequality)} \nonumber\\
& \le \frac{\nu_G\lambda_{\max}}{2} \|z_{t+1}-z_t\|_2^2  
\qquad \text{(see (\ref{eq:smoothness of G},\ref{eq:dual seq}))}
\label{eq:lem proof 2}
\end{align}
The remaining component on the right-hand side of \eqref{eq:lem proof 1} can be bounded as 
\begin{align}
& \|w_t-G(z_{t+1})\|_2^2 - \|w_t - G(z_t)\|_2^2 +2  \langle DG(z_t)(z_{t+1}-z_t), w_t - G(z_t) \rangle \nonumber\\
& = \|w_t-G(z_{t+1})\|_2^2 - \|w_t - G(z_t)\|_2^2  
+ 2 \langle G(z_{t+1}) - G(z_t), w_t- G(z_t) \rangle 
\nonumber\\
& \qquad -2 \langle G(z_{t+1}) - G(z_t)  -DG(z_t) (z_{t+1}-z_t) , w_t -G(z_t) \rangle  \nonumber\\
& = \|G(z_{t+1})-G(z_t) \|_2^2 
\nonumber\\
& \qquad +2 \langle G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) , w_t -G(z_t) \rangle \nonumber\\
& \le  \|G(z_{t+1})-G(z_t) \|_2^2 
\nonumber\\
& \qquad +2  \|G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) \|_2 \cdot \| w_t -G(z_t)\|_2
\qquad \text{(Cauchy-Shwartz's inequality)} \nonumber\\
& \le  \kappa_G^2 \|z_{t+1}-z_t\|_2^2 
+  \nu_G\| z_{t+1}-z_t \|_2^2   \|w_t - G(z_t) \|_2
\qquad 
\text{(see (\ref{eq:smoothness of G},\ref{eq:lipschitz of G 2}))} \nonumber\\
& \le   \kappa_G^2 \|z_{t+1}-z_t\|_2^2 + \nu_G\|z_{t+1}-z_t\|_2^2 \max_i  \|A_i\|_2. 
\qquad \text{(see (\ref{eq:defn of A}))}
\label{eq:lem proof 3}
\end{align}
Substituting the bounds in (\ref{eq:lem proof 2},\ref{eq:lem proof 3}) back into \eqref{eq:lem proof 1}, we find that 
\begin{align}
& \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \Lagr'_\rho(w_t,z_{t},\lambda_t) - \langle z_{t+1}-z_t, \nabla_z \Lagr'_\rho(w_t,z_t,\lambda_t) \nonumber\\
& \le 
\frac{1}{2}\l(   \nu_G (\lambda_{\max}+\rho \max_i \|A_i\|_2 ) + \rho \kappa_G^2\r) \|z_{t+1}-z_t\|_2^2 \nonumber\\
& =: \frac{ \xi_\rho}{2}\|z_{t+1}-z_t\|_2^2 + \ol{\xi}_\rho, 
\end{align}
which proves \eqref{eq:smoothness lemma z}. To prove \eqref{eq:smoothness lemma zw}, we write that 
\begin{align}
& \| \nabla_w \Lagr'_\rho(w_t,z_{t+1},\lambda_t) - \nabla_w \Lagr'_\rho(w_t,z_t,\lambda_t) \|_2 \nonumber\\
& = \rho \| G(z_{t+1}) - G(z_t) \|_2  
\qquad \text{(see \eqref{eq:ind Lagr prime})} \nonumber\\
& \le \rho  \kappa_G \|z_{t+1}-z_t\|_2 
\qquad \text{(see \eqref{eq:lipschitz of G 2})} \nonumber\\
& =: \tau_\rho \| z_{t+1}-z_t\|_2 + \ol{\tau}_\rho. 
\end{align}
%
%
%
%
%Recalling the definition of $\Lagr_\a$ in \eqref{eq:ind Lagr}, we can write that 
%\begin{align}
%& \Lagr_\a(v_{t+1},\lambda_t) - \Lagr_\a(v_{t},\lambda_t) 
%- \langle  v_{t+1}-v_t, \nabla_v \Lagr_\a (v_t,\lambda_t) \rangle 
%\nonumber\\
%& = L(u_{t+1}) - L(u_k)- \langle u_{k+1}-u_k, \nabla_u L(u_k)
%\nonumber\\
%& \qquad - \langle G(z_{t+1}) - G(z_t) - DG(z_t) (z_{t+1}-z_t) ,
%\lambda_t
%\rangle \nonumber\\
%& \qquad + \frac{\aeta}{2}\l( \|A_{t+1}\|_2^2
%- \|A_t\|_2^2  
%-2 \langle  v_{t+1}-v_t, DA(v_t)^\top A_t  \rangle\r),
%\label{eq:smoothness 0}
%\end{align}
%where 
%\begin{align}
%D A(v)
%= 
%\l[
%\begin{array}{cc}
%I_d & -D_zG(z)^\top
%\end{array}
%\r]^\top.
%\label{eq:DA expression}
%\end{align}
%To bound the last line in \eqref{eq:smoothness 0}, we write that 
%\begin{align}
%&  \|A_{t+1}\|_2^2 - \|A_t\|_2^2 - 2 \langle DA(v_t) (v_{t+1}-v_t),  A_t \rangle \nonumber\\
%& = \|A_{t+1}\|_2^2
%- \|A_t\|_2^2  - 2 \langle u_{t+1}-u_t,A_t \rangle 
%+ 2 \langle DG(z_t)(z_{t+1}-z_t) , A_t  \rangle
%\qquad \text{(see \eqref{eq:DA expression})}
%  \nonumber\\
%& = \|A_{t+1}\|_2^2 + \|A_t\|_2^2 
%- 2 \langle A_{t+1}, A_t \rangle 
%+2  \langle G(z_{t+1})- G(z_t) - DG(z_t) (z_{t+1}-z_t) , A_t  \rangle \qquad \text{(see \eqref{eq:defn of A})} \nonumber\\
%& \le  \|A_{t+1}-A_t\|_2^2 + \nu_G \|z_{t+1}-z_t\|_2^2 \|A_t\|_2 + 2\xi_G\|A_t\|_2
%\qquad \text{(see (\ref{eq:smoothness of G}))}
%\nonumber\\
%& \le 2\|u_{t+1}-u_t\|_2^2 +2 \| G(z_{t+1})-G(z_t) \|_2^2
%+ \nu_G \|z_{t+1}-z_t\|_2^2 \|A_t\|_2 + 2\xi_G\|A_t\|_2 
%\qquad 
%\l( \text{(\ref{eq:defn of A}) and } \|a+b\|_2^2 \le 2 \|a\|_2^2+2\|b\|_2^2 \r)
%\nonumber\\
%& \le 2\|u_{t+1}-u_t\|_2^2 +4 \nu'^2_G \|z_{t+1}-z_t\|_2^2 +  4 \xi_G'^2 
%+ \nu_G \|z_{t+1}-z_t\|_2^2 \|A_t\|_2 + 2\xi_G\|A_t\|_2  
%\qquad \l( \text{(\ref{eq:lipschitz of G 2}) and } \|a+b\|_2^2 \le 2\|a\|_2^2+2\|b\|_2^2 \r) \nonumber\\
%& =  2\|u_{t+1}-u_t\|_2^2 + ( \nu_G \|A_t\|_2 + 4\nu'^2_G )\|z_{t+1}-z_t\|_2^2 + 2\xi_G \|A_t\|_2+ 4\xi'^2_G. 
%\label{eq:smoothness 1}
%\end{align}
%Substituting the above bound back into \eqref{eq:smoothness 0} and also invoking (\ref{eq:smoothness of L},\ref{eq:smoothness of G}), we find that 
%\begin{align}
%& \Lagr_\a(v_{t+1},\lambda_t) - \Lagr_\a(v_{t},\lambda_t) 
%- \langle  v_{t+1}-v_t, \nabla_v \Lagr_\a (v_t,\lambda_t) \rangle \nonumber\\
%& \le \frac{\nu_L}{2}\|u_{t+1}-u_t\|_2^2+ \xi_L +  \l(\frac{\nu_G}{2}\|z_{t+1}-z_t\|_2^2  + \xi_G \r) \|\lambda_t\|_2
% \nonumber\\
%& \qquad 
%+ \aeta \|u_{t+1}-u_t\|_2^2 +   \frac{\a}{2}(\nu_G\|A_t\|_2+4\nu'^2_G)  \|z_{t+1}-z_t\|_2^2 
%+ \a\xi_G\|A_t\|_2+2\a\xi'^2_G
%\qquad \text{(see (\ref{eq:smoothness of L},\ref{eq:smoothness of G},\ref{eq:smoothness 0},\ref{eq:smoothness 1}))} \nonumber\\
%& = \frac{ \nu_L + 2\aeta }{2}\|u_{t+1}-u_t\|_2^2 
%+ \frac{1}{2} ( \nu_G (\|\lambda_t\|_2+ \aeta \|A_t\|_2 ) + 4\aeta\nu'^2_G  ) \|z_{t+1}-z_t\|_2^2 
%+ \xi_L+ \xi_G \|\lambda_t\|_2+ \a\xi_G\|A_t\|_2+ 2\a\xi'^2_G
%\nonumber\\
%& \le \frac{\nu_\aeta}{2} \|u_{t+1}-u_t\|_2^2 + \frac{\nu_\aeta}{2}\|z_{t+1}-z_t\|_2^2 + \xi_\a, 
%\qquad \text{(see below and \eqref{eq:dual seq})}
%\end{align}
%where we set 
%\begin{align}
%\nu_\aeta : =  \max\l( \nu_L + 2\aeta,  \nu_G (\|\lambda_0\|_2+c\sigma_0+ \aeta \max_{t'} \|A_{t'}\|_2 ) + 4\aeta\nu'^2_G    \r),
%\end{align}
%\begin{align}
%\xi_\a :=  \xi_L+ \xi_G \|\lambda_0\|_2 + c\xi_G \sigma_0 + \a\xi_G\max_{t'} \|A_{t'}\|_2+ 2\a\xi'^2_G. 
%\qquad \text{(see \eqref{eq:dual seq})}
%\end{align}
This completes the proof of Lemma \ref{lem:smoothness}. 

\section{Proof of Lemma \ref{lem:str cvx} \label{sec:str cvx}}

For future reference, we record that 
\begin{align}
&   \langle v_{t} - \wh{v}, \nabla_v \Lagr'_\rho (\wh{v}) \rangle 
\nonumber\\
& = \langle w_{t} - \wh{w} , \nabla_w \Lagr'_\rho (\wh{v}) \rangle 
+ \langle z_{t} -\wh{z} , \nabla_z \Lagr'_\rho (\wh{v})  \rangle 
\qquad \l( v = (w,z) \r)
\nonumber\\
& = \langle w_{t} - \wh{w} , \nabla L(\wh{w}) + \wh{\lambda} + \rho (\wh{w}-G(\wh{z}) \rangle 
- \langle DG(\wh{z})(z_{t} - \wh{z}) , \wh{\lambda} + \rho (\wh{w} - G(\wh{z})) \rangle 
\qquad \text{(see \eqref{eq:ind Lagr prime})}
 \nonumber\\
 & = \langle w_{t} - \wh{w} , \nabla L(\wh{w}) + \wh{\lambda}  \rangle 
- \langle DG(\wh{z})(z_{t} - \wh{z}) , \wh{\lambda} \rangle,
\qquad \qquad \text{(see \eqref{eq:opt cnds})}
\label{eq:opt cnd consq}
\end{align}
where the last line above uses the feasibility of $v^*$ in \eqref{eq:emp loss min}. 
To prove \eqref{eq:str cvx lemma 1}, we use the definition of $\Lagr_\rho$ in \eqref{eq:ind Lagr} to write that 
\begin{align}
& \Lagr_\rho(v_{t},\lambda_{t}) - \Lagr_\rho(\wh{v},\wh{\lambda}) \nonumber\\
& = \Lagr'_\rho(v_t,\lambda_t) - \Lagr'_\rho(v^*,\lambda^*) 
+ R(w_t) - R(w^*) + L(z_t) - L(z^*) 
\qquad \text{(see (\ref{eq:ind Lagr},\ref{eq:ind Lagr prime}))}
\nonumber\\
& \ge \Lagr'_\rho(v_t,\lambda_t) - \Lagr'_\rho(v^*,\lambda^*)  
- \langle v_t - v^* ,
\nabla_v \Lagr'_\rho (v^*,\lambda^* ) 
 \rangle 
 \qquad \text{(see (\ref{eq:opt cnds}))}
  \nonumber\\
  & = L(w_{t}) - L(\wh{w}) - \langle w_{t} - \wh{w}, \nabla L(\wh{u}) \rangle \nonumber\\
& \qquad + \langle A_{t} , \lambda_{t} \rangle - \langle w_{t} - \wh{w}  - DG(\wh{z}) (z_{t} - \wh{z}),  \wh{\lambda} \rangle + \frac{\rho}{2}\|A_{t}\|_2^2 
\qquad \text{(see (\ref{eq:opt cnd consq}))} 
\nonumber\\
& \ge \frac{\mu_L \d_t^2}{2} + \langle A_{t}, \lambda_{t}- \wh{\lambda}\rangle + \frac{\rho}{2}\|A_{t}\|_2^2 \nonumber\\
& \qquad + \langle G(z_{t}) - G(\wh{z}) - DG(\wh{z}) (z_{t} - \wh{z}_k) , \wh{\lambda} \rangle 
\qquad \text{(see (\ref{eq:str cvx of L},\ref{eq:defn of delta}))} 
\nonumber\\
& \ge \frac{\mu_L\d_t^2}{2} + \langle A_{t}, \lambda_{t}- \wh{\lambda}\rangle + \frac{\rho}{2}\|A_{t}\|_2^2 -\frac{\nu_G\d'^2_t}{2}      \| \lambda^*\|_2. 
\qquad \text{(see (\ref{eq:smoothness of G},\ref{eq:defn of delta}))}
\label{eq:lwr bnd 0}
\end{align}
To control the terms involving $A_t$ in the last line above, we write that 
\begin{align}
& \langle A_t, \lambda_t - \lambda^* \rangle + \frac{\rho}{2}\|A_t\|_2^2 \nonumber\\
& = \frac{\rho}{2}\l\| A_t - \frac{\lambda_t - \lambda^*}{\rho}\r\|_2^2 - \frac{\|\lambda_t-\lambda^*\|_2^2}{2\rho} \nonumber\\
& = \frac{\rho}{2}\l\| w_t - w^* - (G(z_t) - G(z^*)) - \frac{\lambda_t - \lambda^*}{\rho}  \r\|_2^2  - \frac{\|\lambda_t-\lambda^*\|_2^2}{2\rho}
\qquad \text{(see (\ref{eq:opt cnds},\ref{eq:defn of A}))} \nonumber\\
& \ge \frac{\rho}{4}\|G(z_t)-G(z^*)\|_2^2 - \rho\d_t^2 - \frac{3\|\lambda_t - \lambda^*\|_2^2}{2\rho}
\qquad \l(  \|a-b-c\|_2^2 \ge \frac{\|a\|_2^2}{2} - 2\|b\|_2^2 - 2\|c\|_2^2  \r) \nonumber\\
& \ge \frac{\rho\iota_G^2\d'^2_t}{4}  - \rho\d_t^2 - \frac{3\|\lambda_t - \lambda^*\|_2^2}{2\rho}
\qquad \text{(see (\ref{eq:defn of delta},\ref{eq:lipschitz of G 2}))} \nonumber\\
& \ge \frac{\rho \iota_G^2 \d'^2_t}{4}  - \rho\d_t^2 - \frac{3  }{\rho}(\lambda_{\max}^2 + \|\lambda^*\|_2^2),
\qquad ( (a+b)^2 \le 2a^2 +2b^2 \text{ and (\ref{eq:dual seq})})
\end{align}
which, after substituting in \eqref{eq:lwr bnd 0}, yields that 
\begin{align}
& \Lagr_\rho(v_t,\lambda_t) - \Lagr_\rho(v^*,\lambda^*)  \nonumber\\
& \ge \frac{\mu_L - 2\rho }{2}\d_t^2 + \frac{1}{2}\l( \frac{\rho\iota^2_G}{2} - \nu_G\|\lambda^*\|_2 \r) \d'^2_t  - 
\frac{3}{\rho}\l( \lambda_{\max}^2+ \|\lambda^*\|_2^2\r) \nonumber\\
& \ge \frac{\mu_\rho \d_t^2}{2}+ \frac{\mu_\rho'\d'^2_t}{2} - \ol{\mu}_\rho,
\end{align}
where 
\begin{align}
\mu_\rho :=  \mu_L - 2\rho,
\qquad 
\mu'_\rho := \frac{\rho {\iota}^2_G}{2}-\nu_G\|\lambda^*\|_2 ,
\end{align}
\begin{align}
\ol{\mu}_\rho :=  
\frac{3}{\rho}\l( \lambda_{\max}^2 + \|\lambda^*\|_2^2\r). 
\end{align}
This proves \eqref{eq:str cvx lemma 1}. To prove \eqref{eq:smoothness lemma 2}, we use the definition of $\Lagr'_\rho$ in \eqref{eq:ind Lagr prime} to write that 
\begin{align}
& \Lagr'_\rho(v^*,\lambda^*) - \Lagr'_\rho(v_{t},\lambda_{t}) - \langle v^*- v_{t}, \nabla_v \Lagr'_\rho(v_{t},\lambda_{t}) \rangle \nonumber\\
& = L(w^*) - L(w_{t}) - \langle w^* - w_{t} , \nabla L(w_{t}) \rangle \nonumber\\
& \qquad - \langle 
A_t + DA(v_t)(v^*- v_{t})  
,\lambda_{t} \rangle\nonumber\\
& \qquad 
- \frac{\rho}{2}\langle A_{t} + 2 DA(v_t) (v^* - v_{t}) , A_{t} \rangle,
\qquad \text{(see \eqref{eq:ind Lagr prime})}
\label{eq:str cvx lem 0}
\end{align}
where 
\begin{align}
D A(v) & = \l[
\begin{array}{cc}
I_d & - DG(z)
\end{array}
\r],
\label{eq:defn of Jacobian of A}
\end{align}
is the Jacobian of the map $A$. 
The second inner product on the right-hand side of \eqref{eq:str cvx lem 0} can be bounded as 
\begin{align}
&  - \langle 
A_t + DA(v_t)(v^*- v_{t})  
,\lambda_{t} \rangle  \nonumber\\
& =- \langle 
w_{t}-G(z_{t}) + (w^*- w_{t}) - DG(z_{t})(z^* - z_{t})
,\lambda_{t} \rangle 
\qquad \text{(see (\ref{eq:defn of A},\ref{eq:defn of Jacobian of A}))}
\nonumber\\
& = -\langle 
G(z^*) -G(z_{t}) -  DG(z_{t})(z^* - z_{t})
,\lambda_{t} \rangle 
\qquad \l( w^* = G(z^*) \r) \nonumber\\
& \ge- \frac{\nu_G\d'^2_t}{2}   \|\lambda_{t}\|_2   
\qquad \text{(see (\ref{eq:smoothness of G},\ref{eq:defn of delta}))} \nonumber\\
& \ge -\frac{\nu_G\d'^2_t}{2}  \lambda_{\max}.
\qquad \text{(see \eqref{eq:dual seq})} 
\label{eq:lwr bnd proof 0}
\end{align}
To control  the last  inner product on the right-hand side of  \eqref{eq:str cvx lem 0}, we write that 
\begin{align}
& - \frac{\rho}{2}\langle A_t + 2 DA(v_t) (v^* - v_t), A_t \rangle \nonumber\\
& = \frac{ \rho}{2} \|A_t\|_2^2 - \rho \langle A_t + DA(v_t)(v^* - v_t), A_t \rangle \nonumber\\
& \ge -\rho \|A_t +DA(v_t)(v^*-v_t)\|_2 \|A_t\|_2
\qquad \text{(Holder's inequality)}
 \nonumber\\
& = -\rho \| (w^* - G(z^*)) - (w_t - G(z_t))  - (w^* - w_t) + DG(z_t) (z^* - z_t) \|_2 
\qquad (\text{see (\ref{eq:defn of A},\ref{eq:defn of Jacobian of A}) and } w^* = G(z^*) )  
\nonumber\\
& = - \rho \| G(z^*) - G(z_t) - DG(z_t) (z^* - z_t) \|_2 \nonumber\\
& \ge - \frac{\rho \nu_G}{2}\|z^* - z_t\|_2^2 
\qquad \text{(see \eqref{eq:smoothness of G})}
\nonumber\\
&  = - \frac{\rho \nu_G \d'^2_t}{2}.
\qquad \text{(see \eqref{eq:defn of delta})}
\label{eq:lwr bnd proof 3}
\end{align}
By substituting the bounds in  (\ref{eq:lwr bnd proof 0},\ref{eq:lwr bnd proof 3}) back into (\ref{eq:str cvx lem 0}) and also using the convexity of $L$, we reach 
\begin{align}
&  \Lagr'_\rho(v^*,\lambda^*) - \Lagr'_\rho(v_{t},\lambda_{t}) - \langle v^*- v_{t}, \nabla_v \Lagr'_\rho(v_{t},\lambda_{t}) \rangle \nonumber\\
& \ge - \frac{\nu_G  }{2} \l(\lambda_{\max}+ \rho   \r)
 \d'^2_t. 
\end{align}
%

% 
%
% first observe that 
%\begin{align}
%-\frac{\rho}{2} \langle A_t +2 DA(v_t) (v^*-v_t), A_t \rangle = - \frac{\rho}{2} \langle A_t + 2 (w^*-w_t) , A_t \rangle
%+\rho \langle DG(z_t) (z^*-z_t), A_t \rangle.
%\qquad \text{(see (\ref{eq:defn of Jacobian of A}))}
%\label{eq:lwr bnd proof 1}
%\end{align}
%For the first term on the right-hand side above, we note that 
%\begin{align}
%& -  \langle A_{t}+2(w^* - w_{t}) , A_{t} \rangle  \nonumber\\
%& = - \langle w_{t} - G(z_{t}) + 2(w^* - w_{t}) , w_{t} - G(z_{t})\rangle 
%\qquad \text{(see (\ref{eq:defn of A}))}
%\nonumber\\
%& =  \langle G(z_{t}) - G(z^*) + (w_{t} - w^*) , (w_{t} - w^*) - (G(z_{t}) - G(z^*) ) \rangle 
%\qquad \l( w^* = G(z^*) \r)
%\nonumber\\
%& =  \|  (w_{t}- w^*) - (G(z_{t})-G(z^*)) \|_2^2 \nonumber\\
%& =  \| w_{t} - G(z_{t})\|_2^2
%\qquad \l( u^* = G(z^*) \r) \nonumber\\
%& =  \| A_{t}\|_2^2,
%\qquad \text{(see \eqref{eq:defn of A})}
%\label{eq:lwr bnd proof 2}
%\end{align}
%which in turn allows to revisit \eqref{eq:lwr bnd proof 1} and write that 
%\begin{align}
%& -\frac{\rho}{2} \langle A_t +2 DA(v_t) (v^*-v_t), A_t\rangle \nonumber\\
%& = - \frac{\rho}{2}\langle A_{t} + 2 (w^* - w_{t}) ,A_t \rangle +\rho \langle  DG(z_{t})( z^* - z_{t} ), A_{t}  \rangle 
%\qquad \text{(see (\ref{eq:lwr bnd proof 1}))}
%\nonumber\\ 
%& =  \frac{\rho}{2} \|A_{t}\|_2^2 + \rho \langle DG(z_{t})(z^* - z_{t}), A_{t} \rangle
%\qquad \text{(see (\ref{eq:lwr bnd proof 2}))}
% \nonumber\\
%& \ge \frac{\rho}{2} \|A_{t}\|_2^2  - \rho (\kappa_G \|z^* - z_{t}\|_2 + \ol{\kappa}_G ) \|A_{t}\|_2  
%\qquad \text{(see \eqref{eq:smoothness of G 2})} \nonumber\\
%& \ge   - \frac{\rho}{2} (\kappa_G \|z^* - z_{t}\|_2 + \ol{\kappa}_G )^2  
%\qquad \l(2 ab\le a^2+b^2 \r)
% \nonumber\\
% & \ge - \rho \kappa^2_G \|z^* - z_{t}\|_2^2  - \rho \ol{\kappa}^2_G .
%\qquad \l( (a+b)^2\le 2a^2+2b^2 \r)
%\label{eq:lwr bnd proof 3}
%\end{align}
%\begin{align}
%% \Lagr'_\rho(v^*,\lambda^*) - \Lagr'_\rho(v_t,\lambda_t) - \langle v^*- v_t, \nabla_v \Lagr'_\rho(v_t,\lambda_t)   \ge -   \frac{\omega_\rho}{2}\|w_t - w^*\|_2^2  -   \frac{\omega'_\rho}{2}\|z_t - z^*\|_2^2 - \ol{\omega}_\rho,
%%\end{align}
%where 
%\begin{align}
%\omega_\rho := 0,
%\qquad 
%\omega'_\rho :=
%\nu_G \lambda_{\max} + 2\rho\kappa^2_G, 
%\end{align}
%\begin{align}
%\ol{\omega}_\rho := \ol{\nu}_G\lambda_{\max}+\rho\ol{\kappa}^2_G. 
%\end{align}
This proves \eqref{eq:smoothness lemma 2}, thus completing the proof of Lemma \ref{lem:str cvx}. 

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%To prove \eqref{eq:smoothness lemma 2}, we use the definition of $\Lagr'_\rho$ in \eqref{eq:ind Lagr prime} to write that 
%\begin{align}
%& \Lagr'_\rho(v^*,\lambda^*) - \Lagr'_\rho(v_{t},\lambda_{t}) - \langle v^*- v_{t}, \nabla_v \Lagr'_\rho(v_{t},\lambda_{t}) \rangle \nonumber\\
%& = L(w^*) - L(w_{t}) - \langle w^* - w_{t} , \nabla L(w_{t}) \rangle \nonumber\\
%& \qquad - \langle 
%A_t + DA(v_t)(v^*- v_{t})  
%,\lambda_{t} \rangle\nonumber\\
%& \qquad 
%- \frac{\rho}{2}\langle A_{t} + 2 DA(v_t) (v^* - v_{t}) , A_{t} \rangle,
%\label{eq:str cvx lem 0}
%\end{align}
%where 
%\begin{align}
%D A(v) & = \l[
%\begin{array}{cc}
%I_d & - DG(z)^\top 
%\end{array}
%\r]^\top,
%\label{eq:defn of Jacobian of A}
%\end{align}
%is the Jacobian of the map $A$. 
%The second inner product on the right-hand side of \eqref{eq:str cvx lem 0} can be bounded as 
%\begin{align}
%&  - \langle 
%A_t + DA(v_t)(v^*- v_{t})  
%,\lambda_{t} \rangle  \nonumber\\
%& =- \langle 
%w_{t}-G(z_{t}) + (w^*- w_{t}) - DG(z_{t})(z^* - z_{t})
%,\lambda_{t} \rangle \nonumber\\
%& = -\langle 
%G(z^*) -G(z_{t}) -  DG(z_{t})(z^* - z_{t})
%,\lambda_{t} \rangle 
%\qquad \l( w^* = G(z^*) \r) \nonumber\\
%& \ge -\l(\frac{\nu_G}{2} \|z_{t}-z^*\|_2^2  + \ol{\nu}_G \r) \|\lambda_{t}\|_2   
%\qquad \text{(see \eqref{eq:smoothness of G})} \nonumber\\
%& \ge -\l(\frac{\nu_G}{2} \|z_{t}-z^*\|_2^2 + \ol{\nu}_G\r)\lambda_{\max}.
%\qquad \text{(see \eqref{eq:dual seq})} 
%\label{eq:lwr bnd proof 0}
%\end{align}
%To control  the last  inner product on the right-hand side of  \eqref{eq:str cvx lem 0}, we write that 
%\begin{align}
%& \langle A_t + 2DA(v_t)(v^*-v_t), A_t \rangle  \nonumber\\
%& = \| A_t + DA(v_t) (v^*-v_t) \|_2^2 - \| DA(v_t)(v^*-v_t)\|_2^2 \nonumber\\
%& = \| A_t  - A(v^*) + DA(v_t) (v^*-v_t) \|_2^2 - \| DA(v_t)(v^*-v_t)\|_2^2 
%\qquad \l( A(v^*) = 0 \text{ by \eqref{eq:A_shorhtand}}\r)
%\nonumber\\
%& = \| (w_t - w^*) + (G(z^*) - G(z_t) - DG(z_t) (z^*-z_t) )  \|_2^2  - \| w^*-w_t\|_2^2 - \|  DG(z_t) (z^*-z_t) \|_2^2 
%\qquad \text{(see \eqref{eq:defn of Jacobian of A})}
%\nonumber\\
%& \ge \frac{1}{2}\|w_t - w^*\|_2^2 - \| G(z^*) - G(z_t) - DG(z_t)(z^*- z_t) \|_2^2 \nonumber\\
%& \qquad 
%- \|w^* - w_t\|_2^2 - \|DG(z_t) (z^* - z_t) \|_2^2 
%\qquad ( (a+b)^2 \ge \frac{a^2}{2}-b^2  ) \nonumber\\
%& \ge - \frac{1}{2}\|w_t - w^*\|_2^2 - ( \frac{\nu_G}{2}\|z_t - z^*\|_2^2 + \ol{\nu}_G )^2 - ( \kappa_G \|z_t - z^*\|_2^2 + \ol{\kappa}_G )^2 
%\end{align}
%
%uuuuu
%
%
% first observe that 
%\begin{align}
%-\frac{\rho}{2} \langle A_t +2 DA(v_t) (v^*-v_t), A_t \rangle = - \frac{\rho}{2} \langle A_t + 2 (w^*-w_t) , A_t \rangle
%+\rho \langle DG(z_t) (z^*-z_t), A_t \rangle.
%\qquad \text{(see (\ref{eq:defn of Jacobian of A}))}
%\label{eq:lwr bnd proof 1}
%\end{align}
%For the first term on the right-hand side above, we note that 
%\begin{align}
%& -  \langle A_{t}+2(w^* - w_{t}) , A_{t} \rangle  \nonumber\\
%& = - \langle w_{t} - G(z_{t}) + 2(w^* - w_{t}) , w_{t} - G(z_{t})\rangle 
%\qquad \text{(see (\ref{eq:defn of A}))}
%\nonumber\\
%& =  \langle G(z_{t}) - G(z^*) + (w_{t} - w^*) , (w_{t} - w^*) - (G(z_{t}) - G(z^*) ) \rangle 
%\qquad \l( w^* = G(z^*) \r)
%\nonumber\\
%& =  \|  (w_{t}- w^*) - (G(z_{t})-G(z^*)) \|_2^2 \nonumber\\
%& =  \| w_{t} - G(z_{t})\|_2^2
%\qquad \l( u^* = G(z^*) \r) \nonumber\\
%& =  \| A_{t}\|_2^2,
%\qquad \text{(see \eqref{eq:defn of A})}
%\label{eq:lwr bnd proof 2}
%\end{align}
%which in turn allows to revisit \eqref{eq:lwr bnd proof 1} and write that 
%\begin{align}
%& -\frac{\rho}{2} \langle A_t +2 DA(v_t) (v^*-v_t), A_t\rangle \nonumber\\
%& = - \frac{\rho}{2}\langle A_{t} + 2 (w^* - w_{t}) ,A_t \rangle +\rho \langle  DG(z_{t})( z^* - z_{t} ), A_{t}  \rangle 
%\qquad \text{(see (\ref{eq:lwr bnd proof 1}))}
%\nonumber\\ 
%& =  \frac{\rho}{2} \|A_{t}\|_2^2 + \rho \langle DG(z_{t})(z^* - z_{t}), A_{t} \rangle
%\qquad \text{(see (\ref{eq:lwr bnd proof 2}))}
% \nonumber\\
% & = \frac{\rho}{2}\l\| A_t + DG(z_t) (z^*-z_t)  \r\|_2^2 - \frac{\rho}{2}\| DG(z_t)(z^*-z_t) \|_2^2
% \nonumber\\
% & \ge  \frac{\rho}{2}\l\| A_t + DG(z_t) (z^*-z_t)  \r\|_2^2 - \frac{\rho}{2}(\kappa_G \|z_t - z^*\|_2 + \ol{\kappa}_G )^2 
%\qquad \text{(see (\ref{eq:smoothness of G 2}))} 
% \nonumber\\
% &=  \frac{\rho}{2}\l\| A_t - A(v^*) + DG(z_t) (z^*-z_t)  \r\|_2^2 - \frac{\rho}{2}(\kappa_G \|z_t - z^*\|_2 + \ol{\kappa}_G )^2  
% \qquad \l(  A(v^*) = 0  \text{ by \eqref{eq:A_shorhtand}}\r)
% \nonumber\\
% &=  \frac{\rho}{2}\l\| (w_t -w^*) +  G(z^*) - G(z_t) - DG(z_t) (z^*-z_t)  \r\|_2^2 - \frac{\rho}{2}(\kappa_G \|z_t - z^*\|_2 + \ol{\kappa}_G )^2  
% \nonumber\\ 
%& \ge \frac{\rho}{2} \|A_{t}\|_2^2  + \rho (\kappa_G \|z^* - z_{t}\|_2 + \ol{\kappa}_G ) \|A_{t}\|_2  
%\qquad \text{(see \eqref{eq:smoothness of G 2})} \nonumber\\
%& \le \rho \|A_{t}\|_2^2  + \frac{\rho}{2} (\kappa_G \|z^* - z_{t}\|_2 + \ol{\kappa}_G )^2  
%\qquad \l(2 ab\le a^2+b^2 \r)
% \nonumber\\
% & \le \rho \|A_{t}\|_2^2  + \rho \kappa^2_G \|z^* - z_{t}\|_2^2  + \rho \ol{\kappa}^2_G 
%\qquad \l( (a+b)^2\le 2a^2+2b^2 \r) \nonumber\\
%& = \rho \|(w_t - w^*) - (G(z_t) - G(z^*))\|_2^2  + \rho \kappa^2_G \|z^* - z_{t}\|_2^2  + \a\ol{\kappa}^2_G 
%\qquad \text{(see (\ref{eq:opt cnds},\ref{eq:defn of A}))}\nonumber\\
%& \le 2\rho \|w_t - w^*\|_2^2 + 2\rho\|G(z_t) - G(z^*)\|_2^2  + \rho \kappa^2_G \|z^* - z_{t}\|_2^2  + \rho\ol{\kappa}^2_G  
%\qquad \l( \|a+b\|_2^2 \le 2\|a\|_2^2+2\|b\|_2^2 \r)
%\nonumber\\
%& \le 2\rho \|w_t - w^*\|_2^2 + 2\rho ( \kappa_G \|z_t - z^*\|_2+ \ol{\kappa}_G )^2 + \rho \kappa^2_G \|z^* - z_{t}\|_2^2  + \rho\ol{\kappa}^2_G  
%\qquad \text{(see (\ref{eq:lipschitz of G 2}))} \nonumber\\
%& \le 2\rho \|w_t - w^*\|_2^2 +   5\rho \kappa^2_G  \|z_t - z^*\|_2^2 + 5\rho \ol{\kappa}^2_G.
%\qquad ( (a+b)^2 \le 2a^2+2b^2 ) 
%\label{eq:lwr bnd proof 3}
%\end{align}
%By substituting the bounds in  (\ref{eq:lwr bnd proof 0},\ref{eq:lwr bnd proof 3}) back into (\ref{eq:str cvx lem 0}) and also the convexity of $L$, we reach 
%\begin{align}
% \Lagr'_\rho(v^*,\lambda^*) - \Lagr'_\rho(v_t,\lambda_t) - \langle v^*- v_t, \nabla_v \Lagr'_\rho(v_t,\lambda_t)   \ge -   \frac{\omega_\rho}{2}\|w_t - w^*\|_2^2  -   \frac{\omega'_\rho}{2}\|z_t - z^*\|_2^2 - \ol{\omega}_\rho,
%\end{align}
%where 
%\begin{align}
%\omega_\rho := 4\rho ,
%\qquad 
%\omega'_\rho :=
%\nu_G \lambda_{\max} + 10\rho\kappa^2_G, 
%\end{align}
%\begin{align}
%\ol{\omega}_\rho := \ol{\nu}_G\lambda_{\max}+5\rho\ol{\kappa}^2_G. 
%\end{align}
%This proves \eqref{eq:smoothness lemma 2}, thus completing the proof of Lemma \ref{lem:str cvx}. 

\section{Relation with Gradient Descent \label{sec:gd-admm}}

%This section uncovers the relation between several first-order algorithms that have been proposed in the literature to solve Program~\eqref{eq:emp loss min}. Loosely speaking, we will establish that Algorithm~\ref{alg:admm} is closely related to previous algorithms, and that our convergence analysis in Section~\ref{sec:guarantees1} also applies to the algorithm proposed in \cite{Bora2017} without rates. We caution the reader that the discussion in this section is less formal by its nature. 
%
%Let us now turn to the details. 
Throughout this section, we set $R\equiv 0$ and $H\equiv 0$ in problem~\eqref{eq:emp loss min} and consider the updates in Algorithm~2, namely, 
\begin{equation}
\begin{split}
    z_{ t+1} &=  z_{ t} - \b \grad_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) , \\
    w_{ t+1} &\in \underset{w}{\operatorname{argmin}} \,\, \Lagr_\rho(w,z_{t+1},\lambda_t), \\
    \lambda_{t+1} &= \lambda_{ t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1})).
\end{split}
\label{eq:aug lagr alg full}
\end{equation}
From \eqref{eq:defn_aug_lagr}, recall that $\Lagr_\rho(w,z,\lambda)$ is convex in $w$ and the second step in \eqref{eq:aug lagr alg full} is therefore often easy to implement  with any over-the-shelf standard convex solver. 
 Recalling~(\ref{eq:defn_aug_lagr}), note also that the optimality condition for $w_{t+1}$ in \eqref{eq:aug lagr alg full} is  
\begin{align}
w_{t+1} - G(z_{t}) & = -\frac{1}{\rho}(\nabla L_m(w_{t+1})+ \lambda_t).
\label{eq:feas_to_grads}
\end{align}
Using \eqref{eq:defn_aug_lagr} again, we also write that 
\begin{align}
& \nabla_z \Lagr_\rho(w_{t+1},z_t,\lambda_t) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t +\rho (w_{t+1}-G(z_t)) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t  - \lambda_{t-1}- \nabla L_m(w_t)  ) \nonumber\\
& = - DG(z_t)^\top  ( \s_t (w_t - G(z_t)) - \nabla L(w_t)  ) ,
\label{eq:nablaL}
\end{align}
where the last two lines above follow from (\ref{eq:feas_to_grads},\ref{eq:aug lagr alg full}), respectively. Substituting back into the $z$ update in \eqref{eq:aug lagr alg full}, we reach
\begin{align}
z_{t+1} & = z_t + \b \s_t DG(z_t)^\top (w_t - G(z_t)) - \b \nabla L(w_t) 
\qquad \text{(see (\ref{eq:aug lagr alg full},\ref{eq:nablaL}))},
\label{eq:collapsed-admm}
\end{align}
from which it follows that 
\begin{align}
& \l\|z_{t+1}-(z_t -\b \nabla L(G(z_t)) )   \r\|_2 \nonumber\\
& \le \b\s_t \| DG(z_t)^\top (w_t - G(z_t)) \|_2+ \b \| \nabla L(w_t) - \nabla L( G(z_t) ) \|_2
\qquad \text{(see \eqref{eq:collapsed-admm})} \nonumber\\
& \le  \b \l( \s_t \kappa_G+ \nu_L \r) \| w_t - G(z_t) \|_2 .
\qquad \text{(see Assumptions \ref{assump:risk} and \ref{defn:G_iso})}
\end{align}
That is, as the feasibility gap vanishes in \eqref{eq:feas-thm} in Theorem \ref{thm:main},  the updates of Algorithm 2 match those of GD.
%
%When $t\gg 1$, the choice of dual step sizes in Algorithm~\ref{alg:admm} satisfies $\s_t\|w_t - G(z_t)\|_2 \approx 0$. Therefore, the $z$ update in \eqref{eq:aug lagr alg full} simplifies to 
%\begin{align}
%z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(w_t),
%\label{eq:z_approx}
%\end{align}
%provided that $G$ is sufficiently smooth. 
%In addition, when $\rho \gg 1$, the $w$ update in \eqref{eq:aug lagr alg full} ensures that $w_t \approx G(z_t)$ which, together with \eqref{eq:z_approx},  implies that 
%\begin{align}
%z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(G(z_t)), 
%\label{eq:grad_step}
%\end{align}
%if the  prior $G$ and empirical loss $L_m$ are sufficiently smooth. Note that \eqref{eq:grad_step} corresponds to one step of gradient descent (GD) with step size $\b$ applied to the program 
%\begin{align}
%\min_z \,\,L_m(G(z)),
%\label{eq:parameter_space}
%\end{align}
%which is equivalent to Program~\eqref{eq:emp loss min} with $R=H=0$. That is, for a sufficiently large penalty weight, the updates in \eqref{eq:aug lagr alg full} approximately coincide  with those in GD applied to  Program~\eqref{eq:parameter_space}. Since the updates in \eqref{eq:aug lagr alg full} can only improve over Algorithm~\ref{alg:admm}, the convergence rate in Section~\ref{sec:guarantees1} also applies to GD for Program~\eqref{eq:parameter_space}, thereby providing convergence rate as a special case for the algorithm introduced in~\citet{Bora2017} without supporting theory. 


\section{Proof of Lemma \ref{lem:ws_to_wn} \label{sec:proof of ws_to_wn}}

Recall that $R=1_W$ and $H\equiv 0$ for this proof. Using the optimality of $w^*\in\text{relint}(W)$ in~\eqref{eq:emp loss min supp}, we can write that 
\begin{align}
\| \nabla L(w^*) \|_2 & \le \| \nabla L_m(w^*) \|_2 + \| \nabla L_m(w^*) - \nabla L(w^*) \|_2
\qquad 
\text{(triangle inequality)} \nonumber\\
& =  \| \nabla L_m(w^*) - \nabla L(w^*) \|_2
\qquad \l( \nabla L_m(w^*) = 0  \r) \nonumber\\
& \le \max_{w\in W}\| \nabla L_m(w) - \nabla L(w) \|_2.
\label{eq:near_st}
\end{align}
On the other hand, using the strong convexity of $L$ in \eqref{eq:L_str_cvx_supp}, we can write that 
\begin{align}
\| w^\n - w^* \|_2 &
\le \frac{1}{\zeta_L} \| \nabla L(w^\n) - \nabla L(w^*) \|_2 
\qquad \text{(see \eqref{eq:L_str_cvx_supp})}
\nonumber\\
& = \frac{1}{\zeta_L} \|\nabla L(w^*) \|  
\qquad (\nabla L(w^\n) = 0 )
\nonumber\\
& \le \frac{1}{\zeta_L} \max_{w\in W}\| \nabla L_m(w) - \nabla L(w) \|_2,
\qquad \text{(see \eqref{eq:near_st})}
\end{align}
which completes the proof of Lemma \ref{lem:ws_to_wn}. 

==> sections/conclusion.tex <==
We evaluated the a linearized ADMM and its partial exact minimization variant EADMM
on the compressive sensing tasks and $\ell_1$ denoising tasks.


==> sections/experiments.tex <==
We now benchmark the following algorithms for solving problem \eqref{eq:final_problem}:
\begin{itemize}
    \item \textbf{Gradient Descent (GD): } \citep{Bora2017} Perform a fixed
        number of gradient descent iterations for the function
        $\loss(G(\prior))$.

    \item \textbf{Projected Gradient Descent (PGD): } \citep{Shah2018,
        Hegde2018} Performs a step in the direction of the gradient of
        $\loss(w)$ and the resulting iterate $w'$ is projected back to
        $G(z)$ via minimization of the function $\norm{G(z) - w'}_2^2$. This
        projection step is approximately achieved via a fixed number of
        gradient descent iterations.

    \item \textbf{Inexact ADMM (IADMM): } \ref{alg:admm} (Ours).

    \item \textbf{Partial exact minimization ADMM (PADMM): } Our algorithm
        \ref{alg:admm} with the following change: we perform exact minimization
        on the primal variable $w$. For example, in the
        linear regression case this involves one matrix inversion per
        iteration. Performing SVD once on the measurement matrix $X$ allows us
        to perform such inversion with small overhead per iteration.
\end{itemize}

We now describe the generator architecture $G$, for each of the test datasets
that we consider:
\begin{itemize}
    \item \textbf{MNIST:} We use the same architecture as one in \cite{gulrajani2017improved},
        which contains one fully-connected layer followed by three deconvolutional layers.
    \item \textbf{LSUN \& CelebA:} As a practice in \cite{gulrajani2017improved},
        we downsampled the images into $64 \times 64$ pixels and use the same generator architecture.
        The generator networks includes 4 residual blocks followed by a convolutional layer.
\end{itemize}

Notice that in the the \textit{Deep Image Prior} setting, we use the
network architecture initialized with random weight matrices. We consider
three different tasks: $(i)$ Linear regression with generative prior (LIN-G),
$(ii)$ Phase retrieval with generative prior (PHASE-G), and $(iii)$
Linear Regression with deep image prior (LIN-DIP). For MNIST we run the
algorithms for $4000$ iterations using either $100$, $200$ or $400$ measurements.
For the CelebA and LSUN datasets we use $8000$ iterations using either
$200$, $800$ or $1600$ measurements. For the (LIN-G) and (PHASE-G) tasks, we
consider two scenarios for the test images: either we choose random images from
a test set, not used for the training of the generative model, or we choose
random images on the image of the generative model, by choosing random latent
vectors $z$. For the (LIN-DIP) task we consider only images on a test set.

%\begin{figure}[H]
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/originals.png}
%    \label{fig:1}
%  \end{subfigure}
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/gd.png}
%    \label{fig:2}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/admm.png}
%    \label{fig:3}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/eadmm.png}
%    \label{fig:4}
%  \end{subfigure}%
%
%    \begin{subfigure}{\linewidth}
%    \centering
%    \includegraphics[width=.7\linewidth]{\mnistreallineartwohundredelu/pgd.png}
%    \label{fig:5}
%  \end{subfigure}%
%
%  \caption{Recovered test images from 200 linear measurements. MNIST dataset.
%  From top to bottom: Original images, GD, IADMM (ours), PADMM (ours), PGD.}
%  \label{fig:images}
%\end{figure}
%
%\begin{figure}[H]
%    \centering
%    \includegraphics[width=\linewidth]{\comparisonfolder/4000_mnist_comparison.pdf}
%    \label{fig:mnist_comparison}
%
%    \caption{Function value across iterations for task (LIN-G). Recovering images on the test set (top).
%    Recovering images on the range of the generator (bottom).}
%  \label{fig:images}
%\end{figure}


==> sections/guarantees2.tex <==

Building upon the results in Section~\ref{sec:guarantees1}, the main result in this section (Theorem~\ref{thm:main_stat}) quantifies the convergence of the iterates $\{w_t\}_{t\ge 0}$ of Algorithm~\ref{alg:admm} to the true parameter $w^\n$. 


In other words, Theorem~\ref{thm:main_stat} below controls the generalization error of Program~\eqref{eq:emp loss min}, namely, the error  incurred by using the empirical risk $L_m$ in lieu of the population risk $L$. Indeed, Theorem~\ref{thm:main} is  silent about $\|w_t - w^\n\|_2$.  We address this shortcoming with the following result, proved in Section~\ref{sec:proof of ws_to_wn} of the supplementary material.  
\begin{lemma}\label{lem:ws_to_wn}
Let $R=1_W$ be the indicator function on $W\subset\R^p$ and set $H=0$ in Program~(\ref{eq:emp loss min}).\footnote{To be complete, $1_W(w)=0$ if $w\in W$ and $1_W(w)=\infty$ otherwise. } Suppose that $w^*$ belongs to the relative interior of $W$. 
%\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ denotes the relative interior of the set $W$.  
Then it holds that 
\begin{align}
\|w^\n - w^*\|_2 \le \frac{1}{\zeta_L} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w) \|_2.
\label{eq:before_Upsilon}
\end{align}
\end{lemma}
Before bounding the right-hand side of \eqref{eq:before_Upsilon}, we remark that it is possible to extend Lemma~\ref{lem:ws_to_wn} to the case where the regularizer $R$ is a \emph{decomposable} norm, along the lines of~\cite{negahban2012unified}. We will however not pursue this direction in the present work. 
Next note that \eqref{eq:linr_cvg_thm} and Lemma~\ref{lem:ws_to_wn} together imply that 
\begin{align}
& \| w_t - w^\n\|_2^2  \nonumber\\
& \le ( \|w_t - w^*\|_2+ \|w^* - w^\n\|_2  )^2 
\qquad \text{(triangle inequality)} \nonumber\\
& \le 2 \|w_t - w^*\|_2^2 + 2 \|w^*-w^\n\|_2^2
\quad ( (a+b)^2 \le 2a^2+2b^2  )
 \nonumber\\
& \le 2\eta_{\rho}^t\widetilde{\Delta}_0 
+ 2\widetilde{\psi}_\rho \nonumber\\
& \qquad 
+ \frac{2}{\zeta_L^2} \max_{w\in W} \| \nabla L_m(w) - \nabla L(w)\|_2^2. 
\label{eq:before_rademacher}
\end{align}
According to Theorem~\ref{thm:main}, the right-hand side of \eqref{eq:before_rademacher} depend on $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$, which were introduced in Definition~\ref{defn:Lm_scvx}, with the exact dependence specified in the proof of the theorem. Note that $\mu_L,\ol{\mu}_L,\nu_L,\ol{\nu}_L$  and the right-hand side of \eqref{eq:before_Upsilon} are all random variables because they depend on $L_m$ and thus on the randomly drawn training data $\{x_i\}_{i=1}^m$. To address this issue,  we apply a basic result in statistical learning theory as follows. For every $w\in \R^p$ and every pair $x,x'\in \mathbb{X}$, we use Assumption~\ref{assump:props_of_l} to write that 
\begin{align}
\| \nabla l(w,x) - \nabla l(w,x') \|_2 & \le \s_l \| x-x'\|_2
\qquad \text{(see \eqref{eq:props_of_l})} \nonumber\\
& \le \s_l \text{diam}(\mathbb{X}),
\end{align}
where $\text{diam}(\mathbb{X})$ denotes the diameter of the compact set $\mathbb{X}$. Note also that 
\begin{align}
\E_{\{x_i\}_i} \nabla L_m(w) = \nabla L(w), 
\qquad \forall w\in W,
\end{align}
where the expectation is over the training data $\{x_i\}_i$. 
Then, for $\varepsilon>0$ and except with a probability of at most $e^{-\varepsilon}$, it holds that 
\begin{align}
& \| \nabla L_m(w) - \nabla  L(w) \|_2  \nonumber\\
& \le 2 \mathcal{R}_W(x_1,\cdots,x_m) +3\s_l\text{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}} \nonumber\\
& =: \Upsilon_{m,W}(\varepsilon),
\label{eq:emp_proc}
\end{align}
for every $w\in W$~\cite{mohri2018foundations}. Above, 
\begin{align}
& \mathcal{R}_W(x_1,\cdots,x_m) \nonumber\\
& = 
\E_{E} \l[ \max_{w\in W}    \l \| \frac{1}{m} \sum_{i=1}^{m} e_i \nabla_w l(w,x_i)\r \|_2 \r],
\label{eq:emp rademach}
\end{align}
is the \emph{empirical Rademacher complexity} and $E=\{e_i\}_i$ is a Rademacher sequence, namely, a sequence of independent random variables taking $\pm 1$ with equal probabilities.  We can now revisit \eqref{eq:before_rademacher} and write that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le 2\eta_{\rho}^t\widetilde{\Delta}_0  + 
2\widetilde{\psi}_\rho + \frac{2\Upsilon_{m,W}^2(\varepsilon)}{\zeta_L^2},
\end{align}
which holds except with a probability of at most $e^{-\varepsilon}$. In addition, for every $w,w'\in W$, we may write that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \le   \| \nabla L(w) - \nabla L(w')\|_2+ \| \nabla L_m(w) - \nabla L(w) \|_2\nonumber\\
& \qquad  + \| \nabla L_m(w') - \nabla L(w')\|_2
\quad \text{(triangle inequality)} \nonumber\\
& \le  \s_L\|w-w'\|_2+  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx},\ref{eq:emp_proc} ))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. 
Likewise, for every $w,w'\in W$, we have that 
\begin{align}
& \| \nabla L_m(w) - \nabla L_m(w') \|_2  \nonumber\\
& \ge \| \nabla L_m(w) - \nabla L_m(w) \|_2  -  \| \nabla L_m(w) - \nabla L(w)\|_2\nonumber\\
& \qquad - \| \nabla L_m(w') - \nabla L(w')\|_2
\qquad \text{(triangle inequality)} \nonumber\\
& \ge  \zeta_L\|w-w'\|_2-  2\Upsilon_{m,W}(\varepsilon),
\qquad \text{(see (\ref{eq:L_str_cvx},\ref{eq:emp_proc} ))}
\end{align} 
except with a probability of at most $e^{-\varepsilon}$. Therefore, $L_m$ satisfies the restricted strong convexity and smoothness in Definition~\ref{defn:Lm_scvx} with
\begin{align}
\mu_L = \s_L,
\qquad 
\nu_L = \zeta_L,
\nonumber\\
\ol{\mu}_L = \ol{\zeta}_L =  2\Upsilon_{m,W}(\varepsilon). 
\end{align}
%Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold. These findings are summarized below in our second main result.  For a convex set $W\subset\R^p$, let  $R=1_W$  be the (convex) indicator function on $W$ and set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of Program~(\ref{eq:emp loss min}) satisfies $w^*\in \operatorname{relint}(W)$, where $\operatorname{relint}(W)$ is the relative interior of the set $W$.  
Our findings in this section are summarized below. 
\begin{theorem} \label{thm:main_stat}\textbf{\emph{(Generalization error)}} 
Suppose that Assumptions~\ref{defn:Lm_scvx}-\ref{defn:G_iso} hold and recall that the training samples $\{x_i\}_{i=1}^m$ are drawn independently from the probability space $(\mathbb{X},\chi)$ for a compact set $\mathbb{X} \subset \R^d$  with diameter $\operatorname{diam}(\mathbb{X})$.   

For a set $W\subset\R^p$, let  $R=1_W$  be the indicator function on $W$, and set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of Program~(\ref{eq:emp loss min}) belongs to the relative interior of $W$. 
For $\varepsilon>0$, evaluate the quantities in Theorem~\ref{thm:main} with 
\begin{align}
\mu_L & = \s_L,
\qquad 
\nu_L = \zeta_L, \nonumber\\
\ol{\mu}_L & = \ol{\zeta}_L =   
4 \mathcal{R}_W(x_1,\cdots,x_m) \nonumber\\
& \qquad +6\s_l\operatorname{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}},
\end{align}
where $\mathcal{R}_W(x_1,\cdots,x_m)$ in the empirical  Rademacher complexity defined in (\ref{eq:emp loss min}). If the requirements on the step sizes in~(\ref{eq:step_size_reqs_thm}) hold, we then have that 
\begin{align}
\|w_t- w^\n \|_2^2  & 
\le   2\eta_{\rho}^t\widetilde{\Delta}_0   + 
2\psi_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2  \nonumber\\
& \qquad +  \frac{18\s_l^2 \operatorname{diam}(\mathbb{X})^2( \varepsilon+2)}{m}, 
\end{align}
 except with a probability of at most $e^{-\varepsilon}$. 
\end{theorem}
Most of the remarks about Theorem~\ref{thm:main} also apply to Theorem~\ref{thm:main_stat} and we note that $\|w_t-w^\n\|_2$ reduces by increasing the number of training samples $m$, before asymptotically reaching the generalization error
\begin{align}
2\psi_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2.
\label{eq:statistical ball}
\end{align}
Computing the Rademacher complexity above for specific choices of the network structure and loss is itself potentially a complicated task, which we will not pursue by the virtue of the generality of our results so far. The key technical challenge there is computing the corresponding \emph{entropy integral}, which involves estimating the \emph{covering numbers} of the set $W$ \cite{mohri2018foundations}. One last takeaway point from the statistical accuracy in \eqref{eq:statistical ball} is the following. If  
\begin{align}
\psi_\rho=O(\mathcal{R}_W(x_1,\cdots,x_m)^2/\zeta_L^2),
\label{eq:statistacll ball 2}
\end{align}
the asymptotic optimization error  in Theorem~\ref{thm:main} does not play an important role in determining the generalization error above. In words, i \eqref{eq:statistacll ball 2} holds, then Algorithm~\ref{alg:admm} converges to the ball of statistical accuracy around $w^\n$. Here, $O$ stands for the standard Big-O notation. 





==> sections/guarantees_temp.tex <==
\section{Convergence Rate \label{sec:cvg rate}}

In this section, we investigate the convergence rate of our algorithm for finding first-order and second-order stationary points, along with iteration complexity results.
The proofs are deferred to Appendix~\ref{sec:theory} for clarity of exposition.

\subsection{Complexity results for first-order stationarity}
Theorem~\ref{thm:main} characterizes the convergence rate of Algorithm~\ref{Algo:2} for finding first-order stationary points in terms of the number of outer iterations.\\
{\color{red}{Ahmet: I think that it is possible to remove sufficiently large k0 assumption here. }}
\begin{theorem}
\label{thm:main}
In addition to the smoothness of $f$ and $A$ as in (\ref{eq:smoothness basic}) and for $\rho'>0$, let us define 
\begin{align}
\lambda'_f = \max_{\|x\|\le \rho'} \|\nabla f(x)\|,
~~
\lambda'_A = \max_{\|x\| \le \rho'} \|DA(x)\|,
\end{align}
to be the (restricted) Lipschitz constants of $f$ and $A$, respectively. 
 For sufficiently large integers $k_0\le k_1$, consider the interval $K=[k_0:k_1]$.  Let $\{x_k\}_{k\in K}$ be the output sequence of Algorithm~\ref{Algo:2} and, for $\nu>0$, assume that 
 \begin{align}
\nu \|A(x_k)\|  
& \le \dist\left( -DA(x_k)^\top A(x_k) , \frac{\partial g(x_k)}{ \b_{k-1}}  \right), 
\label{eq:regularity}
\end{align}
for every $k\in K$. 
Then the output of Algorithm~\ref{Algo:2} satisfies 
\begin{align}
& \dist^2( -\nabla_x \L_{\b_{k-1}}(x_k,y_k),\partial g(x_k)) + \| A(x_k)\|^2   \nonumber\\
& = \frac{1}{\b_{k-1}^2}\left( \frac{8 \lambda'_A\s_k^2 + 4}{ \nu^2} ( \lambda'_f+\lambda'_A y_{\max})^2 + 2\right) \nonumber \\ 
&=: \frac{Q}{\beta_{k-1}^2}. 
\end{align}
\end{theorem}
A few remarks are in order about Theorem~\ref{thm:main}. 

\textbf{Tradeoff.}
Roughly speaking, Theorem~\ref{thm:main} states that the iterates of Algorithm~\ref{Algo:2} approach first-order stationarity for~\eqref{prob:01} at the rate of $1/{\b_k}$, where $\b_k$ is the penalty weight in AL in iteration $k$ as in~\eqref{eq:Lagrangian}. Note the inherent tradeoff here: For a faster sequence $\{\b_k\}_k$, the iterates approach stationarity faster but the computational cost of the inexact primal subroutine (Step 2) increases since a higher accuracy is required and Lipschitz constant of the unconstrained problem is also affected by $\beta_k$. In words, there is a tradeoff between the number of outer and inner loop iterations of Algorithm~\ref{Algo:2}. We highlight this tradeoff for a number of subroutines below.

First, we characterize the iteration complexity of Algorithm~\ref{Algo:2} for finding a first-order stationary point of~\eqref{prob:01}.
We propose to use the standard accelerated proximal method (APGM), guarantees of which are analyzed in~\cite{ghadimi2016accelerated} for nonconvex problems of the form~\eqref{e:exac}.
They show that APGM can find $\epsilon$ first-order stationary point in 
\begin{equation}
\mathcal{O}\left ( \frac{\lambda_\beta^2\left( \|x^\star \|^2 + M^2 \right)}{\epsilon} \right)
\end{equation}
iterations, where $\lambda_\beta$ denotes the Lipschitz constant of the gradient of ${\mathcal{L}_{\beta}(x, y)}$ as in~\eqref{eq:smoothness of Lagrangian} and $M$ is defined with the following bound:
%
\begin{equation}
\min_{\text{dom}\{g\}}\|x\| \leq M.
\end{equation}
%
Using this result, we can get the following corollary describing the iteration complexity in terms of the calls to the first-order oracle:

\begin{corollary}\label{cor: first_order}
Let us use the following form for $\beta$
\begin{equation*}
\beta_k = \alpha^k, ~~ \alpha > 1.
\end{equation*}

If we use APGM from~\cite{ghadimi2016accelerated} for step 2 in Algorithm~\ref{Algo:2}, it finds an $\epsilon$-first-order stationary point in the sense that
\begin{equation}
\dist(-\nabla_x \mathcal{L}_\beta(x,y), \partial g(x)) \leq \epsilon, ~~~~
A(x) = 0 \leq \epsilon,
\end{equation}
in $T_K$ number of calls to the first-order oracle, where

\begin{equation}
T_K \leq \tilde{\mathcal{O}} \left( \frac{Q^{\frac{3}{2}}(\|x^\star\|^2 + M^2)}{\epsilon^{3}} \right).
\end{equation}
\end{corollary}


\subsection{Complexity results for second-order stationarity}
{\color{red}{Ahmet (note to myself): not sure of the constants of trust-region, check again}} \\
In this subsection, we focus on finding second-order stationary points of~\eqref{prob:01}.
For this purpose, we need to use a subroutine in Step 2 of Algorithm~\ref{Algo:2} to find approximate second-order stationary points of the subproblem~\eqref{e:exac}.
As shown in~\cite{nouiehed2018convergence}, finding approximate second-order stationary points for constrained problems is in general NP-hard.
For this reason, we focus on the special case of~\eqref{prob:01} with $g=0$ in this section.

In this case, we focus on find second-order stationary points of~\eqref{prob:01} in the sense of~\eqref{eq:sec_opt}.

We first give a theorem to show the convergence rate of the algorithm for second order stationarity: \\
{\color{red}{Ahmet: I think that it is possible to remove sufficiently large k0 assumption here. }} 
\begin{corollary}
\label{thm:main_second}
Under the assumptions of Theorem~\ref{thm:main}, the output of Algorithm~\ref{Algo:2} satisfies 
\begin{align}
%& \dist^2( -\nabla_x \L_{\b_{k-1}}(x_k,y_k),\partial g(x_k)) + \| A(x_k)\|^2   \nonumber\\
%& = \frac{1}{\b_{k-1}^2}\left( \frac{8 \lambda'_A\s_k^2 + 4}{ \nu^2} ( \lambda'_f+\lambda'_A y_{\max})^2 + 2\right) \nonumber \\ 
%&=: \frac{Q}{\beta_{k-1}^2}. 
\lambda_{\text{min}}(\nabla _{xx}\mathcal{L}_{\beta_{k-1}}(x_k, y_k)) \geq - \frac{C}{\beta_{k-1}} - \epsilon_{k-1}.
\end{align}
\end{corollary}
%
We now focus on total complexity of finding second-order stationary points of~\eqref{prob:01} in terms of calls to the second-order oracle.
We consider using trust region method for Step 2 of Algorithm~\ref{Algo:2} developed in~\cite{cartis2012complexity}.
In~\cite{cartis2012complexity}, the complexity for finding the second order stationary points of an unconstrained problem is derived to be
%
\begin{equation}
\mathcal{O}\left ( \frac{\lambda_{\beta, H}^2 (\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y))}{\epsilon^3} \right),
\end{equation}
%
where $\lambda_{\beta, H}$ is the Lipschitz constant of the Hessian of the augmented Lagrangian, which is of the order of $\beta$.
In~\cite{cartis2012complexity}, the term $\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y)$ is bounded by a constant independent of $\epsilon$.
We have a similar assumption for this quantity $\forall \beta_k$.

Consequently, we get the following result:
%
\begin{corollary}\label{cor: second_order}
Let us use the following form for $\beta$
\begin{equation*}
\beta_k = \alpha^k, ~~ \alpha > 1.
\end{equation*}
%
We use the trust region method from~\cite{cartis2012complexity} for step 2 in Algorithm~\ref{Algo:2} and assume that 
\begin{equation}
\mathcal{L}_{\beta}(x_1, y) - \min_{x}\mathcal{L}_{\beta}(x, y)
\end{equation}
is upper bounded by a constant independent of $\epsilon$.
Algorithm~\ref{Algo:2} then finds an $\epsilon$-second-order stationary point of~\eqref{prob:01} in $T_K$ total number of calls to the second order oracle where
%
\begin{equation}
T_K \leq \tilde{\mathcal{O}}\left( \frac{Q^{\frac{5}{2}}}{\epsilon^{5}} \right).
\end{equation}
\end{corollary}
%
{\color{red} Ahmet: I'll check again the constants of the corollaries, eps dependence should be correct.}\\
%
\textbf{Regularity.}  The key condition in Theorem~\ref{thm:main} is \eqref{eq:regularity}. As the penalty weight $\b_k$ grows, the primal subroutine (Step 2) places an increasing emphasis on reducing the feasibility gap and \eqref{eq:regularity} formalizes this intuition. We verify this condition rigorously in several examples in Section~\ref{sec:experiments}. 

We argue that such a condition is necessary for controlling the feasibility gap of~\eqref{prob:01} and ensuring the success of Algorithm~\ref{Algo:2}. To motivate this condition, recall the Slater's condition for $g(\cdot) = \delta_{\mathcal{X}}(\cdot)$ which states that
\begin{equation}
\text{relint} (\mathcal{X}) \cap \{ x\in\mathbb{R}^d: A(x) = b \} \neq \emptyset.
\end{equation}
This condition plays a key role in convex optimization since it is a sufficient condition for strong duality. 
As a result, Slater's condition guarantees the success of a variety of primal-dual algorithms for linearly constrained convex optimization.

As a visual example, in~\eqref{prob:01}, we consider the case where $f=0$,  $g=\delta_\mathcal{X}$ where $\mathcal{X}$ is a convex set, and $A$ is a linear  operator. 
Slater's condition removes any pathological cases by ensuring that the affine subspace is not tangent to $\mathcal{X}$, see Figure~\ref{fig:convex_slater}.  
In such pathological cases, finding a feasible point of~\eqref{prob:01} is particularly difficult. 
For example, the iterates of the alternating projection algorithm (which iteratively projects onto $\null(A)$ and $\mathcal{X}$) have arbitrarily slow convergence, as show in Figure~\ref{fig:conve_slater}.

{\color{red}{We should add a figure here with circle and line.}}




==> sections/relations.tex <==
This section uncovers the relation between several first-order algorithms that have been proposed in the literature to solve Program~\eqref{eq:emp loss min}. Loosely speaking, we will establish that Algorithm~\ref{alg:admm} is closely related to previous algorithms, and that our convergence analysis in Section~\ref{sec:guarantees1} also applies to the algorithm proposed in \cite{Bora2017} without rates. We caution the reader that the discussion in this section is less formal by its nature. 

Let us now turn to the details. 
Throughout this section, we set $R=H=0$ in Program~\eqref{eq:emp loss min} since the current literature for deep-net priors in unable to provably and efficiently handle nonsmooth regularizers, to the best of our knowledge, unlike Algorithm~\ref{alg:admm}. Instead of the (linearized) updates in Algorithm~\ref{alg:admm}, consider the updates 
\begin{equation}
\begin{split}
    z_{ t+1} &=  z_{ t} - \b \grad_{z} \Lagr_{\rho} (w_{t}, z_{t},  \lambda_{t}) , \\
    w_{ t+1} &\in \underset{w}{\operatorname{argmin}} \,\, \Lagr_\rho(w,z_{t+1},\lambda_t), \\
    \lambda_{t+1} &= \lambda_{ t} + \sigma_{t+1}  (w_{t+1}-G(z_{t+1})).
\end{split}
\label{eq:aug lagr alg full}
\end{equation}
From \eqref{eq:defn_aug_lagr}, recall that $\Lagr_\rho(w,z,\lambda)$ is convex in $w$ and the second step in \eqref{eq:aug lagr alg full} is therefore often easy to implement  with any over-the-shelf standard convex solver. 
 Recalling~(\ref{eq:defn_aug_lagr}), note also that the optimality condition for $w_{t+1}$ in \eqref{eq:aug lagr alg full} is  
\begin{align}
w_{t+1} - G(z_{t}) & = -\frac{1}{\rho}(\nabla L_m(w_{t+1})+ \lambda_t).
\label{eq:feas_to_grads}
\end{align}
Using \eqref{eq:defn_aug_lagr} again, we also write that 
\begin{align}
& \nabla_z \Lagr_\rho(w_{t+1},z_t,\lambda_t) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t +\rho (w_{t+1}-G(z_t)) \nonumber\\
& = - DG(z_t)^\top ( \lambda_t  - \lambda_{t-1}- \nabla L_m(w_t)  ) \nonumber\\
& = - DG(z_t)^\top  ( \s_t (w_t - G(z_t)) - \nabla L_m(w_t)  ) ,
\end{align}
where the last two lines above follow from (\ref{eq:feas_to_grads},\ref{eq:aug lagr alg full}), respectively. When $t\gg 1$, the choice of dual step sizes in Algorithm~\ref{alg:admm} satisfies $\s_t\|w_t - G(z_t)\|_2 \approx 0$. Therefore, the $z$ update in \eqref{eq:aug lagr alg full} simplifies to 
\begin{align}
z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(w_t),
\label{eq:z_approx}
\end{align}
provided that $G$ is sufficiently smooth. 
In addition, when $\rho \gg 1$, the $w$ update in \eqref{eq:aug lagr alg full} ensures that $w_t \approx G(z_t)$ which, together with \eqref{eq:z_approx},  implies that 
\begin{align}
z_{t+1} \approx z_t - \b DG(z_t)^\top \nabla L_m(G(z_t)), 
\label{eq:grad_step}
\end{align}
if the  prior $G$ and empirical loss $L_m$ are sufficiently smooth. Note that \eqref{eq:grad_step} corresponds to one step of gradient descent (GD) with step size $\b$ applied to the program 
\begin{align}
\min_z \,\,L_m(G(z)),
\label{eq:parameter_space}
\end{align}
which is equivalent to Program~\eqref{eq:emp loss min} with $R=H=0$. That is, for a sufficiently large penalty weight, the updates in \eqref{eq:aug lagr alg full} approximately coincide  with those in GD applied to  Program~\eqref{eq:parameter_space}. Since the updates in \eqref{eq:aug lagr alg full} can only improve over Algorithm~\ref{alg:admm}, the convergence rate in Section~\ref{sec:guarantees1} also applies to GD for Program~\eqref{eq:parameter_space}, thereby providing convergence rate as a special case for the algorithm introduced in~\citet{Bora2017} without supporting theory. 


The next observation highlights the relation between GD in \eqref{eq:grad_step} (with exact equality therein) and the Projected Gradient Descent (PGD) applied to Program~\eqref{eq:emp loss min}. Indeed, with  the step size $\alpha_{\operatorname{pgd}}>0$, an iteration of PGD is specified as 
\begin{align}
w_{t+1} & \in  \Proj_G(w_t - \a_{\operatorname{pgd}} \nabla L_m(w_t) ) \nonumber\\
& = \Proj_G( G(z_t) - \alpha_{\operatorname{pgd}} \nabla L_m(G(z_t)) ), 
\label{eq:PGD update}
\end{align}
where the possibly set-valued operator $\Proj_G:\R^p\rightarrow\R^p$ denotes the projection onto the  prior, taking $w\in \R^p$ to 
\begin{align}
\Proj_G(w) & = 
\underset{z}{\operatorname{argmin}}\,\, \frac{1}{2}\| w - G(z)\|^2_2,
\label{eq:proj_gan}
\end{align}
and $z_t$ satisfies $w_t = G(z_t)$. 
Program~\eqref{eq:proj_gan} can be solved numerically by GD, for instance, to first-order stationarity. Initialized at $z_t$ and with the step size of $\alpha_{\operatorname{proj}}>0$,  the first iterate of gradient descent for computing $w_{t+1}$ in \eqref{eq:PGD update}  takes $z_t$ to 
\begin{align}
z_t - \alpha_{\operatorname{proj}} \alpha_{\operatorname{pgd}} DG(z_t)^\top 
 \nabla L_m (G(z_t)), 
\end{align}
which coincides with the right-hand side of \eqref{eq:grad_step} with the choice of $\b= \alpha_{\operatorname{proj}}\alpha_{\operatorname{pgd}}$. That is, the first iterate of PGD for solving Program~\eqref{eq:emp loss min} matches the first GD update for Program~\eqref{eq:parameter_space}.



==> sections/setup.tex <==
For the sake of completeness, in this section we provide a more detailed problem formulation, which follows the standard setup in learning theory~\cite{mohri2018foundations}. 
Consider the probability space $(\mathbb{X}, \chi)$, where
$\mathbb{X} \subset \R^d$ is a compact set, equipped with the Borel sigma
algebra, and $\chi$ is the corresponding probability measure. To learn an
unknown parameter $w^\n \in \R^d$, consider the optimization program
\begin{align}
\underset{w\in \R^p}{\text{min}} \,\,  L(w),
\qquad
L(w) := \E_{x \sim \chi} l(w,x),
\label{eq:pop loss min}
\end{align}
where $L:\R^p\rightarrow \R$ is the differentiable \textit{population risk}
and $l:\R^d \times \R^p \rightarrow\R$ is the corresponding \emph{loss function}. We
also assume that Program \eqref{eq:pop loss min} has a unique solution $w^\n\in
\R^p$. The probability measure $\chi$ above is itself often unknown and we instead
have access to $m$ samples drawn independently from $\chi$, namely,
$\{x_i\}_{i=1}^m \sim \chi$. This allows us to form the \emph{empirical loss}
\begin{align}
L_m(w) := \frac{1}{m} \sum_{i=1}^m l(w,x_i).
\label{eq:emp loss defn supp}
\end{align}
Often, $m \ll p$ and to avoid an ill-posed problem, we must leverage any
inherent structure in $w^\n$. In this work, we consider a differentiable map
$G: \R^s \to \R^d$ and we assume that $w^\n \in G(\R^s)$.  That is,
there exists $z^\n \in \R^s$ such that $w^\n = G(z^\n)$. While not necessary, we limit ourselves in this paper to the important case where $G$ corresponds to a deep neural network, a GAN for instance. 

The defferentiability assumption on $G$ is not
restrictive. For example, the non-differentiable ReLU activation function in a GAN can be  replaced with its smooth alternative ELU \citep{clevert2015fast}, which only differs
 from ReLU near the origin. In our experiments, we were able to succesfully train GANs with ELU activation function. \citet{gulrajani2017improved} also reports
successful training of GANs with another differentiable activation function. See also the discussion after Assumption~\ref{assump:G_ssmth}. 

To learn $w^\n$ with the deep-net prior $w^\n=G(z^\n)$,  we propose
to solve the program
\begin{align}
\begin{array}{lll}
\underset{w,z}{\text{minimize}} & & L_m(w) + R(w) + H(z)\\
\text{subject to } & & w = G(z),
\end{array}
\label{eq:emp loss min supp}
\end{align}
where $R:\R^p \rightarrow \R$ and $H: \R^s \rightarrow \R$ are convex but not
necessarily smooth. Depending on the specific problem at hand, the \emph{regularizers}
$R$ and $H$ allow us to impose  additional structure on $w$ and
$z$, such as sparsity or set inclusion. Throughout, we only require that
the \emph{proximal maps} \citep{Parikh2014} for $R$ and $H$ can be computed
efficiently, as detailed in Section \ref{sec:algorithm}. Several examples of
this broad learning framework are discussed in Section \ref{sec:experiments},
including \emph{compressive sensing} with deep-net priors.

%\subsection{\edita{Empirical Risk }Minimization}
%\label{sec:error_min}
%\notea{Changing $x$ to $u$ for parameter. $u$ could be the labels, could be the image itself. This is to cover the general learning with GAN prior rather than just inverse problems.}
%We consider the optimization problem
%\begin{equation}
%\begin{array}{llll}
%& \underset{\up}{\text{minimize}}
%& & \loss(\up) \\
%& \text{subject to}
%& & \up \in \bigcup_{k=1}^K G_k(\Sprior)
%\end{array}
%\label{eq:problem_general}
%\end{equation}
%where we assume that the objective function $\loss$ as well as each $G_k$ for
%$k \in [K]$ are differentiable. The measurement error minimization problem
%corresponds to $\loss(\up)=\norm{A\up - b}_2^2$.  
%Finally, each constraint of the form $\up_k \in G_k(\Sprior)$ can be rewritten as
%$\up_k = G_k(\prior_k)$ for every $ \prior_k \in \Sprior$. 
%Writing $\Prior=[\prior_1, \ldots,
%\prior_K]$ we arrive at the optimization problem


==> sections/stat_guarantees_main_body.tex <==
Building upon the results in Section~\ref{sec:guarantees1}, the main result in
this section (Theorem \ref{thm:main_stat}) quantifies the convergence of the
iterates $\{w_t\}_{t\ge 0}$ of Algorithm~\ref{alg:admm} to the true parameter
$w^\n$.

In other words, Theorem~\ref{thm:main_stat_body} below controls the generalization
error of Program~\eqref{eq:emp loss min}, namely, the error  incurred by using
the empirical risk $L_m$ in lieu of the population risk $L$. Indeed,
Theorem \ref{thm:main} is silent about $\|w_t - w^\n\|_2$. Our findings in this
section are summarized below.
\begin{theorem}
\label{thm:main_stat_body}
\textbf{\emph{(Generalization error) }}
Suppose that Assumptions \ref{defn:Lm_scvx}-\ref{defn:G_iso} hold and recall
that the training samples $\{x_i\}_{i=1}^m$ are drawn independently from the
probability space $(\mathbb{X},\chi)$ for a compact set $\mathbb{X} \subset
\R^d$ with diameter $\operatorname{diam}(\mathbb{X})$.

For a set $W\subset\R^p$, let  $R=1_W$  be the indicator function on $W$, and
set $H=0$ in Program~(\ref{eq:emp loss min}). Suppose that solution $w^*$ of
Program \eqref{eq:emp loss min} belongs to the relative interior of $W$.
For $\varepsilon>0$, evaluate the quantities in Theorem \ref{thm:main} with
\begin{align}
    \mu_L = \s_L, \qquad&
    \nu_L = \zeta_L, \qquad &
\ol{\mu}_L = \ol{\zeta}_L =
4 \mathcal{R}_W(x_1,\cdots,x_m) +6 \s_l\operatorname{diam}(\mathbb{X}) \sqrt{\frac{\varepsilon+2}{2m}}
\end{align}
where $\mathcal{R}_W(x_1,\cdots,x_m)$ in the empirical  Rademacher complexity
defined in (\ref{eq:emp loss min}). If the requirements on the step sizes
in~(\ref{eq:step_size_reqs_thm}) hold, we then have that
\begin{align}
\|w_t- w^\n \|_2^2
\le   2\eta_{\rho}^t\widetilde{\Delta}_0 +
2\widetilde{\psi}_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2
+ \frac{18\s_l^2 \operatorname{diam}(\mathbb{X})^2( \varepsilon+2)}{m}
\end{align}
 except with a probability of at most $e^{-\varepsilon}$.
\end{theorem}
Most of the remarks about Theorem~\ref{thm:main} also apply to
Theorem~\ref{thm:main_stat} and we note that $\|w_t-w^\n\|_2$ reduces by
increasing the number of training samples $m$, before asymptotically reaching
the generalization error
\begin{align}
2\widetilde{\psi}_\rho + \frac{8 }{\zeta_L^2} \mathcal{R}_W(x_1,\cdots,x_m)^2.
\label{eq:statistical ball_body}
\end{align}
Computing the Rademacher complexity above for specific choices of the network
structure and loss is itself potentially a complicated task, which we will not
pursue by the virtue of the generality of our results so far. The key technical
challenge there is computing the corresponding \emph{entropy integral}, which
involves estimating the \emph{covering numbers} of the set $W$
\cite{mohri2018foundations}. One last takeaway point from the statistical
accuracy in \eqref{eq:statistical ball_body} is the following. If
\begin{align}
\widetilde{\psi}_\rho=O(\mathcal{R}_W(x_1,\cdots,x_m)^2/\zeta_L^2),
\label{eq:statistacll ball 2_body}
\end{align}
the asymptotic optimization error  in Theorem~\ref{thm:main} does not play an
important role in determining the generalization error above. In words, if
\eqref{eq:statistacll ball 2_body} holds, then Algorithm \ref{alg:admm} converges to
the ball of statistical accuracy around $w^\n$. Here, $O$ stands for the
standard Big-O notation. An extended version of this section that includes the proof of Theorem~\ref{thm:main_stat_body} appears in the supplementary material. 

